On Architecture to Architecture Mapping for Concurrency

Mapping programs from one architecture to another plays a key role in technologies such as binary translation, decompilation, emulation, virtualization, and application migration. Although multicore architectures are ubiquitous, the state-of-the-art translation tools do not handle concurrency primitives correctly. Doing so is rather challenging because of the subtle differences in the concurrency models between architectures. In response, we address various aspects of the challenge. First, we develop correct and efficient translations between the concurrency models of two mainstream architecture families: x86 and ARM (versions 7 and 8). We develop direct mappings between x86 and ARMv8 and ARMv7, and fence elimination algorithms to eliminate redundant fences after direct mapping. Although our mapping utilizes ARMv8 as an intermediate model for mapping between x86 and ARMv7, we argue that it should not be used as an intermediate model in a decompiler because it disallows common compiler transformations. Second, we propose and implement a technique for inserting memory fences for safely migrating programs between different architectures. Our technique checks robustness against x86 and ARM, and inserts fences upon robustness violations. Our experiments demonstrate that in most of the programs both our techniques introduce significantly fewer fences compared to naive schemes for porting applications across these architectures.

==> app-compositional.tex <==
% !TEX root = paper.tex

\section{Compositional Fence Elimination}
\label{app:compositional}

%Now we prove the theorem for x86, ARMv8, ARMv7, and ARMv7-mca.

Suppose $\ex$ is a consistent execution of $\mbbp$ and $\cyc(\mbbp,R)$ holds. 
In this case for all $a,b \in \ex.\E$ if $a,b \in \cyc(\mbbp,R)$ then $\ex.\lpo(a,b) \implies R(a,b)$. 


\paragraph{x86}

We restate the theorem \cref{th:xcycfenceelim} and then prove the same.

\xcycfenceelim*

\begin{proof}

From definition $(a,b) \notin \cyc(\srcp)$ and therefore $(a,b) \notin \cyc(\tgtp)$ as well. 

Let $\ex_t$ be a consistent execution of $\tgtp$ and $\ex_s$ be the corresponding execution from $\srcp$ 
with intermediate fence between $a$ and $b$. 

In this case $\ex_s.\lrf =\ex_t.\lrf$, $\ex_s.\co =\ex_t.\co$, $\ex_s.\fr =\ex_t.\fr$ hold. 

$\ex_s$ satisfies (irrHB), (irrFRHB) as we already know that $\ex_s.\lrf =\ex_t.\lrf$, $\ex_s.\co =\ex_t.\co$, $\ex_s.\fr =\ex_t.\fr$ hold. 

(irrFRMO)
We know that $\ex_s.\fr;\ex_s.\mo \implies \ex_s.\fr;\ex_s.\co \implies \ex_t.\fr;\ex_t.\co \implies \ex_t.\fr;\ex_t.\mo$. 
However, we know (irrFRMO) holds on $\ex_t$. 
Therefore $\ex_s$ satisfies (irrFRMO).

\bigskip

It remains to show that rest of the x86 axioms also hold.

Let $c$ be the introduced fence event in $\ex_s$.  

Let $W = \ex_s.\Wlab \cup \ex_s.\Ulab \cup \ex_s.\Flab$.

In this case 

$\ex_s.\mo = \ex_t.\mo \cup O \times [\set{c}] \cup [\set{c}] \times (W \setminus O)$ where 

$O \subseteq W$ and $[O];\ex_s.\mo^?;\ex_s.\rfe^?;\ex_s.\lpo;[\set{c}]$. 

%Note that $[O];\ex_s.\mo^?;\ex_s.\rfe^?;\ex_s.\lpo;[\set{c}];\ex_s.\mo;[W \setminus O]$
%
%$\implies $
%
%
%Therefore $\ex_s.\mo$ is total as $\ex_t$ satisfies (irrFMRP).


(irrMOHB)

Assume $c$ introduces a $\ex_s.\mo;\ex_s.\xhb$ cycle. 

However, from definition of $\ex_s.\mo$,
$[\set{c}];\ex_s.\xhb;[\ex_s.\Wlab \cup \ex_s.\Ulab \cup \ex_s.\Flab]$ 

$\implies [\set{c}];\ex_s.\mo;[\ex_s.\Wlab \cup \ex_s.\Ulab \cup \ex_s.\Flab]$

Hence a contradiction and therefore $\ex_s$ satisfies (irrMOHB).

\medskip
(irrFMRP)

Assume $\ex_s.\fr;\ex_s.\mo;\ex_s.\rfe;\ex_s.\lpo$ creates a cycle.
However, $\ex_s.\fr;\ex_s.\mo;\ex_s.\rfe;\ex_s.\lpo$

$\implies \ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo;[\ex_s.\WUlab];\ex_s.\rfe;\ex_s.\lpo$ and therefore $c$ is not on the cycle.

$\implies \ex_t.\fr;[\ex_t.\WUlab];\ex_t.\mo;[\ex_t.\WUlab];\ex_t.\rfe;\ex_t.\lpo$ 

We know $\ex_t$ satisfies (irrFMRP) and therefore $\ex_s$ also satisfies (irrFMRP).

\medskip
(irrUF)

Assume $\ex_s.\fr;\ex_s.\mo;[\ex_s.\Ulab \cup \ex_s.\Flab];\ex_s.\lpo$ creates a cycle through $c$.

Therefore $\ex_s.\fr;\ex_s.\mo;[\set{c}];\ex_s.\lpo$ is a cycle.

From the definition of $\ex_s.\mo$

$\ex_s.\fr;\ex_s.\mo;[\set{c}];\ex_s.\lpo$ is a cycle.

Therefore $\ex_s.\mo;[\set{c}];\ex_s.\lpo;\ex_s.\fr$ is a cycle.

Considering the subcases:

\Subcase{$\ex_s.\mo;[\set{c}];\ex_s.\lpo;\ex_s.\fri$ is a cycle.}

It implies $[O];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\rfe^?;\ex_s.\lpo;[\set{c}];\ex_s.\lpo$ is a cycle.

It implies $[O];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\xhb$ is a cycle.

It implies $[\ex_t.\WUlab \cup \ex_t.\Flab];\ex_t.\mo^?;[\ex_t.\WUlab];\ex_t.\xhb$ is a cycle. 

This is a contradiction as $\ex_t$ satisfies (irrHB) and (irrMOHB).


\Subcase{$\ex_s.\mo;[\set{c}];\ex_s.\lpo;\ex_s.\fre$ is a cycle.}

It implies $[O];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\rfe^?;\ex_s.\lpo;[\set{c}];\ex_s.\lpo;\ex_s.\fre$ is a cycle.

Two subcases:

(i) $[O];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\lpo;[\set{c}];\ex_s.\lpo;\ex_s.\fre$ is a cycle.

(ii) $[O];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\rfe;[\ex_s.\Rlab];\ex_s.\lpo;[\set{c}];\ex_s.\lpo;\ex_s.\fre$ is a cycle.

\textbf{subcase (i)}

It implies $[\ex_s.\Wlab \cup \ex_s.\Ulab \cup \ex_s.\Flab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\lpo;\ex_s.\fre$ is a cycle.

It implies $[\ex_t.\Wlab \cup \ex_t.\Ulab \cup \ex_t.\Flab];\ex_t.\mo^?;[\ex_t.\WUlab];\ex_t.\lpo;\ex_t.\fre$ is a cycle which 
is a contradiction.

\textbf{subcase (ii)}

It implies $[O];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\rfe;[\set{a}];\ex_s.\lpo;[\set{c}];\ex_s.\lpo;[\set{b}];\ex_s.\fre$ is a cycle.

From the definition of $\cyc$, we also know that $\ex_s.R(-,a) \land \ex_s.R(b,-)$ is not possible where $R = \rfe \cup \coe \cup \fre$. 

Therefore a contradiction.

\bigskip

As a result, $\ex_s$ is x86 consistent and $\behav(\ex_s) = \behav(\ex_t)$ holds as $\ex_s.\co \iff \ex_t.\co$.

\end{proof}

\paragraph{ARMv8}

We restate the theorem \cref{th:armv8cycfenceelim} and then prove the same.

\armvacycfenceelim*

\begin{proof}

From definition $(a,b) \notin \cyc(\srcp)$ and therefore $(a,b) \notin \cyc(\tgtp)$ as well. 

Let $\ex_t$ be a consistent execution of $\tgtp$ and $\ex_s$ be the corresponding execution from $\srcp$ 
with intermediate fence between $a$ and $b$. 

In this case $\ex_s.\lrf =\ex_t.\lrf$, $\ex_s.\co =\ex_t.\co$, $\ex_s.\fr =\ex_t.\fr$, $\ex_s.\poloc = \ex_t.\poloc$ hold. 

Therefore $\ex_s$ satisfies (internal) as $\ex_t$ satisfies (internal) and (atomic).

\medskip

(external)

In this case $\ex_s.\bob = \ex_t.\bob \cup \set{(a,b)}$. 

However, from the definition of $\cyc$, we also know that $\ex_s.R(-,a) \land \ex_s.R(b,-)$ is not possible where $R = \rfe \cup \coe \cup \fre$. 

As a result, $\ex_s$ does not have any $\ob$ cycle and $\ex_s$ supports (external). 

\bigskip

As a result, $\ex_s$ is x86 consistent and $\behav(\ex_s) = \behav(\ex_t)$ holds as $\ex_s.\co \iff \ex_t.\co$.

\end{proof}


\paragraph{ARMv7/ARMv7-mca}

We restate the theorem \cref{th:armv7cycfenceelim} and then prove the same.

\armvscycfenceelim*

\begin{proof}

From definition $(a,b) \notin \cyc(\srcp)$ and therefore $(a,b) \notin \cyc(\tgtp)$ as well. 

Let $\ex_t$ be a consistent execution of $\tgtp$ and $\ex_s$ be the corresponding execution from $\srcp$ 
with intermediate fence between $a$ and $b$. 

In this case $\ex_s.\lrf =\ex_t.\lrf$, $\ex_s.\co =\ex_t.\co$, $\ex_s.\fr =\ex_t.\fr$, $\ex_s.\poloc = \ex_t.\poloc$ hold. 

Therefore $\ex_s$ satisfies (total-mo), (sc-per-loc), and (atomicity) as $\ex_t$ satisfies (total-mo), (sc-per-loc), and (atomicity).

(observation), (propagation), (no-thin-air)

From the definition of $\cyc$, we know that $\ex_s.R(-,a) \land \ex_s.R(b,-)$ is not possible where $R = \rfe \cup \coe \cup \fre$. 

Hence the introduced $\fence$ relation does not create any cycle in $\ex_s$ and as a result, $\ex_s$ is consistent. 

Moreover,  $\behav(\ex_s) = \behav(\ex_t)$ holds as $\ex_s.\co \iff \ex_t.\co$.
\end{proof}

\subsection{Robustness Analysis}
\label{app:robustness}

\paragraph{x86}

We restate x86-robust against SC theorem \cref{th:xsc} and prove the same. 

\xsc*

\begin{proof}

%Let $\ex$ be an execution of $\mbbp$. 

We show that $(\ex.\lpo \cup \ex.\lrf \cup \ex.\fr \cup \ex.\co)$ is acyclic by contradiction.

Assume  $(\ex.\lpo \cup \ex.\lrf \cup \ex.\fr \cup \ex.\co)$ creates a cycle.

We know that the cycle has atleast one write access.

If there is one write access then it can create a $\ex.\lrf;\ex.\fr$ cycle which violates (irrFRHB). 

Hence there are more than one write events on the cycle. 

Let $(w,w')$ is immediate pair of writes on $(\ex.\lpo \cup \ex.\lrf \cup \ex.\fr \cup \ex.\co)$  cycle.

Possible cases:

\Case{$\ex.\co(w,w')$}

It implies $\ex.\mo(w,w')$.

\bigskip

\Case{$\ex.\lpo(w,w')$}

It implies $\ex.\mo(w,w')$.

\bigskip

\Case{$(w,w') \in \ex.\lrf;\ex.\lpo^?;\ex.\fr$}

It implies $w.\lloc = r.\lloc = w'.\lloc$.

Therefore $\ex.\co(w,w')$ holds from \cref{lem:noloadx}.

It implies $\ex.\mo(w,w')$ holds.

\bigskip

\Case{$(w,w') \in \ex.\poloc;\ex.\fr$}

Therefore $\ex.\co(w,w')$ holds from \cref{lem:noloadx}.

It implies $\ex.\mo(w,w')$ holds.

\bigskip

\Case{$(w,w') \in \ex.\po;[\Flab];\ex.\lpo;\ex.\fr$}

In this case $\ex.\mo(w,w')$ as it otherwise violates (irrUF).

\bigskip

Therefore a $(\ex.\lpo \cup \ex.\lrf \cup \ex.\fr \cup \ex.\co)$  cycle implies a $\ex.\mo$ cycle which is a contradiction. 

Therefore $(\ex.\lpo \cup \ex.\lrf \cup \ex.\fr \cup \ex.\co)$ is acyclic and as a result $\ex$ is SC.

\end{proof}

\paragraph{ARMv8}

We restate \cref{th:armasc} and prove the same.

\armasc*

\begin{proof}
%Let $\ex$ be an execution of $\mbbp$. 


We show $(\ex.\lpo \cup \ex.\lrf \cup \ex.\fr \cup \ex.\co)$ is acyclic by contradiction.

Assume  $(\ex.\lpo \cup \ex.\lrf \cup \ex.\fr \cup \ex.\co)$ creates a cycle.

It implies $(\ex.\epo \cup \ex.\rfe \cup \ex.\coe \cup \ex.\fre)$ creates a cycle.

It implies $\ex.\poloc \cup (\ex.\aob \cup \ex.\bob \cup \ex.\bob)^+  \cup \ex.\rfe \cup \ex.\coe \cup \ex.\fre$ creates a cycle.

Considering a $\ex.\poloc \cup \ex.\rfe \cup \ex.\coe \cup \ex.\fre$ cycle, possible cases:

(1) $[\Rlab];\ex.\poloc;[\Rlab];\ex.\fre;[\Wlab] \implies [\Rlab];\ex.\fre$

(2) $[\Wlab];\ex.\poloc;[\Rlab];\ex.\fre;[\Wlab] \implies [\Wlab];\ex.\coe$

(3) $[\Wlab];\ex.\rfe;[\Rlab];\ex.\poloc;[\Wlab] \implies [\Wlab];\ex.\coe$

(4) $(\ex.\coe \cup \ex.\fre);[\Wlab];\ex.\poloc;[\Wlab] \implies \ex.\coe \cup \ex.\fre$

Therefore a $\ex.\poloc \cup (\ex.\aob \cup \ex.\bob \cup \ex.\bob)^+  \cup \ex.\rfe \cup \ex.\coe \cup \ex.\fre$ implies 
a $(\ex.\aob \cup \ex.\bob \cup \ex.\bob)^+  \cup \ex.\rfe \cup \ex.\coe \cup \ex.\fre$ cycle.

It implies an $\ex.\ob$ cycle which violates (external) and therefore a contradiction.
\end{proof}


%\begin{restatable}{theorem}{x86A}
%\label{th:x86A}
%x86 and x86A are equivalent.
%\end{restatable}

We restate the theorem and then prove the same.

\xA*


\begin{proof}
We show that for a program $\mbbp$, for each x86 execution there exist a corresponding x86A execution and vice versa. 

($\Rightarrow$)

We show $\forall \ex \in \denot{\mbbp}_{x86} \exists \ex_a \in \denot{\mbbp}_{\mathsf{x86A}}.~\behav(\ex) = \behav(\ex_a)$.

Given an $\ex \in \denot{\mbbp}_{x86}$ we define $\ex_a$ such that

\begin{itemize}

\item $\ex.\Flab \implies \ex_a.\dmbfull$

\item $\ex.\lpo;[\Ulab] \implies \ex_a.\lpo;[\Rlab] \cup \ex_a.\lpo;[\Wlab]$ as $\rmw \subseteq \lpo$ 

\item $[\Ulab];\lpo \implies [\Rlab];\ex_a.\lpo \cup [\Wlab];\ex_a.\lpo;$ as $\rmw \subseteq \lpo$ 

\item $[\Ulab];\ex.\lrf \implies [\codom(\rmw)];\ex_a.\lrf$

\item $\ex.\lrf;[\Ulab] \implies \ex_a.\lrf;[\dom(\rmw)]$

\item $[\Ulab];\ex.\mo \implies [\codom(\rmw)];\ex_a.\mo$

\item $\ex.\mo;[\Ulab] \implies \ex_a.\mo;[\codom(\rmw)]$
\end{itemize}

%Therefore 
%
%$\ex_a.\E = \ex.\E[\Ulab \mapsto [\Rlab]\rmw;[\Wlab]]$
%
%$\ex_a.\lpo = (\ex.\lpo \cup [\ex_a.\Rlab];\rmw;[\ex_a.\Wlab] \setminus ([\Ulab];\ex.\lpo \cup \ex.\lpo;[\Ulab]))^+$ 
%
%$\ex_a.\lrf = \ex.\lrf \cup \ex.\lrf;[\dom(\rmw)] \cup [\codom(\rmw)];\ex.\lrf  \setminus (\ex.\lrf;[\Ulab] \cup [\Ulab];\ex.\lrf)$
%
%$\ex_a.\mo = \ex.\mo \cup \ex.\mo;[\codom(\rmw)] \cup [\codom(\rmw)];\ex.\mo \setminus (\ex.\mo;[\Ulab] \cup [\Ulab];\ex.\mo)$


Now we show that $\ex_a$ is x86A consistent.

(AirrHB)

Assume $\ex_a.\xhb$ creates a cycle.

It implies $(\ex_a.\lpo \cup \ex_a.\lrf)^+$ creates a cycle.

From definition, it implies $(\ex.\lpo \cup \ex.\lrf)^+$ creates a cycle which contradicts (irrHB). 

Therefore (AirrHB) holds.

\medskip

(AirrMOHB)

Assume $\ex_a.\mo;\ex_a.\xhb$ creates a cycle.

It implies $\ex_a.\mo;(\ex_a.\lpo \cup \ex_a.\lrf)^+$ creates a cycle.

From definition, it implies $\ex.\mo;(\ex.\lpo \cup \ex.\lrf)^+$ creates a cycle which contradicts (irrMOHB). 

Therefore (AirrMOHB) holds.

\medskip

(AirrFRHB)

Assume $\ex_a.\fr;\ex_a.\xhb$ creates a cycle.

It implies $\ex_a.\fr;(\ex_a.\lpo \cup \ex_a.\lrf)^+$ creates a cycle.

From definition, it implies $\ex.\fr;(\ex.\lpo \cup \ex.\lrf)^+$ creates a cycle which contradicts (irrFRHB). 

Therefore (AirrFRHB) holds.

\medskip

(AirrFMRP)

Assume $\ex_a.\fr;\ex_a.\mo;\ex_a.\rfe;\ex_a.\lpo$ creates a cycle.

It implies $\ex.\fr;\ex.\mo;\ex.\rfe;\ex.\lpo$ creates a cycle which contradicts (irrFMRP). 

Therefore (AirrFMRP) holds.

\medskip

(AirrUF)

Assume $\ex_a.\fr;\ex_a.\mo;[\codom(\ex_a.\rmw) \cup \ex.\dmbfull];\ex_a.\lpo$ creates a cycle.

It implies $\ex.\fr;\ex.\mo;[\ex.\Ulab \cup \ex.\Flab];\ex.\lpo$ creates a cycle which contradicts (irrUF). 

Therefore (AirrUF) holds.

\medskip

Therefore $\ex_a \in \denot{\mbbp}_{\mathsf{x86A}}$ and $\behav(\ex_a) = \behav(\ex)$ holds from definition of $\ex_a$.

\bigskip

($\Leftarrow$)


$\forall \ex_a \in \denot{\mbbp}_{\mathsf{x86A}} \exists \ex \in \denot{\mbbp}_{x86}.~\behav(\ex) = \behav(\ex_a)$

Now we show that $\ex$ is x86 consistent.



(irrHB)

Assume $\ex.\xhb$ creates a cycle.

It implies $(\ex.\lpo \cup \ex.\lrf)^+$ creates a cycle.

From definition, it implies $(\ex_a.\lpo \cup \ex_a.\lrf)^+$ creates a cycle which contradicts (AirrHB). 

Therefore (AirrHB) holds.

\medskip

(irrMOHB)

Assume $\ex.\mo;\ex.\xhb$ creates a cycle.

It implies $\ex.\mo;(\ex.\lpo \cup \ex.\lrf)^+$ creates a cycle.

From definition, it implies $\ex_a.\mo;(\ex_a.\lpo \cup \ex_a.\lrf)^+$ creates a cycle which contradicts (AirrMOHB). 

Therefore (irrMOHB) holds.

\medskip

(irrFRHB)

Assume $\ex.\fr;\ex.\xhb$ creates a cycle.

It implies $\ex.\fr;(\ex.\lpo \cup \ex.\lrf)^+$ creates a cycle.

From definition, it implies $\ex_a.\fr;(\ex_a.\lpo \cup \ex_a.\lrf)^+$ creates a cycle which contradicts (AirrFRHB). 

Therefore (irrFRHB) holds.

\medskip

(irrFMRP)

Assume $\ex.\fr;\ex.\mo;\ex.\rfe;\ex.\lpo$ creates a cycle.

It implies $\ex_a.\fr;\ex_a.\mo;\ex_a.\rfe;\ex_a.\lpo$ creates a cycle which contradicts (irrFMRP). 

Therefore (irrFMRP) holds.

\medskip

(irrUF)

Assume $\ex_a.\fr;\ex_a.\mo;[\codom(\ex_a.\rmw) \cup \ex.\dmbfull];\ex_a.\lpo$ creates a cycle.

It implies $\ex.\fr;\ex.\mo;[\ex.\Ulab \cup \ex.\Flab];\ex.\lpo$ creates a cycle which contradicts (irrUF). 

Therefore (AirrUF) holds.

\medskip

Therefore $\ex \in \denot{\mbbp}_{x86}$ and $\behav(\ex_a) = \behav(\ex)$ holds from definition of $\ex$.

\end{proof}




We restate \cref{th:robustarmax} and prove the same.

\robustarmax*

\begin{proof}
%For an execution $\ex$ of ARMv8 program $\mbbp$ which follows $\cyc$ from  \cref{th:robustarmax} 
%satisfies ARM-x86 constraints.

We show that ARMv8 consistent execution $\ex$ satisfies x86A constraints. 

We set the $\mo$ relation as follows:

$\ob \cup [\dmbfull];\lpo;\fr^? \cup \lpo;[\dmbfull] \cup \coi \implies \mo$

(AirrHB)

Assume $\ex.\xhb$ is a cycle. 

$\implies (\ex.\epo \cup \ex.\rfe)^+$ is a cycle.

$\implies (\ex.\poloc \cup \ex.\xwr \cup (\ex.\aob \cup \ex.\bob \cup \ex.\dob)^+ \cup \ex.\rfe)^+$ is a cycle.

$\implies ((\ex.\aob \cup \ex.\bob \cup \ex.\dob)^+ \cup \ex.\coe \cup \ex.\rfe)^+$ is a cycle as 

$[\Wlab];\rfe;[\Rlab]\poloc;[\Wlab] \implies \coe$ and $\codom(\ex.\xwr) \cap \dom(\ex.\rfe) = \emptyset$.

$\implies \ex.\ob$ is a cycle. 

This is a contradiction and therefore $\ex$ satisfies (AirrHB). 

\medskip

(AirrMOHB)

Assume $\ex.\mo;[\Wlab \cup \Llab \cup \dmbfull]\ex.\xhb;[\Wlab \cup \Llab \cup \dmbfull]$ is a cycle. 

It implies $\ex.\mo;[\Wlab \cup \Llab]\ex.\xhb;[\Wlab \cup \Llab] \cup [\dmbfull];\ex.\lpo \cup \ex.\lpo;[\dmbfull]$ is a cycle.

It implies $\ex.\mo;[\Wlab \cup \Llab];(\ex.\lpo;[\Wlab \cup \Llab])^?;\ex.\ob;[\Wlab \cup \Llab] \cup [\dmbfull];\ex.\lpo \cup \ex.\lpo;[\dmbfull]$ is a cycle.

It implies $\ex.\mo;[\Wlab \cup \Llab];\ex.\ob;[\Wlab \cup \Llab] \cup [\dmbfull];\ex.\lpo \cup \ex.\lpo;[\dmbfull]$ is a cycle.

It implies $\ex.\mo;[\Wlab \cup \Llab]\ex.\mo;[\Wlab \cup \Llab] \cup [\dmbfull];\ex.\mo \cup \ex.\mo;[\dmbfull]$ is a cycle.

It implies $\ex.\mo$ is a cycle which is a contradiction.

Therefore $\ex$ satisfies (AirrMOHB).

\medskip

(AirrFRHB)

Assume a $\ex.\fr;\ex.\xhb$ cycle.

Two cases 

\Case{$\ex.\fri;\ex.\xhb$ cycle}

It implies $\ex.\fr;\ex.\poloc$ cycle.

Hence a contradiction as $\ex$ satisfies (internal)

\Case{$\ex.\fre;\ex.\xhb$ cycle}

It implies $\ex.\fre;\ex.\xhb$ cycle

It implies $\ex.\fre;[\Wlab \cup \Llab];(\ex.\epo \cup \ex.\rfe)^+;[\Rlab \cup \Alab]$ cycle

It implies $\ex.\fre;[\Wlab \cup \Llab];\ex.\ob;[\Rlab \cup \Alab]$ cycle from the definition of $\epo$.

It implies $\ex.\ob$ cycle which is a contradiction.

Therefore $\ex$ satisfies (AirrFRHB). 

\medskip

%(AirrFRMO)
%
%Assume $\ex.\fr;\ex.\mo$ is a cycle.
%
%It implies $\ex.\fr;\ex.\co$ is a cycle.
%
%It is a contradiction as $\ex$ satisfies (internal).
%
%Therefore $\ex$ satisfies (AirrFRMO).
%
%\medskip

(AirrFMRP)

Assume $\ex.\fr;[\Wlab \cup \Llab];\ex.\mo;[\Wlab \cup \Llab];\ex.\rfe;[\Rlab \cup \Alab];\ex.\lpo;[\Rlab \cup \Alab]$ is a cycle.

It implies $[\Rlab \cup \Alab];\ex.\lpo;[\Rlab \cup \Alab];\ex.\fr;[\Wlab \cup \Llab];\ex.\mo;[\Wlab \cup \Llab];\ex.\rfe$ is a cycle.

If $[\Rlab \cup \Alab];\ex.\lpo;[\Rlab \cup \Alab] \subseteq [\Rlab \cup \Alab];\ex.\poloc;[\Rlab \cup \Alab]$ 
then there is a cycle on the same location which violates (sc-per-loc) for $\ex$. 
Therefore a contradiction and $\ex$ satisfies (AirrFMRP).

\medskip

\textbf{Otherwise.}

$[\Rlab \cup \Alab];\ex.\lpo;[\Rlab \cup \Alab] \implies [\Rlab \cup \Alab];\ex.\obi;[\Rlab \cup \Alab]$ where $\obi = \ob \cap \lpo$ and $\obe = \ob \setminus \lpo$.

Moreover, in this case $[\Wlab \cup \Llab];\ex.\mo;[\Wlab \cup \Llab]$ results from $[\Wlab \cup \Llab];\ex.\ob;[\Wlab \cup \Llab]$.

Now $[\Wlab \cup \Llab];\ex.\ob;[\Wlab \cup \Llab] \implies [\Wlab \cup \Llab];\ex.\obi;[\Wlab \cup \Llab] \cup [\Wlab \cup \Llab];\ex.\obe;[\Wlab \cup \Llab]$ 

In case of $[\Wlab \cup \Llab];\ex.\obi;[\Wlab \cup \Llab]$, it creates a $\poloc;\lrf$ cycle violates (sc-per-loc) in $\ex$.

Therefore a contradiction and $\ex$ satisfies (AirrFMRP).

Now we consider, 

$[\Rlab \cup \Alab];\ex.\obi;[\Rlab \cup \Alab];\ex.\fr;[\Wlab \cup \Llab];\ex.\obe;[\Wlab \cup \Llab];\ex.\rfe$ is a cycle.

Case split on $\ex.\fr$:
\[
\inarr{
[\Rlab \cup \Alab];\ex.\obi;[\Rlab \cup \Alab];\ex.\fri;[\Wlab \cup \Llab];\ex.\obe;[\Wlab \cup \Llab];\ex.\rfe 
\\ \cup [\Rlab \cup \Alab];\ex.\obi;[\Rlab \cup \Alab];\ex.\fre;[\Wlab \cup \Llab];\ex.\obe;[\Wlab \cup \Llab];\ex.\rfe  
}
\]

Consider $[\Rlab \cup \Alab];\ex.\obi;[\Rlab \cup \Alab];\ex.\fre;[\Wlab \cup \Llab];\ex.\obe;[\Wlab \cup \Llab];\ex.\rfe$

$\implies [\Rlab \cup \Alab];\ex.\obi;[\Rlab \cup \Alab];\ex.\obe;[\Wlab \cup \Llab];\ex.\obe;[\Wlab \cup \Llab];\ex.\obe$

$\implies [\Rlab \cup \Alab];\ex.\ob$

Now consider $[\Rlab \cup \Alab];\ex.\obi;[\Rlab \cup \Alab];\ex.\fri;[\Wlab \cup \Llab];\ex.\obe;[\Wlab \cup \Llab];\ex.\rfe$

considering $[\Wlab \cup \Llab];\ex.\obe;[\Wlab \cup \Llab]$, 

it implies $[\Wlab \cup \Llab];\ex.\lpo^?;(\ex.\coe \cup \ex.\rfe \cup \ex.\rfe);\ex.\ob^?;[\Wlab \cup \Llab]$

Therefore $[\Rlab \cup \Alab];\ex.\obi;[\Rlab \cup \Alab];\ex.\fri;[\Wlab \cup \Llab];\ex.\obe;[\Wlab \cup \Llab];\ex.\rfe$ is a cycle.

Now $[\Wlab \cup \Llab];\ex.\obe;[\Wlab \cup \Llab]$
  
$\implies [\Wlab \cup \Llab];\ex.\lpo^?;\ex.\obs;\ex.\ob^?;[\Wlab \cup \Llab]$

Therefore $[\Rlab \cup \Alab];\ex.\obi;[\Rlab \cup \Alab];\ex.\fri;[\Wlab \cup \Llab];(\ex.\lpo;[\Wlab \cup \Llab])^?;\ex.\obs;\ex.\ob^?;[\Wlab \cup \Llab];\ex.\rfe$ is a cycle.

Now we consider the $[\Rlab \cup \Alab];\ex.\obi;[\Rlab \cup \Alab];\ex.\fri;[\Wlab \cup \Llab];(\ex.\lpo;[\Wlab \cup \Llab])^?$ component.

Considering cases for $[\Rlab \cup \Alab];\ex.\obi;[\Rlab \cup \Alab];\ex.\fri;[\Wlab \cup \Llab];(\ex.\lpo;[\Wlab \cup \Llab])^?$

\medskip

\Subcase{$[\Rlab \cup \Alab];\ex.\poloc;[\Rlab \cup \Alab]$}
 
In this case $[\Rlab \cup \Alab];\ex.\poloc;[\Rlab \cup \Alab];\ex.\obs \implies [\Rlab \cup \Alab];\ex.\fre$.

Therefore $[\Rlab \cup \Alab];\ex.\fre;\ex.\ob^?;[\Wlab \cup \Llab];\ex.\rfe$ is a cycle.

It implies $[\Rlab \cup \Alab];\ex.\ob;\ex.\ob^?;[\Wlab \cup \Llab];\ex.\ob$ is a cycle which is a contradiction.
 
\medskip

\Subcase{$[\Rlab \cup \Alab];\ex.\poloc;[\Wlab \cup \Llab]$}

In this case $[\Wlab \cup \Llab];\ex.\rfe;[\Rlab \cup \Alab];\ex.\poloc$ is a cycle which violates (sc-per-loc).which is a contradiction.

\Subcase{$[\Rlab \cup \Alab];(\ex.\lpo \setminus \ex.\poloc)$}
 
It implies $[\Rlab \cup \Alab];(\ex.\aob \cup \ex.\dob \cup \ex.\bob)^+$

It implies $[\Rlab \cup \Alab];\ex.\ob$.

Therefore it results in a $[\Rlab \cup \Alab];\ex.\ob;\ex.\obs;\ex.\ob^?;\ex.\rfe$ cycle. 

It implies a $\ex.\ob$ cycle which is a contradiction.

Therefore $\ex$ satisfies (AirrFMRP).

(AirrUF)

Assume $\ex.\fr;[\Wlab \cup \Llab];\ex.\mo;[\codom(\ex.\rmw) \cup \ex.\dmbfull];\ex.\lpo;[\Rlab \cup \Alab]$ is a cycle.

It implies $\ex.\mo;[\codom(\ex.\rmw) \cup \ex.\dmbfull];\ex.\lpo;[\Rlab \cup \Alab];\ex.\fr;[\Wlab \cup \Llab]$ is a cycle.

It implies $\ex.\mo;[\codom(\ex.\rmw) \cup \ex.\dmbfull];\ex.\lpo;[\Rlab \cup \Alab];\ex.\fr;[\Wlab \cup \Llab]$ is a cycle.


\Subcase{$\ex.\mo;[\codom(\ex.\rmw)];\ex.\lpo;[\Rlab \cup \Alab];\ex.\fr;[\Wlab \cup \Llab]$ is a cycle.}

It implies $\ex.\mo;[\codom(\ex.\rmw)];\ex.\bob;\ex.\fre^?;[\Wlab \cup \Llab]$ is a cycle.

It implies $\ex.\mo;[\codom(\ex.\rmw)];\ex.\ob;[\Wlab \cup \Llab]$ is a cycle.

It implies $\ex.\mo;[\codom(\ex.\rmw)];\ex.\mo;[\Wlab \cup \Llab]$ is a cycle.

This is a contradiction and therefore  $\ex$ satisfies (AirrUF).

\medskip

\Subcase{$\ex.\mo;[\ex.\dmbfull];\ex.\lpo;[\Rlab \cup \Alab];\ex.\fr;[\Wlab \cup \Llab]$ is a cycle.}

\textbf{subcase} 

$\ex.\mo;[\ex.\dmbfull];\ex.\lpo;[\Rlab \cup \Alab];\ex.\fri;[\Wlab \cup \Llab]$ is a cycle.

$\implies \ex.\mo;[\ex.\dmbfull];\ex.\mo;[\Wlab \cup \Llab]$ is a cycle.

This is a contradiction and therefore  $\ex$ satisfies (AirrUF).

\textbf{subcase} 

$\ex.\mo;[\ex.\dmbfull];\ex.\lpo;[\Rlab \cup \Alab];\ex.\fre;[\Wlab \cup \Llab]$ is a cycle.

$\implies \ex.\mo;[\ex.\dmbfull];\ex.\mo;[\Wlab \cup \Llab]$ is a cycle.

This is a contradiction and therefore  $\ex$ satisfies (AirrUF).

\end{proof}


\paragraph{ARMv7}


We restate \cref{th:robustarmssc} and prove the same.

\robustarmssc*

\begin{proof}

We show that $(\ex.\lpo \cup \ex.\lrf \cup \ex.\fr \cup \ex.\co)$ is acyclic by contradiction.

Assume  $(\ex.\lpo \cup \ex.\lrf \cup \ex.\fr \cup \ex.\co)$ creates a cycle.

It implies $(\ex.\lpo \cup \ex.\rfe \cup \ex.\fre \cup \ex.\coe)$ creates a cycle.

In that case $(\ex.\poloc \cup \ex.\fence \cup \ex.\rfe \cup \ex.\fre \cup \ex.\coe)$ creates a cycle.

Considering the incoming and outgoing edges for $\ex.\poloc$:

$[\Rlab];\ex.\poloc;[\Rlab];\ex.\fre \implies [\Rlab];\ex.\fre$

$[\Wlab];\ex.\rfe;[\Rlab];\ex.\poloc;[\Wlab] \implies [\Wlab];\ex.\coe$

$(\ex.\fre \cup \ex.\coe);[\Wlab];\ex.\poloc;[\Wlab] \implies (\ex.\fre \cup \ex.\coe)$

$[\Wlab];\ex.\poloc;[\Rlab];\ex.\fre \implies [\Wlab];\ex.\coe$

It implies  $(\ex.\fence \cup \ex.\rfe \cup \ex.\fre \cup \ex.\coe)$ creates a cycle.

Now we consider $[\codom(fence)];(\ex.\rfe \cup \ex.\fre \cup \ex.\coe);[\dom(fence)]$ path.

Possible cases:

\Case{$[\Rlab];(\ex.\rfe \cup \ex.\fre \cup \ex.\coe);[\Rlab]$}

It implies $\ex.\fre;\ex.\rfe$.

\smallskip

\Case{$[\Rlab];(\ex.\rfe \cup \ex.\fre \cup \ex.\coe);[\Wlab]$}

It implies $\ex.\fre$

\smallskip

\Case{$[\Wlab];(\ex.\rfe \cup \ex.\fre \cup \ex.\coe);[\Wlab]$}

It implies $\ex.\coe$

\smallskip

\Case{$[\Wlab];(\ex.\rfe \cup \ex.\fre \cup \ex.\coe);[\Rlab]$}

It implies $\ex.\coe;\ex.\rfe$

Thus an $(\ex.\fence \cup \ex.\rfe \cup \ex.\fre \cup \ex.\coe)$ cycle implies 

a $((\ex.\coe \cup \ex.\fre);\ex.\rfe^?;\ex.\fence)^+$ cycle.

It implies a $\prop^+$ cycle which violates (propagation).

Hence a contradiction and therefore SC is preserved.

%\Case{$\robust(\mbbp,\slocs)$} 
%
%In this case the cycle is on same-location events. 
%However, it violates (sc-per-loc) in $\ex$ which is a contradiction.
%
%\Case{$\robust(\mbbp, \poloc;[\Rlab] \cup \ppo \cup \fence)$} 
%
%In this case the inter-thread events are related by $\rfe \cup \coe \cup \fre$ and 
%$\ex.\epo \subseteq  \ex.\poloc;[\Rlab] \cup \ex.\ppo \cup \ex.\fence$.
%
%
%Assume $(\ex.\lpo \cup \ex.\rfe \cup \ex.\fre \cup \ex.\coe)$ creates a cycle.
%
%It implies $(\ex.\poloc;[\Rlab];\ex.\fre \cup \ex.\ppo \cup \ex.\fence \cup\ex.\rfe \cup \ex.\fre \cup \ex.\coe)$ creates a cycle.
%
%We know $[\Rlab];\poloc;[\Rlab];\fre \implies \fre$ and $[\Wlab];\poloc;[\Rlab];\fre \implies \coe$. 
%
%Therefore $(\ex.\ppo \cup \ex.\fence \cup\ex.\rfe \cup \ex.\fre \cup \ex.\coe)$ creates a cycle.
%
%It implies $(\ex.\fre;\ex.\ahb \cup \ex.\coe;\ex.\ahb)$ creates a cycle.
%
%It implies $(\ex.\prop \cup \ex.\prop)$ creates a cycle from the definition of $\prop$
%
%However, $\ex$ satifies (propagation) and hence a contradiction.
%
%Therefore $\ex$ is SC.

\end{proof}

We restate \cref{th:robustarmsx} and prove the same.

\robustarmsx*

\begin{proof}
%We show an execution $\ex$ of ARMv7 program $\mbbp$ which follows $\cyc$ from \cref{th:robustarmsx}
%satisfies ARM-x86 constraints.

We set the $\mo$ relation as follows:

$[\Wlab];(\co \cup \prop);[\Wlab] \cup [\dmb];\lpo;\fr^? \cup \lpo;[\dmb] \cup \fence \implies \mo$

(AirrHB)

Assume $\ex.\xhb$ is a cycle.

It implies $(\ex.\lpo \cup \ex.\lrf)^+$ is a cycle.

It implies $(\ex.\poloc \cup \ex.\fence \cup [\Wlab \setminus \codom(\rmw)];\ex.\lpo;[\Rlab \setminus \dom(\rmw)] \cup \ex.\rfe)^+$ is a cycle.

It implies $(\ex.\poloc \cup \ex.\fence \cup \ex.\rfe)^+$ is a cycle as $\Rlab \cap \dom(\rfe) = \emptyset$.

It implies a $\prop$ cycle which violates (propagation) as shown in the proof of \cref{th:robustarmssc}.

Therefore a contradiction and $\ex$ satisfies (AirrHB).

\medskip

(AirrMOHB)

Assume $\ex.\mo;\ex.\xhb$ is a cycle.

We know $\ex.\xhb \implies \ex.\prop$ from earlier proofs.

It implies $[\Wlab \cup \dmbfull];\ex.\mo;[\Wlab \cup \dmbfull];\ex.\prop$ is a cycle.
 

We know $[\Wlab];(\co \cup \prop);[\Wlab] \cup [\dmb];\lpo;\fr^? \cup \lpo;[\dmb] \cup \fence \implies \mo$

Therefore $[\Wlab];(\co \cup \prop);[\Wlab];\ex.\prop$ is a cycle.

However, it violates (propagation) and therefore a contradiction.


It implies $\ex.\mo;(\ex.\lpo \cup \ex.\lrf)^+$ is a cycle.

%It implies $\ex.\mo;((\ex.\poloc;[\Rlab] \cup \ex.\ppo \cup \ex.\fence \cup \ex.R \cup \ex.\rfe)^+$ is a cycle 
%where $R = [\Wlab \setminus \codom(\rmw)];\lpo;[\Rlab \setminus \dom(\rmw)] \setminus \slocs$
%
%Now $\codom(\ex.\poloc;[\Rlab] \cup \ex.R) \cap \dom(\ex.\rfe) = \emptyset$.
%
%It implies $\ex.\mo;([\Rlab];\ex.\ppo;[\Wlab] \cup [\Rlab];\ex.\fence;[\Wlab] \cup \ex.\rfe)^+$ is a cycle.
%
%It implies $\ex.\mo;[\Wlab];\ex.\ahb;[\Wlab]$ is a cycle.
%
%It implies $\ex.\mo;[\Wlab];\ex.\prop;[\Wlab]$ is a cycle.
%
%It implies $\ex.\mo;\ex.\mo$ is a cycle and hence a contradiction.

Therefore $\ex$ satisfies (AirrHB).

\medskip

(AirrFRHB)

Assume $\ex.\fr;\ex.\xhb$ is a cycle.

It implies $\ex.\fre; \ex.\xhb$ cycle.

It implies $\ex.\fre;\ex.\prop$ cycle which contradicts (observation).

Therefore $\ex$ satisfies (AirrFRHB).

\medskip

(AirrFMRP)

Assume $\ex.\fr;\ex.\mo;\ex.\rfe;\ex.\lpo$ is is a cycle. 

It implies $\ex.\fr;\ex.\mo;\ex.\rfe;(\poloc \cup \fence \cup [\Wlab \setminus \codom(\rmw)];\lpo;[\Rlab \setminus \dom(\rmw)])$ is a cycle. 

It implies $\ex.\fr;\ex.\mo;\ex.\rfe;(\poloc \cup \fence)$ is a cycle. 

It implies $\ex.\fre;\ex.\mo;\ex.\rfe;(\poloc \cup \fence)$ is a cycle as $\fri \subseteq \poloc \cup \fence$.


It implies $\ex.\mo;[\Wlab];\ex.\rfe;(\ex.\poloc \cup \ex.\fence);[\Wlab]$ is a cycle.

It implies $\ex.\mo;[\Wlab];\ex.\rfe;\ex.\poloc;[\Wlab] \cup \ex.\mo;[\Wlab];\ex.\rfe;\ex.\fence;[\Wlab]$ is a cycle.

It implies $\ex.\mo;\ex.\co \cup \ex.\mo;[\Wlab];\ex.\prop;[\Wlab]$ is a cycle.

$\ex.\mo;\ex.\co \implies \ex.\co$ cycle which violates (sc-per-loc).

Considering $\ex.\mo;[\Wlab];\ex.\prop;[\Wlab]$, it implies $\ex.\mo;\ex.\mo$ is a cycle and hence a contradiction.

Therefore $\ex$ satisfies (AirrFMRP).

%\medskip
%
%\Subcase{$\ex.\fre;\ex.\mo;\ex.\rfe;\ex.\lpo$ is a cycle.}
%
%It implies $\ex.\mo;[\Wlab]\ex.\rfe;[\Rlab];(\ex.\poloc;[\Rlab] \cup \ex.\ppo \cup \ex.\fence \cup \ex.R);[\Rlab];\ex.\fre;[\Wlab]$ is a cycle. 
%
%Now $\ex.\mo;[\Wlab]\ex.\rfe;[\Rlab];\ex.\poloc;[\Rlab];\ex.\fre$ 
%
%$\implies \ex.\mo;[\Wlab]\ex.\rfe;[\Rlab];\ex.\fre$ 
%
%$\implies \ex.\mo;\ex.\co \implies \ex.\mo$
%
%Moreover $\dom(R) \cap \Rlab = \emptyset$.
% 
%It implies $\ex.\mo \cup \ex.\mo;[\Wlab]\ex.\rfe;[\Rlab];(\ex.\ppo \cup \ex.\fence);[\Rlab];\ex.\fre;[\Wlab]$ is a cycle. 
%
%$\ex.\mo$ is total and hence a contradiction.
%
%It implies $\ex.\mo;[\Wlab]\ex.\rfe;[\Rlab];(\ex.\ppo \cup \ex.\fence);[\Rlab];\ex.\fre;[\Wlab]$ is a cycle 
%
%It implies $\ex.\mo;[\Wlab];\ex.\co;[\Wlab]$ is a cycle.
%
%It implies $\ex.\mo;[\Wlab];\ex.\mo;[\Wlab]$ is a cycle and hence a contradiction.
% 
%Therefore $\ex$ satisfies (AirrFMRP).
%
\medskip

(AirrUF)

Assume $\ex.\fr;\ex.\mo;[\codom(\ex.\rmw) \cup \ex.\dmbfull];\ex.\lpo$ is a cycle.

\Subcase{$\ex.\fr;\ex.\mo;[\codom(\ex.\rmw)];\ex.\lpo$ is a cycle.}

It implies $\ex.\mo;[\Wlab];(\ex.\poloc \cup \ex.\fence \cup \ex.R);\fre^?;[\Wlab]$ is a cycle.

We know $[\Wlab];\ex.\poloc;[\Rlab];\ex.\fre \implies \ex.\co \implies \ex.\mo$ and 

$[\Wlab];\ex.R;\ex.\fre;[\Wlab] \implies [\Wlab];\ex.\lpo;\ex.\fre;[\Wlab] \implies \ex.\mo$.

It implies $\ex.\mo;[\Wlab];\ex.\fence;\fre^?;[\Wlab]$ is a cycle.

It implies $\ex.\mo;[\Wlab];\ex.\mo;[\Wlab]$ is a cycle and hence a contradiction.
 
Therefore $\ex$ satisfies (AirrUF).
\end{proof}

\paragraph{ARMv7}

We restate \cref{th:robustarmsa} and then prove the same.

\robustarmsa*

\begin{proof}
%We show an execution $\ex$ of ARMv7 program $\mbbp$ which follows $\cyc$ from \cref{th:robustarmsa}
%satisfies ARMv8 constraints.
%
%We know if $\ex$ satisfies $\set{cyc(\mbbp,\slocs)}$ then it satisfies SC and therefore ARMv8 consistent. 
%
%Suppose $\ex$ satisfies $\set{cyc(\mbbp,\slocs)}$.

We show $\ex$ is ARMv8 consistent.

(internal)

Assume a $(\ex.\poloc \cup \ex.\fr \cup \ex.\co \cup \ex.\lrf)$ cycle.

However, $\ex$ satisfies (sc-per-loc) and hence a contradiction. 

Therefore, $\ex$ satisfies (internal).

\medskip

(external)

Assume a $\ex.\ob$ cycle.

It implies $(\ex.\obs;(\ex.\aob \cup \ex.\bob \cup \ex.\dob))^+$ creates cycle.

From the definition, 

$(\ex.\aob \cup \ex.\bob \cup \ex.\dob) \subseteq \poloc \cup \fence \cup [\Wlab];\lpo$ and therefore 

$((\ex.\rfe \cup \ex.\coe \cup \ex.\fre);(\ex.\poloc \cup \fence))^+$ creates cycle.

It implies $\prop$ creates a cycle which violates (propagation).

Therefore a contradiction and $\ex$ satisfies (external).

\medskip

(atomicity)

ARMv7 execution $\ex$ satisfies (atomicity).

\medskip

Therefore $\ex$ has only ARMv8 execution.

\end{proof}

We restate \cref{th:robustarmssmca} and then prove the same.

\robustarmssmca*

\begin{proof}

%We show an execution $\ex$ of ARMv7 program $\mbbp$ which follows $\cyc$ from \cref{th:robustarmssmca}
%satisfies ARMv7-mca constraints.

We show that $\ex$ satisfies (mca).

Assume $\ex$ violates (mca) and therefore a $\wo^+$ cycle.

It implies a $(\ex.\rfe;[\Rlab];\ex.\ppo;[\Rlab];\ex.\fre)^+$ cycle.

However, $[\Rlab];\ex.\ppo;[\Rlab] \subseteq \poloc \cup \fence$.

$[\Rlab];\ex.\ppo;[\Rlab] \subseteq \poloc$ violates (sc-per-loc) and therefore a contradiction.

Otherwise it implies a $(\ex.\rfe;[\Rlab];\ex.\fence;[\Rlab];\ex.\fre)^+$ cycle. 

It implies a $\ex.\prop$ cycle which violates (propagation) 

Therefore a contradiction and hence $\ex$ is ARMv7-mca consistent.
\end{proof}

==> app-experiment.tex <==
% !TEX root = paper.tex


\section{Additional Results from Experiments}
\label{app:experiment}

\begin{figure}
\begin{tabular}{|c|c|c|c|}
\hline
Programs         & \begin{tabular}[c]{@{}c@{}}x86\\ Ld,St,U,F\end{tabular} & \begin{tabular}[c]{@{}c@{}}ARMv8\\ Ld,St,SC,DMBLD,DMBST,DMBFULL\end{tabular} & \begin{tabular}[c]{@{}c@{}}ARMv7\\ Ld,St,SC,DMB\end{tabular} \\ \hline
barrier          & 5,3,4,0                                                   & 5,3,4,0,0,0                                                        & 5,3,4,10                                                     \\ \hline
dekker-tso       & 10,10,0,4                                                 & 10,10,0,0,0,4                                                      & 10,10,0,8                                                    \\ \hline
dekker-sc        & 10,10,0,0                                                 & 10,10,0,0,0,0                                                      & 10,10,0,4                                                    \\ \hline
peterson-ra      & 4,8,0,4                                                   & 4,8,0,0,0,4                                                        & 4,8,0,4                                                      \\ \hline
peterson-tso     & 4,8,0,2                                                   & 4,8,0,0,0,2                                                        & 4,8,0,2                                                      \\ \hline
peterson-sc      & 4,8,0,0                                                   & 4,8,0,0,0,0                                                        & 4,8,0,0                                                      \\ \hline
lamport-ra       & 11,8,0,4                                                  & 10,8,0,0,0,4                                                       & 11,8,0,13                                                    \\ \hline
lamport-tso      & 9,8,0,2                                                   & 8,8,0,0,0,2                                                        & 9,8,0,9                                                      \\ \hline
lamport-sc       & 9,8,0,0                                                   & 8,8,0,0,0,0                                                        & 9,8,0,7                                                      \\ \hline
spinlock         & 4,4,4,0                                                   & 2,4,4,0,0,0                                                        & 4,4,4,12                                                     \\ \hline
spinlock4        & 8,8,8,0                                                   & 4,8,8,0,0,0                                                        & 8,8,8,24                                                     \\ \hline
ticketlock       & 6,4,2,0                                                   & 4,4,2,0,0,0                                                        & 6,4,2,8                                                      \\ \hline
ticketlock4      & 12,8,4,0                                                  & 8,8,4,0,0,0                                                        & 12,8,4,16                                                    \\ \hline
seqlock          & 8,2,4,0                                                   & 8,2,4,0,0,0                                                        & 8,2,4,8                                                      \\ \hline
nbw              & 9,6,5,0                                                   & 7,7,4,0,0,0                                                        & 9,7,4,7                                                      \\ \hline
rcu              & 16,11,0,0                                                 & 14,11,0,0,0,0                                                      & 16,11,0,10                                                   \\ \hline
rcu-offline      & 18,12,5,4                                                 & 16,15,2,0,0,4                                                      & 19,15,2,19                                                   \\ \hline
cilk-tso         & 7,4,11,2                                                  & 13,11,4,0,0,2                                                      & 14,11,4,10                                                   \\ \hline
cilk-sc          & 7,4,11,0                                                  & 13,11,4,0,0,0                                                      & 14,11,4,8                                                    \\ \hline
chase-lev-dq-ra  & 6,3,2,3                                                   & 6,3,2,0,0,3                                                        & 6,3,2,5                                                      \\ \hline
chase-lev-dq-tso & 6,3,2,1                                                   & 6,3,2,0,0,1                                                        & 6,3,2,3                                                      \\ \hline
chase-lev-dq-sc  & 6,3,2,0                                                   & 6,3,2,0,0,0                                                        & 6,3,2,2                                                      \\ \hline
\end{tabular}
\caption{memory accesses and fences of original programs.}
\label{fig:app:rmemacc}
\end{figure}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{x86 Prog.} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Naive \\ scheme\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Robustness \\ enforcement\end{tabular}}     \\ \cline{3-5} 
                          &                                                                          & \multicolumn{1}{l|}{inserted} & \multicolumn{1}{l|}{existing} & \multicolumn{1}{l|}{total} \\ \hline
Barrier                   & 8                                                                        & 1                             & 0                             & 1                          \\ \hline
Dekker-tso                & 16                                                                       & 0                             & 4                             & 4                          \\ \hline
Dekker-sc                 & 20                                                                       & 8                             & 0                             & 8                          \\ \hline
Peterson-ra               & 8                                                                        & 0                             & 4                             & 4                          \\ \hline
Peterson-ra-Bartosz       & 10                                                                       & 2                             & 0                             & 2                          \\ \hline
Peterson-ra-Dmitriy       & 10                                                                       & 0                             & 0                             & 0                          \\ \hline
Peterson-tso              & 10                                                                       & 0                             & 2                             & 2                          \\ \hline
Peterson-sc               & 12                                                                       & 4                             & 0                             & 4                          \\ \hline
Lamport-ra                & 15                                                                       & 8                             & 4                             & 12                         \\ \hline
Lamport-tso               & 17                                                                       & 6                             & 2                             & 8                          \\ \hline
Lamport-sc                & 17                                                                       & 8                             & 0                             & 8                          \\ \hline
Spinlock                  & 8                                                                        & 0                             & 0                             & 0                          \\ \hline
Spinlock4                 & 16                                                                       & 0                             & 0                             & 0                          \\ \hline
Ticketlock                & 10                                                                       & 0                             & 0                             & 0                          \\ \hline
Ticketlock4               & 20                                                                       & 0                             & 0                             & 0                          \\ \hline
Seqlock                   & 10                                                                       & 0                             & 0                             & 0                          \\ \hline
nbw                       & 15                                                                       & 0                             & 0                             & 0                          \\ \hline
rcu                       & 27                                                                       & 10                            & 0                             & 10                         \\ \hline
rcu-offline               & 30                                                                       & 8                             & 4                             & 12                         \\ \hline
cilk-tso                  & 9                                                                        & 0                             & 2                             & 2                          \\ \hline
cilk-sc                   & 11                                                                       & 0                             & 0                             & 0                          \\ \hline
Chase-lev-dq-ra           & 9                                                                        & 0                             & 3                             & 3                          \\ \hline
Chase-lev-dq-tso          & 11                                                                       & 0                             & 1                             & 1                          \\ \hline
Chase-lev-dq-sc           & 11                                                                       & 1                             & 0                             & 1                          \\ \hline
\end{tabular}
\caption{\#fences to enforce SC by naive scheme vs proposed robustness approach in x86.}
\label{app:tab:scx}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{ARMv8 Prog.} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Naive \\ scheme\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}SC-Robustness \\ enforcement \\ inserted\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}x86-Robustness \\ enforcement \\ inserted\end{tabular}} \\
                             &                                                                          &                                                                                                   &                                                                                                    \\ \hline
Barrier                      & 12                                                                       & 6                                                                                                 & 5                                                                                                  \\ \hline
Dekker-tso                   & 16                                                                       & 6                                                                                                 & 6                                                                                                  \\ \hline
Dekker-sc                    & 20                                                                       & 12                                                                                                & 9                                                                                                  \\ \hline
Peterson-ra                  & 8                                                                        & 7                                                                                                 & 7                                                                                                  \\ \hline
Peterson-ra-Bartosz          & 12                                                                       & 2                                                                                                 & 2                                                                                                  \\ \hline
Peterson-ra-Dmitriy          & 12                                                                       & 8                                                                                                 & 8                                                                                                  \\ \hline
Peterson-tso                 & 10                                                                       & 9                                                                                                 & 9                                                                                                  \\ \hline
Peterson-sc                  & 12                                                                       & 11                                                                                                & 11                                                                                                 \\ \hline
Lamport-ra                   & 14                                                                       & 8                                                                                                 & 4                                                                                                  \\ \hline
Lamport-tso                  & 16                                                                       & 11                                                                                                & 10                                                                                                 \\ \hline
Lamport-sc                   & 16                                                                       & 14                                                                                                & 13                                                                                                 \\ \hline
Spinlock                     & 10                                                                       & 0                                                                                                 & 0                                                                                                  \\ \hline
Spinlock4                    & 20                                                                       & 0                                                                                                 & 0                                                                                                  \\ \hline
Ticketlock                   & 10                                                                       & 0                                                                                                 & 0                                                                                                  \\ \hline
Ticketlock4                  & 20                                                                       & 0                                                                                                 & 0                                                                                                  \\ \hline
Seqlock                      & 14                                                                       & 0                                                                                                 & 0                                                                                                  \\ \hline
nbw                          & 18                                                                       & 12                                                                                                & 12                                                                                                 \\ \hline
rcu                          & 25                                                                       & 16                                                                                                & 12                                                                                                 \\ \hline
rcu-offline                  & 33                                                                       & 27                                                                                                & 25                                                                                                 \\ \hline
cilk-tso                     & 26                                                                       & 8                                                                                                 & 8                                                                                                  \\ \hline
cilk-sc                      & 28                                                                       & 9                                                                                                 & 9                                                                                                  \\ \hline
Chase-lev-dq-ra              & 11                                                                       & 3                                                                                                 & 3                                                                                                  \\ \hline
Chase-lev-dq-tso             & 11                                                                       & 5                                                                                                 & 5                                                                                                  \\ \hline
Chase-lev-dq-sc              & 11                                                                       & 6                                                                                                 & 6                                                                                                  \\ \hline
\end{tabular}
\caption{\#fences to enforce SC and x86 inserted by naive scheme vs proposed robustness approach in ARMv8.}
\label{app:tab:scx}
\end{table}

==> app-overview.tex <==
% !TEX root = paper.tex

%\section{Examples from Overview}
%\label{app:overview}



%\begin{center}
%\begin{minipage}{0.35\textwidth}
%\[
%\inparII{
%\irmw(X,0,1);
%\\ a= Y;
%}{
%\irmw(X,0,1);
%\\ b = X; 
%}
%\]
%\end{minipage}
%\hfill\vline\hfill
%\begin{minipage}{0.28\textwidth}
%\centering
%\begin{tikzpicture}[yscale=0.8]
%  \node (t11) at (-1,0)  {$\Ulab(X,0,1)$};
%  \node (t12) at (-1,-2.5) {$\Rlab(Y,0)$};
%%
%  \node (t21) at (1,0) {$\Ulab(Y,0,1)$};
%  \node (t22) at (1,-2.5) {$\Rlab(X,0)$};
%%
%  \draw[po] (t11) to (t12);
%  \draw[po] (t21) to (t22);
%%
%  \draw[fr] (t12) to node[below]{$\fre$} (t21);
%  \draw[fr] (t22) to (t11);
%\end{tikzpicture}
%\end{minipage}
%\hfill\vline\hfill
%\begin{minipage}{0.32\textwidth}
%\centering
%\begin{tikzpicture}[yscale=0.8]
%  \node (t11) at (-1.2,0)  {$\Rlab(X,0)$};
%  \node (t12) at (-1.2,-1) {$\Wlab(X,1)$};
%  \node (t13) at (-1.2,-2)  {$\dmbfull$};
%  \node (t14) at (-1.2,-3)  {$\Rlab(Y,1)$};
%%
%  \node (t21) at (1.2,0)  {$\Rlab(Y,0)$};
%  \node (t22) at (1.2,-1) {$\Wlab(Y,1)$};
%  \node (t23) at (1.2,-2)  {$\dmbfull$};
%  \node (t24) at (1.2,-3)  {$\Rlab(X,0)$};
%%
%  \draw[po] (t11) to node[right]{$\rmw$} (t12);
%  \draw[po] (t12) to  (t13);  
%  \draw[po] (t13) to (t14);  
%  \draw[po] (-1.2,0.5) to (t11);  
%%
%  \draw[po] (t21) to node[left]{$\rmw$} (t22);
%  \draw[po] (t22) to (t23);  
%  \draw[po] (t23) to node[left]{$\rmw$} (t24);  
%  \draw[po] (1.2,0.5) to (t21);  
%%
%  \draw[fr] (t14) to node[below]{$\fre$} (t22);
%  \draw[fr] (t24) to  (t12);
%\end{tikzpicture}
%\end{minipage}
%\end{center}
%

%\subsubsection{Tradeoff in $\cmm \mapsto \xarch \mapsto \arma$}
%\label{app:cxarmtradeoff}
%
%The $\cmm \mapsto \xarch \mapsto \arma$ scheme also differs from $\xarch \mapsto \arma$ for mapping $\movst_\MOat$ accesses. 
%The scheme introduces a leading $\idmbfull$ fence instead of $\idmbst$ to preserve correctness. 
%Consider the example below 
%%in \cref{fig:cxarmdmb} 
%where 
%a C11 to x86 to ARMv8 translation is performed. 
%\[
%\inparII{
%a = X_\MOna; %\codecomment{2}
%\\ Y_\MOna = 1;
%\\ Z_\MOrel = 1;
%}{
%r = Z_\MOacq; %\codecomment{1}
%\\ \Cif{r==1} \{
%\\ \quad X_\MOna = 2;
%\\ \quad Y_\MOna = 2;
%\\ \quad c = Y_\MOna; %\codecomment{1}
%\\ \}
%}
%\quad \mapsto \quad
%\inparII{
%a = X_\MOna; %\codecomment{2}
%\\ Y_\MOna = 1;
%\\ Z_\MOat = 1;
%}{
%r = Z_\MOat; %\codecomment{1}
%\\ \Cif{r==1} \{
%\\ \quad X_\MOna = 2;
%\\ \quad Y_\MOna = 2;
%\\ \quad c = Y_\MOna; %\codecomment{1}
%\\ \}
%}
%\quad \mapsto \quad
%\inparII{
%a = X; %\codecomment{2}
%\\ Y = 1;
%\\ \idmbfull
%\\ Z = 1;
%}{
%r = Z; %\codecomment{1}
%\\ \idmbld
%\\ \Cif{r==1} \{
%\\ \quad X = 2;
%\\ \quad Y=2;
%\\ \quad c = Y; %\codecomment{1} 
%\\ \}
%}
%\] 
%The C11 program is data race free as it is well-synchronized 
%by release-acquire accesses on $Z$ and 
%the outcome $a=2,r=1,c=1$ is disallowed in the program. 
%The generated ARMv8 program disallows the outcome, however, 
%without the $\idmbfull$ in the first thread the outcome would be possible. 
%It is because a $\idmbld$ or $\idmbfull$ fence is required to 
%preserve $\bob$ relation between 
%$\Rlab(X,2)$ and $\Wlab(Z,1)$ events.
%However, a $\idmbld$ is not sufficient to establish $\bob$ relation between 
%$\Wlab(Y,1)$ and $\Wlab(Z,1)$ and for that we require a $\idmbst$ or $\idmbfull$ fence. 
%Therefore we require a leading $\idmbfull$ or a leading pair of $\dmbld$ and $\dmbst$ fences or a $\dmbfull$ fence for a $\movst_\MOat$ mapping. 
% 
%As a result there is a tradeoff between the mapping schemes in \cref{tab:xarm} and \cref{tab:cxarm}. 
%While \cref{tab:cxarm} provides more efficient mapping for $\movld_\MOna$ and $\movst_\MOna$ 
%accesses, scheme in \cref{tab:cxarm} incurs more cost for $\movst_\MOat$ 
%as it introduces a leading $\idmbfull$ instead of a $\idmbst$ fence. 
%After the mapping we may weaken a $\idmbfull$ fence whenever appropriate.  


==> compositional.tex <==
% !TEX root = paper.tex

\section{Compositional Analysis Based Fence Elimination}
\label{sec:compositional}

In this section we identify the possible memory access pairs from each thread 
and then compose their possible effects on program execution. 
We have already discussed such an example in \cref{idea}. 
\TODO{discuss example in idea section}
Now we define the correctness theorems and 
propose the compositional analysis techniques. 

We first define $\pairs$ and $\cyc$; for a given program $\mbbp$, $\pairs(\mbbp,R)$ returns the set of same-thread 
event pairs in $\mbbp$ with relation $R$. 
\begin{definition}
$\pairs(\mbbp) \triangleq \set{(a,b) \mid \exists i.~a \cdot \tau \cdot b \in \mbbp(i)}$
\end{definition}

$\cyc(\mbbp,R)$ is the set of event pairs which follow certain conditions as defined below. 
\begin{definition}
\begin{align*}
\cyc(\mbbp) \triangleq & \set{(a,b) \mid (a,b) \in \pairs(\mbbp) \land \exists (p,q),( r,s) \in \pairs(\mbbp).~(a,b) \neq (p,q) \land (a,b) \neq (r,s) 
\\ & \land b.\lloc = p.\lloc \land a.\lloc = s.\lloc \land (b,p), (s,a) \notin (\Rlab \times \Rlab)}
\end{align*}
\label{def:cyc}
\end{definition}

%Next we define $\ncyc(\mbbp)$ to check if there exists at least one access pair on $\cyc(\mbbp)$ where the accesses are on different locations.
%\begin{definition}
%\begin{align*}
%\ncyc(\mbbp) \triangleq \true \text{ if } \exists (a,b) \in \cyc(\mbbp).~a.\lloc \neq b.\lloc
%\end{align*}
%\label{def:slcyc}
%\end{definition}

Given a program $\cyc$ overapproximates the event pairs 
for an execution in a memory model such that 
$\lpo \cup \rfe \cup \coe \cup \fre$ cycle is allowed 
but any $R \cup \rfe \cup \coe \cup \fre$ cycle is disallowed.   

Therefore if an event pair is not in $\cyc$ then the event pair does 
not appear on any cycle in any execution. 
As a result the consistency conditions of the execution are not affected by the 
ordering of such an event pair and therefore any fence 
between such an event pair is redundant. 
Therefore it is safe to remove fences between such event pairs even if the event pair is unordered. 

We state such safe transformations for x86, ARMv8, and ARMv7/ARMv7-mca programs in \cref{th:xcycfenceelim,th:armv8cycfenceelim,th:armv7cycfenceelim}. 
The detailed proofs are in \cref{app:compositional}.

\begin{restatable}{theorem}{xcycfenceelim}
\label{th:xcycfenceelim}
Let $\srcp$ be an x86 program and $\tgtp$ is the program after eliminating an $\mfence$ from thread $i$ i.e. 
$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \F \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
The transformation is safe when $(a,b) \notin \cyc(\srcp)$.
\end{restatable}

\begin{restatable}{theorem}{armvacycfenceelim}
\label{th:armv8cycfenceelim}
Let $\srcp$ be an ARMv8 program and $\tgtp$ is the program after eliminating a fence from thread $i$ i.e. 
$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot c \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$ where $c = \dmbfull \lor \dmbld \lor \dmbst$. 
The transformation is safe when $(a,b) \notin \cyc(\srcp)$.
\end{restatable}

\begin{restatable}{theorem}{armvscycfenceelim}
\label{th:armv7cycfenceelim}
Let $\srcp$ be an ARMv7 or ARMv7-mca program and $\tgtp$ is the program after eliminating a $\dmb$ fence from thread $i$ i.e. 
$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \dmb \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
The transformation is safe when $(a,b) \notin \cyc(\srcp)$.
\end{restatable}
Based on these theorems we develop fence elimination algorithms for x86, ARMv8, and ARMv7 in \cref{fig:ncycfelim}.
\begin{figure}[t]
\begin{subfigure}{0.45\textwidth}
\begin{algorithmic}[1]
%\Procedure{$\mathsf{getpairs}$}{$M,\mathsf{pairs}$}
%\For{$\iteri, \iterj \in M$}
%\If{$\iteri.\locs \ !\!= \ \iterj.\locs$}
%\State $\mathsf{pairs} \leftarrow \mathsf{pairs} \cup \set{(\iteri,\iterj)}$ 
%\EndIf
%\EndFor
%\EndProcedure
%\Procedure{$\mathsf{getcyc}$}{$\mathsf{pairs},\cyc$}
%\For{$(a,b), (p,q) \in \mathsf{pairs}$}
%\If{$(a,b) == \ (p,q)$}
%\State continue
%\EndIf
%\For{$(r,s) \in \mathsf{pairs}$}
%\If{$(a,b) == \ (r,s)$}
%\State continue
%\EndIf
%\If{$b.\locs \ !\!= p.\locs$}
%\State continue
%\EndIf
%\If{$a.\locs \ !\!= s.\locs$}
%\State continue
%\EndIf
%\State $\mathsf{cyc} \leftarrow \mathsf{cyc} \cup \set{(a,b)}$ 
%\EndFor
%\EndFor
%\EndProcedure
\Procedure{$\mathsf{getcycfs}$}{$\cyc,\fs,\mathsf{cycfs}$}
\For{$\mathsf{c} \in \cyc$}
\For{$\fnc \in \fs$}
\State a = c.first
\State b = c.second
\If{$\opath(a,\fnc,b)$}
\State $\mathsf{cycfs} \leftarrow \mathsf{cycfs} \cup \fnc$ 
\EndIf
\EndFor
\EndFor
\EndProcedure
\end{algorithmic}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\begin{algorithmic}[1]
\Procedure{x86ncycFelim}{$P$}
\State $\textsc{ncycFelim}(P,\mfence)$
\EndProcedure
\Procedure{ARMv8ncycFelim}{$P$}
\State $\textsc{ncycFelim}(P,\dmbfull)$
\State $\textsc{ncycFelim}(P,\dmbst)$
\State $\textsc{ncycFelim}(P,\dmbld)$
\EndProcedure
\Procedure{ARMv7ncycFelim}{$P$}
\State $\textsc{ncycFelim}(P,\dmb)$
\EndProcedure
\end{algorithmic}
\end{subfigure}
\begin{subfigure}{0.95\textwidth}
\begin{algorithmic}[1]
\Procedure{ncycFelim}{$P, \Flab$}
\For{$i \in \mathbb{N}$}
\State $\getmemaccs(P(i),\maccs_i)$ \Comment{enlist shared memory accesses for $\mathbb{N}$ concurrent threads}
\State $\mathsf{getpairs}(\maccs_i,\mathsf{pairs})$ \Comment{enlist access pairs for each thread}
\EndFor
\State $\mathsf{getcyc}(\mathsf{pairs},\cyc)$ \Comment{identify pairs on cycle}
\State $\getfences(P,\Flab,\fs)$  \Comment{enlist fences with label $\Flab$}
\State $\mathsf{getcycfs}(\cyc,\fs,\mathsf{cycfs})$ \Comment{enlist fences in the cycles}
\State $\oelim(\fs,\mathsf{cycfs})$ \Comment{eliminate non-cycle fences}
\EndProcedure
\end{algorithmic}
\end{subfigure}
\caption{Non-cycle Fence Elimination in all (x86, ARMv8, ARMv7/ARMv7-mca) architectures.}
\label{fig:ncycfelim}
\end{figure}
In \cref{fig:ncycfelim} each architecture calls $\textsc{ncycFelim}$ procedure with 
respective fence labels.
$\textsc{ncycFelim}$ identifies memory accesses in each functions which may run in parallel 
and computes the possible set of pairs of memory accesses in $\pairs$. 
Then $\mathsf{getcyc}$ procedure computes $\cyc$ based on \cref{def:cyc}. 
Next, we identify the fences which are intermediate to the pairs in $\cyc$ and eliminate rest of the fences in 
$\oelim$ procedure.
%%%%%%%%%%%%%%%%%%%%%%%
%
%Suppose a program has 
%For example, consider an x86 program with two functions $$ where each function 
%creates respective threads which may run in parallel. 
%
%
% which 
%
%
%whose access sequence in the first thread 
%may create a pair of events 
%
%
%execution $\ex$ such that a thread has four events $a$, $b$ , $c$, and $d$  
%such that: 
%\begin{itemize}
%\item $a=\Wlab(X, \_)$, $b=\Rlab(Y,\_)$, $a.\tid=b.\tid$, and $\ex.\lpo(a,b)$ 
%\item $a=\Wlab(Y, \_)$, $b=\Rlab(X,\_)$, $c.\tid=d.\tid$, and $\ex.\lpo(c,d)$
%\item $a$ and $b$ run in parallel with $c$ and $d$
%\end{itemize}
%In this case it is possible to come up with a
%
% 
%Following the axiomatic model Given an execution for a given program we check 
%the consistency by certain 
%
%
%More specifically we check if the access sequences which may run in parallel 
%may result in certain events in an execution so that the relations among them 
%  





\subsection{Robustness Analysis}
\label{sec:robustness}

A program $\mbbp$ is M-robust against K when all $M$ 
consistent executions of $\mbbp$ is also K-consistent.

If $M$ and $K$ are defined on same set of accesses then 
we check if an $M$-consistent execution also satisfies the 
consistency conditions of memory model $K$. 
However, if the accesses are different then we map a program 
$\srcp$ to $\tgtp$ and check whether for each $M$ consistent 
execution of $\srcp$ there exists a corresponding 
$K$ consistent execution of $\tgtp$.    

Note that for any program respective mapping schemes 
ensure robustness by introducing additional fences 
along with memory accesses. 
In this section we will consider mappings where we do not introduce 
addtional fence along with memory accesses during mapping. 

\paragraph{Approach} We apply compositional analysis to check robustness properties 
statically for a program for different architectural models. 
Note that in this analysis we compose the memory access pairs from possible 
different thread functions. 
However, we do not assume the number of threads created during an 
execution from each thread function.  
Therefore we provide a stronger guarantee; rather than one program 
our analysis guarantees robustness for a class of programs 
which uses same set of thread functions.

In this analysis we extend $\cyc$ to $\rcyc$ for relation $R$; 
we compute $\rcyc(\mbbp, R)$ where the memory access pairs are in relation $R$. 

\begin{definition}
$\ex.\epo = \ex.\lpo \cap \codom(\ex.\rfe \cup \ex.\coe \cup \ex.fre) \times \dom(\ex.\rfe \cup \ex.\coe \cup \ex.\fre)$ 
\label{def:epo}
\end{definition}


\begin{definition}
\begin{align*}
\rcyc(\mbbp,R) \triangleq & \set{(a,b) \mid (a,b) \in \pairs(\mbbp) \cap R \land \exists (p,q),( r,s) \in \pairs \cap R.~(a,b) \neq (p,q) \land (a,b) \neq (r,s) 
\\ & \land b.\lloc = p.\lloc \land a.\lloc = s.\lloc}
\end{align*}
\label{def:rcyc}
\end{definition}


\begin{definition}
$\pairs(\mbbp,i) \triangleq \set{(a,b) \mid a \cdot \tau \cdot b \in \mbbp(i)}$
\end{definition}

\begin{definition}
%$Re(a) \triangleq \exists j,p.~j \neq a.\tid \land p \in \mbbp(j). \land one(p,a) = \WUlab \land one(p,a) = \RUlab \land a.\lloc = p.\lloc$
% NOTE. We have to take R-->R cases also for non-MCA pattern.
$Re(a) \triangleq \exists j,p.~j \neq a.\tid \land p \in \mbbp(j). \land a.\lloc = p.\lloc \land (a \in \RUlab \implies \WUlab_{a.\lloc} \neq \emptyset) \land (a \in \WUlab \implies \RUlab_{a.\lloc} \neq \emptyset)$
\end{definition}


\begin{definition}
$\cyc(\mbbp,i) \triangleq \set{(a,b) \mid (a,b) \in \pairs(\mbbp,i) \land \exists j,k.~j \neq i \land k \neq i \land Re(a) \land Re(b)}$ 
\end{definition}

\begin{definition}
$\robust(\mbbp,R) \triangleq \forall i.~\cyc(\mbbp,i) \subseteq R$.
\end{definition}

\begin{definition}
An x86 program is x86-robust against SC if $\robust(\mbbp,R)$ holds where $R=...$.
\end{definition}


%\begin{definition}
%$\rcyc(\mbbp,i,R) \triangleq \forall (a,b) \in \pairs(\mbbp,i).~\exists j,k.~j \neq i \land k \neq i \land Re(a) \land Re(b) \implies R(a,b)$ 
%\end{definition}
 
%\begin{table}
%\begin{tabular}{c|c}
%x86 & ARMv8    \\
%\hline
%$\mov(\Rlab)$ & $\ldr$ \\
%$\mov(\Wlab)$ & $\ldr$ \\
%$\mathsf{lock \ cmpxchg}$ & $\ollsc$ \\
%$\mfence$ & $\dmbfull$   \\
%\end{tabular}
%\caption{Static Robustness of x86 to ARMv8 Mappings.}
%\label{tab:robustness-armx}
%\end{table}
%
%\begin{table}
%\begin{tabular}{c|c}
%ARMv8 & ARMv7    \\
%\hline
%$\ldr/\ldar$ & $\ldr$ \\
%$\str/\stlr$ & $\str$ \\
%$\ollsc$ & $\ollsc$ \\
%$\dmbfull$ & $\dmb$   \\
%$\dmbld$ & $\dmb$ \\
%$\dmbst$ & $\dmb$ \\
%$\isb$ & $\isync$
%\end{tabular}
%\caption{Static Robustness of ARMv8 to ARMv7 Mappings.}
%\label{tab:robustness-arm87}
%\end{table}
%
%More specifically we check if a program is:
%\begin{itemize}
%\item ARMv8 robust against SC and x86.
%\item ARMv7 robust against SC, x86, ARMv8, and ARMv7-mca.
%\item ARMv7-mca robust against SC, x86, and ARMv8.
%\end{itemize}

\subsection{x86}

%\begin{theorem}
%For a given program $\srcp$, mappings in \cref{tab:robustness-armx} is robust (has only x86 behaviors) if $\srcp$ has no $static-\ob$ cycle with $\Wlab \times \Wlab \cup \Rlab \times \Rlab \cup \Rlab \times \Wlab$ pairs.
%\end{theorem}

Now we check robustness of x86 programs against SC. 
An x86 program is robust against SC when the program has only 
SC behaviors, that is, interleaving executions. 
We define the required condition in the following \cref{th:xsc}.

\begin{restatable}{theorem}{xsc}
\label{th:xsc}
An x86 program $\mbbp$ is x86-robust against SC if $\robust(\mbbp,R)$ holds where $R = [\RUlab];\lpo \cup \lpo;[\WUlab] \cup \slocs \cup \cup \lpo;[\Flab];\lpo$ i.e. for all x86 consistent execution $\ex$, $\ex.\epo \subseteq \ex.R$ holds.
\end{restatable}

%Next, instead of enumerating all executions of program $\mbbp$ 
%we lift the notion to the thread semantics and perform a 
%conservative analysis of program robustness using the 
%following theorem \cref{th:pxsc}.
%
%\begin{restatable}{theorem}{pxsc}
%\label{th:pxsc} 
%An x86 program $\mbbp$ is x86-robust against SC if $\robust(\mbbp,R)$ holds
%%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp, R)$ 
%where $R = [\RUlab];\lpo \cup \lpo;[\WUlab] \cup \slocs \cup \cup \lpo;[\Flab];\lpo$.
%%$R= (\RWUlab \times \RWUlab) \setminus ([\Wlab];\lpo;[\Rlab] \setminus (\slocs \cup \lpo;[\Flab];\lpo))$.
%%%
%%%there exists no $\cyc(\mbbp, (\Wlab \times \Rlab) \setminus \slocs)$.
%\end{restatable}
%
%\begin{proof}
%For all consistent execution $\ex \in \denot{\mbbp}_{x86}$ 
%$\ex$ satifies SC. 
%Also from definition $\forall \ex \in \denot{\mbbp}_{x86}~R \implies \ex.\epo$. 
%Therefore we check a stricter condition under thread semantics and 
%as a result the program is x86 robust against SC.
%\end{proof}


\subsection{ARMv8}

%\begin{theorem}
%For a given program $\srcp$, mappings in \cref{tab:robustness-arm87} is robust if $\srcp$ has no $static-\wb$ cycle with $\Rlab \times \Rlab$ pairs where there exists set of $\Wlab$ with same locations.
%\end{theorem}

\begin{restatable}{theorem}{armasc}
\label{th:armasc}
An ARMv8 program $\mbbp$ is ARMv8-robust against SC if $\robust(\mbbp, R)$ hold where 
$R= \poloc \cup (\aob \cup \dob \cup \bob)^+$  i.e. for all x86 consistent execution $\ex$, $\ex.\epo \subseteq \ex.R$. 
\end{restatable}

%
%
%\begin{restatable}{theorem}{parmasc}
%\label{th:parmasc}
%An ARMv8 program $\mbbp$ is ARMv8-robust against SC if $\robust(\mbbp,\slocs)$ or $\robust(\mbbp, R)$ hold where 
%$R= \poloc \cup (\aob \cup \dob \cup \bob)^+$ hold.
%
%%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp,\slocs) \cup \rcyc(\mbbp, \aob \cup \bob \cup \dob)$.
%%%
%%%
%%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,\slocs) \lor c = \cyc(\mbbp, R)$ where $R = \aob \cup \bob \cup \dob$. 
%\end{restatable}
%
%\begin{proof}
%
%$\robust(\mbbp,\slocs)$ implies that a cycle may happen only by same-location events. 
%However, it would violate (sc-per-loc) in an execution. 
%Therefore no consistent execution would have such a cycle and all consistent execution 
%are SC consistent.
%Moreover, following \cref{tharmsc}, $\robust(\mbbp, (\ex.\aob \cup \ex.\dob \cup \ex.\bob)^+)$ satisfies SC robustness.
%\end{proof}

We define x86A; x86 constraints for ARMv8 consistent execution $\ex$.
\begin{itemize}
\item $\ex.\xhb$ is irreflexive. \hfill (AirrHB)
\item $\ex.\mo;\ex.\xhb$ is irreflexive. \hfill (AirrMOHB)
\item $\ex.\fr;\ex.\xhb$ is irreflexive. \hfill (AirrFRHB)
%\item $\ex.\fr;\ex.\mo$ is irreflexive. \hfill (AirrFRMO)
\item $\ex.\fr;\ex.\mo;\ex.\rfe;\ex.\lpo$ is irreflexive  \hfill (AirrFMRP)
\item $\ex.\fr;\ex.\mo;[\codom(\ex.\rmw) \cup \ex.\dmbfull];\ex.\lpo$ is irreflexive. \hfill (AirrUF)
%\item $[\ex.\rmw] \cap \ex.\fre;\ex.\coe = \emptyset$ is irreflexive. \hfill (ARMW)
\end{itemize}

We define $\ex.\mo$ such that   

\begin{itemize}

\item $[\ex.\Wlab \cup \ex.\dmbfull];\ex.\ob;[\ex.\Wlab \cup \ex.\dmbfull] \implies \ex.\mo$

\item $[\ex.\Wlab \cup \ex.\dmbfull];\ex.\lpo;[\ex.\Wlab \cup \ex.\dmbfull] \implies \ex.\mo$

\item $ [\ex.\dmbfull];\ex.\lpo;\ex.\fr \implies \ex.\mo$

\item $\ex.\co \implies \rloc {\ex.\mo}$

\end{itemize}


\begin{restatable}{theorem}{xA}
\label{th:x86A}
x86 and x86A are equivalent.
\end{restatable}

We define relation $\xwr$ as follows 
\[
\inarr{
\xwr= [\Wlab \cup \Llab \setminus \codom(\rmw)];\lpo;[\Rlab \cup \Alab \setminus \dom(\rmw)] \setminus (\slocs \cup (\Llab \times \Alab))
}
\]

\begin{restatable}{theorem}{robustarmax}
\label{th:robustarmax}
An ARMv8 program $\mbbp$ is ARMv8-robust against x86 if $\robust(\mbbp, R)$ holds where $R=\poloc \cup \xwr \cup (\aob \cup \bob \cup \dob)^+$   i.e. for all x86 consistent execution $\ex$, $\ex.\epo \subseteq \ex.R$ holds. 
\end{restatable}

%
%\begin{restatable}{theorem}{probustarmax}
%\label{th:probustarmax}
%An ARMv8 program $\mbbp$ is ARMv8-robust against x86 if $\robust(\mbbp, R)$ holds where $R=\poloc \cup \xwr \cup (\aob \cup \bob \cup \dob)^+$. 
%%%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp,\slocs) \cup \rcyc(\mbbp, R \cup \aob \cup \bob \cup \dob)$
%%
%%where $R= [\Wlab \cup \Llab \setminus \codom(\rmw)];\lpo;[\Rlab \cup \Alab \setminus \dom(\rmw)] \setminus (\slocs \cup (\Llab \times \Alab))$.
%%
%%
%%%
%%%
%%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,\slocs) \lor c = \cyc(\mbbp, R)$ where $R = \Wlab \setminus \codom(\rmw) \times \Rlab$. 
%\end{restatable}


\subsection{ARMv7}

\begin{restatable}{theorem}{robustarmssc}
\label{th:robustarmssc}
An ARMv7/ARMv7-mca program $\mbbp$ is ARMv7-robust against SC if $\robust(\mbbp,  R)$ hold where $R=\poloc \cup \fence$  i.e. for all x86 consistent execution $\ex$, $\ex.\epo \subseteq \ex.\poloc \cup \ex.\fence$ holds. 
%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp,\slocs) \cup \rcyc(\mbbp, R)$ 
%where $R =  \ppo \cup \fence$.
%%
%%
%%$\allcycle(\mbbp) \subseteq \set{\cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp, R) \mid R = \ppo \cup \fence}$.
%%
%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,\slocs) \lor c = \cyc(\mbbp, R)$ where $R = \ppo \cup \fence$. 
\end{restatable}

\begin{restatable}{theorem}{robustarmsx}
\label{th:robustarmsx}
An ARMv7/ARMv7-mca program $\mbbp$ is ARMv7-robust against x86 if $\robust(\mbbp, R)$ hold 
%
%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp,\slocs) \cup \rcyc(\mbbp, R)$ 
where $R = \poloc \cup \fence \cup [\Wlab \setminus \codom(\rmw)];\lpo;[\Rlab \setminus \dom(\rmw)]$  i.e. for all ARMv7 consistent execution $\ex$, $\ex.\epo \subseteq \ex.R$ holds.
%
%$\allcycle(\mbbp) \subseteq \set{\cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp, R) \mid R = \ppo \cup \fence \cup (\Wlab \setminus \codom(\rmw) \times \Rlab)}$.
%
%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,\slocs) \lor c = \cyc(\mbbp, R)$ where $R = \ppo \cup \fence \cup (\Wlab \setminus \codom(\rmw) \times \Rlab)$. 
\end{restatable}

\begin{restatable}{theorem}{robustarmsa}
\label{th:robustarmsa}
An ARMv7/ARMv7-mca program $\mbbp$ is ARMv7-robust against ARMv8 if $\robust(\mbbp,\slocs)$ or $\robust(\mbbp, R)$ hold where  $R= \poloc \cup [\Wlab];\lpo \cup \fence$ i.e. for all ARMv7 consistent execution $\ex$, $\ex.\epo \subseteq \ex.R$ holds.
%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp,\slocs) \cup \rcyc(\mbbp, [\Rlab];\ppo;[\Wlab] \cup \fence)$
%%$\cyc(\mbbp,[\Rlab];\ppo;[\Rlab]) \subseteq \set{\cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp,\fence)}$.
%%
%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,[\Rlab];\ppo;[\Rlab]) \implies c = \cyc(\mbbp, \slocs) \lor c = \cyc(\mbbp, \fence)$.
\end{restatable}

\begin{restatable}{theorem}{robustarmssmca}
\label{th:robustarmssmca}
An ARMv7 program $\mbbp$ is ARMv7-robust against ARMv7-mca if $\robust(\mbbp,\slocs)$ or $\robust(\mbbp, R)$ hold where $R=\poloc \cup \fence \cup [\Wlab];\lpo$ i.e. for all ARMv7 consistent execution $\ex$, $\ex.\epo \subseteq \ex.R$ holds.
%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp,\slocs) \cup \rcyc(\mbbp, [\Rlab];\ppo;[\Wlab] \cup \fence)$
%
%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,[\Rlab];\ppo;[\Rlab]) \implies c = \cyc(\mbbp, \slocs) \lor c = \cyc(\mbbp, \fence)$.
\end{restatable}

NOTE. $\data;\coi$ is not captured by $\ppo$. 
So having a $\ppo$ doe not guarantee $\dob$. 
scalar read read may have dob and ii0. 
But we keep fences in between. 
We'll use it in the analysis algorithm.

%
%\begin{theorem}
%An ARMv7-mca program $\mbbp$ is ARMv7-mca-robust against SC if 
%
%$\set{\cyc(\mbbp, \E \times \E)} \subseteq \set{ \cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp, R) \mid R =  \ppo \cup \fence}$.
%%
%%
%%$\allcycle(\mbbp) \subseteq \set{\cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp, R) \mid R = \ppo \cup \fence}$.
%%
%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,\slocs) \lor c = \cyc(\mbbp, R)$ where $R = \ppo \cup \fence$. 
%\end{theorem}
%
%\begin{theorem}
%An ARMv7-mca program $\mbbp$ is ARMv7-mca-robust against x86 if 
%
%$\set{\cyc(\mbbp, \E \times \E)} \subseteq \set{ \cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp, R) \mid R =  \ppo \cup \fence \cup (\Wlab \setminus \codom(\rmw) \times \Rlab)}$.
%%
%%$\allcycle(\mbbp) \subseteq \set{\cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp, R) \mid R = \ppo \cup \fence \cup (\Wlab \setminus \codom(\rmw) \times \Rlab)}$.
%%
%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,\slocs) \lor c = \cyc(\mbbp, R)$ where $R = \ppo \cup \fence \cup (\Wlab \setminus \codom(\rmw) \times \Rlab)$. 
%\end{theorem}
%
%\begin{theorem}
%An ARMv7-mca program $\mbbp$ is ARMv7-mca-robust against ARMv8 if 
%
%$\cyc(\mbbp,[\Rlab];\ppo;[\Rlab]) \subseteq \set{\cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp,\fence)}$.
%%
%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,[\Rlab];\ppo;[\Rlab]) \implies c = \cyc(\mbbp, \slocs) \lor c = \cyc(\mbbp, \fence)$.
%\end{theorem}

\TODO{Proofs done. Later revise.}

\TODO{Algorithm}

\subsection{Robustness Based Optimization}
If an ARMv8 program is x86 robust then we can remove a $\dmbfull$ fence between store and load. 
It keeps the ARMv8 program x86 robust.

==> contributions.tex <==
% !TEX root = main.tex

\section{Contributions}

We perform correct transformation of concurrency primitives between x86, ARMv7, ARMv7-mca, and ARMv8 architectures. 
We do so in two ways. 

\subsection{First Approach}
First, we identify correct mapping scheme between architectures. 
In these schemes a memory access in one architecture is mapped to corresponding memory 
access along with leading and/or trailing fences as required. 
We show that the resulting fences in the mapping is nessary and sufficient. 
We show examples to demonstrate why a fence is necessary in a mapping and we 
show that the fences are sufficient by proving the soundness of the mapping schemes. 
The results are as follows: 
\begin{enumerate}
\item x86 to ARMv8 (\ref{armv8tox86}) and ARMv8 to x86 (\ref{x86toarmv8})

%\item x86 to ARMv7 (\ref{armv7tox86}) and ARMv7 to x86 (\ref{x86toarmv7})

\item ARMv7 to ARMv8 (\ref{sec:armv7toarmv8}) and ARMv8 to ARMv7 (\ref{armv8toarmv7})

\item ARMv7-mca to ARMv8 (\ref{armv7mcatoarmv8}) and ARMv8 to ARMv7-mca (\ref{sec:armv8v7mca}).
\end{enumerate}
We observe that we can perform x86 $\leadsto$ ARMv8 $\leadsto$ ARMv7/ARMv7-mca mappings and 
do not require to prove x86 $\leadsto$ ARMv7/ARMv7-mca mappings directly. 

\subsubsection{Further Optimizations}
We observe that there are a number of scenarios where a program may have redundant fences. 
In this scenario we eliminate or weaken a number of fences based on static program analysis. 
We perform analysis at two levels: thread modular analysis where we analyze each thread individually. 
We also perform a compositional analysis on whole program when we have access to all the program threads. 

Based on thread modular analysis we eliminate fences in \cref{sec:felim} in x86 (\cref{sec:xfelim}) and ARMv8 (\cref{sec:armv8felim}). 
We also weaken fences in ARMv8 based on thread modular analysis in \cref{sec:armv8fweaken}. 
In \cref{sec:cafelim} we eliminate fences based on compositional analysis on whole program. 

\subsection{Second Approach}

In this approach we map the memory accesses without leading or trailing fences. 
Then we check if a fence is required to be introduced to preserve 
the mapping correctness. Otherwise the target program may exhibit certain 
weak behavior which is otherwise not present in the source program. 

To decide whether we require to introduce additional fences 
we note some observation and perform certain static program analysis. 
We observe that when an execution exihibit certain weak behavior it 
forms a cycle on memory access events. 
Thus the weak behavior requires corresponding memory access sequences 
as well in the program. 
If such memory access sequences are absent in a program then the program cannot 
exihibit corresponding weak behavior. 
We exploit this fact and introduce a notion of static robustness in \label{sec:robustness}.
analysis by which we ensure that a program cannot have a particular weak behavior. 

Note that the our static robustness analysis generalizes the robustness property 
in \citet{}. In \citet{} they check robustness of given program for a memory model $M$ against SC. 
The robustness analysis checks if the program exihibit only SC behaviors under memory model $M$. 
In our case we check robustness of a program for a memory model $M$ against memory model $K$ 
where $M$ is weaker than $K$.

Thus when a program is robust in memory model $M$ against memory model $K$, we do not 
perform fence insertion. However, static robustness analysis is a whole program analysis. 
Therefore when do not have access to entire program or a program is not robust we 
introduce appropriate fences to preserve the transformation correctness. 
To do so, we extend the fence elimination algorithm of \citet{} especially for ARMv8 where 
we can use different types of fences.

\subsection{Experimental Result} 
We are implementing the mapping schemes and the analyses in LLVM 
and experiment the effectiveness on a number of testcases. 
We do not intend to perform binary translation from one ISA to another. 
Instead while compiling C11 programs we capture the effect 
of architecture to architecture mapping in the LLVM code generation phase. 
For instance, we know that a non-atomic store $\Wlab$ in C11 generates a 
$\mov(\Wlab)$ instruction in x86 and $\str$ instruction in ARMv8. 
However, following the x86 to ARMv8 mapping in \cref{tab:xarm} 
we know $\mov(\Wlab) \leadsto \dmbst;\str$. 
Therefore to capture C11 $\leadsto$ x86 $\leadsto$ ARMv8 mapping 
we generate $\Wlab \leadsto \dmbst;\str$ for C11 to ARMv8 mapping. 
We expect the later optimizations will remove some of these extra fences and 
the resulting code would be as good as  x86 $\leadsto$ ARMv8 mapping.

{\bf Status.} I have implemented the x86 to ARMv8 mappings. 
Now I am working on the other mappings and the fence elimination optimizations. 



 

==> cxarch.tex <==
% !TEX root = paper.tex


\section{Mappings for C/C++11 Concurrency}
\label{sec:cmappings}

C/C++ concurrency provides a platform independent abstraction for 
all these architectures and intends to achieve efficient mappings on these architectures. 
In this section we study architecture to architecture mapping for C/C++ concurrent programs. 

In this mapping we exploit the C/C++ semantic rule: data race results in undefined behavior. 
We denote such mapping as $\mapsto_{C11}$.
In this case we do not introduce fences if we know that a load or store access is generated from 
a C/C++ non-atomic load or store access respectively. 
We prove that such a mapping safe as stated in \cref{th:cxarch}

\begin{theorem}
If a load or store access is generated from C11 
non-atomic load or store then the following mapping schemes are safe.
\begin{itemize}
\item x86 to ARMv8: $\mov(\Wlab) \mapsto_{C11} \str$ and $\mov(\Rlab) \mapsto_{C11} \ldr$
\item ARMv8 to ARMv7/ARMv7-mca: $\str \mapsto_{C11} \str$ and $\mov(\Rlab) \mapsto_{C11} \str$
\end{itemize}
\end{theorem}

\begin{proof}

%When a C11 program has data race then the behavior is undefined. 
%In that case any mapping is allowed.
%Therefore we consider non racy C11 programs and respective executions. 

Let $\mbbp_{C11} \mapsto \mbbp_{x86} \mapsto \mbbp_{ARMv8}$ following 
the mapping scheme in \cref{fig:cxarma}.

The mapping can be represented as a combination of following transformation steps.

\begin{enumerate}

\item $\mbbp_{C11} \mapsto \mbbp_{x86}$ mapping from \citet{mappings}.

\item $\mbbp_{x86} \mapsto \mbbp_{ARMv8}$ mappings from \cref{tab:xarm} with a 
strengthening of $\dmbst;\str$ to $\dmbfull;\str$ for $\mov(\Wlab)$ mapping.

\item Elimination of 

\begin{enumerate}
\item leading $\dmbfull$ fence after $\mov(\Wlab) \mapsto  \dmbfull;\str$ 
for $\Wlab_\MOna$ accesses and 

\item trailing $\dmbld$ fence after 
$\mov(\Rlab) \mapsto  \ldr;\dmbld$ for $\Rlab_\MOna$.
\end{enumerate}
\end{enumerate}

We know (1) and (2) are sound and show that transformation (3) is sound.

Let $\ex_a$ and $\ex'_a$ be the consistent execution of $\mbbp_{ARMv8}$ 
before and after the transformation (3).
Let $\ex$ be correspnding C11 execution $\mbbp_{C11}$.
 and 
we know $\mbbp_{C11}$ is race-free. 
Therefore for all non-atomic event $a$ in $\ex$ if there exist 
another same-location event $b$ then $\ex.\lhb^=(a,b)$ holds. 


Now we consider x86 to ARMv8 mapping scheme.

Considering the $\lhb$ definition following are the possibilities:
 
\Case{$[\E_\MOna];\ex.\lpo;[\WUlab_{\sqsupseteq \MOrlx}]$}

$\implies [\E];\ex_a.\lpo;[\dmbld];\ex_a.\lpo;[\dmbfull];\ex_a.\lpo;[\E]$

$\implies [\E];\ex'_a.\lpo;[\dmbfull];\ex'_a.\lpo;[\E]$

$\implies [\E];\ex'_a.\bob;[\E]$


\Case{$[\RUlab_{\sqsupseteq \MOrlx}];\ex.\lpo;[\E_\MOna]$} 

$\implies [\Rlab];(\ex_a.\rmw;\ex_a.\dmbfull \cup \ex_a.\lpo;[\dmbld]);\ex_a.\lpo;[\E]$

$\implies [\E];\ex'_a.\bob;[\E]$

Therefore $\ex'_a.\bob = \ex_a.\bob$ and the transfmation is sound for x86 to ARMv8 mapping.

\bigskip

Now we consider ARMv8 to ARMv7 mapping scheme.

Considering the $\lhb$ definition following are the possibilities:
 
\Case{$[\E_\MOna];\ex.\lpo;[\Flab_{\sqsupseteq \MOrel}];\ex.\lpo;[\WUlab_{\MOrlx}] \cup [\E_\MOna];\ex.\lpo;[\WUlab_{\sqsupseteq \MOrlx}]$}

$\implies [\E];\ex_a.\lpo;[\dmbfull];\ex_a.\lpo;[\Wlab \cup \rmw]$

$\implies [\E];\ex'_a.\lpo;[\dmb];\ex'_a.\lpo;[\E]$

$\implies [\E];\ex'_a.\fence;[\E]$


\Case{$[\RUlab_{\sqsupseteq \MOrlx}];\ex.\lpo;[\E_\MOna] \cup [\RUlab_{\MOrlx}];\ex_\lpo;[\Flab_{\sqsupseteq \MOacq}];\ex.\lpo;[\E_\MOna]$} 

$\implies [\Rlab];\ex_a.\lpo;[\dmbfull];\ex_a.\lpo$

$\implies [\E];\ex'_a.\fence;[\E]$

Therefore $\ex'_a.\fence = \ex_a.\fence$ and the transfmation is sound for ARMv8 to ARMv7 mapping.


%
%C11 allows reordering of certain access pairs. 
%The effect of reordering can be observed by certain 
%concurrent events which implies a data race in $\ex$.
%
%Moreover, we know $\eco = (\lrf \cup \co \cup \fr)^+$. 
%
%Therefore $[\E_\MOna];\ex.\eco \subseteq [\E_\MOna];\ex.\lhb$  and 
%$\ex.\eco;[\E_\MOna] \subseteq \ex.\lhb;[\E_\MOna]$.
%
%
%
%
%Assume a 
% 
%Therefore $[\E_\MOna];\ex.\lhb;\ex.\eco^? \cup \ex.\lhb;\ex.\eco^?;\ex[\E_\MOna]$ 
%
%$\implies [\E_\MOna];\ex.\lhb \cup \ex.\lhb;\ex[\E_\MOna]$
%
%$\implies [\E_\MOna];(\ex.\lpo \cup \ex.\lrf)^+ \cup (\ex.\lpo \cup \ex.\lrf)^+;\ex[\E_\MOna]$
%
%$\implies [\E];(\ex_a.\bob \cup \ex_a.\rfe)^+ \cup (\ex_a.\bob \cup \ex_a.\rfe)^+;\ex[\E]$
% 
%$\implies [\E];\ex_a.\ob \cup \ex_a.\ob;\ex[\E]$
%
%Therefore $[\E_\MOna];\ex.\lhb \cup ;[\E_\MOna]$ is irreflexive as $[\E];\ex.\lhb;[\E]$ is irreflexive.
%
% 
%Therefore $\hb;\eco^? \implies $


\end{proof}

%\begin{proof}
%
%
%
%%%%%%%
%Let $a$ be a non-atomic event in $\ex$ and $a'$ be the corresponding event in $\ex_a$. 
%
%If there exists no event $b$ such that $a.\lloc = b.\lloc$. 
%In that case $a$ can be treated as a thread-local variable 
%and requires to additional fence.
%
%\bigskip 
%
%\textbf{Otherwise}
%
%Let $b$ be another event in $\ex$ and $b'$ be the corresponding event in $\ex_a$ 
%such that $a.\lloc = b.\lloc$.
%
%\Case{$\ex.\lhb(a,b)$}
%
%Possible scenarios:
%
%\Subcase{$\ex.\lpo(a,b)$}
%
%In this case $\ex_a.\lpo(a',b')$. 
%
%If 
%
%
%
%$a$ and $b$ are allowed to be reordered in C11 and 
%the 
%
%
%\Subcase{$(a,b) \in \ex.\lpo;[\WUlab_\MOrel];( \ex.\lpo;[\rels] \cup [\rels];\ex.\SW)^*$}
%
%In this case 
%\begin{itemize}
%
%\item Following x86 $\mapsto_{C11}$ ARMv8 mapping in \cref{fig:cxarma}
%
%$\WUlab_\MOrel \mapsto \mov(\Wlab) \mapsto \dmbfull;\Wlab$.
%
%In this cases $[\set{a'}];\ex.\lpo;[\dmbfull];\ex.\lpo$ where $a'$ is generated from $a$. 
%
%It implies $[\set{a'}];\ex.\bob;[\set{e}]$ where $e$ is $\lpo$-successor of $\dmbfull$ event.
%
%\item Following ARMv8 $\mapsto_{C11}$ ARMv7 mapping in \cref{fig:cxarma}
%
%$\WUlab_\MOrel \mapsto \mapsto \dmbst;\Wlab \mapsto \dmb;\Wlab$.
%
%In this cases $[\set{a'}];\ex.\lpo;[\dmb];\ex.\lpo$ where $a'$ is generated from $a$. 
%
%It implies $[\set{a'}];\ex.\fence;[\set{e}]$ where $e$ is $\lpo$-successor of $\dmb$ event.
%
%\end{itemize} 
%
%
%
%\Subcase{$(a,b) \in \ex.\lpo;[\Flab_\MOrel];( \ex.\lpo;[\rels] \cup [\rels];\ex.\SW)^*$}
%
%In this case there exists $c$ such that 
%
%
%
%
%
%Same as the other subcase where $\Flab_\MOrel \mapsto \mov(\Wlab) \mapsto \dmbfull;\Wlab$
%
%In both cases the introduced leading $\dmbfull$ or $\dmb$ fences in respective mappings 
%suffice to establish order with event $a$.
%
%\end{proof}

==> fence-elim.tex <==
% !TEX root = main.tex

\section{Fence Elimination}
\label{sec:felim}






%$\felim(\srcp, \tgtp, A, B, C)$ where there exists $i$ such that  
%\begin{itemize}
%\item $\tau_1.A.\tau_2.\tau_3.B.\tau_4 \in \tgtp(i)$ 
%\item $\tau_1.A.\tau_2.C.\tau_3.B.\tau_4 \in \srcp(i)$
%%\item $\tau_2$ and $\tau_3$ have no fence access $D$ such that $C \sqsubseteq D$ 
%\item $\denot{A}.\lloc \neq \denot{B}.\lloc$, $\denot{C}.\lloc = \bottom$
%\end{itemize}
%
%We define 'singluar' fence as follows:
%
%
%%%%%%%%%
%%
%%$\deletable(\ex, F, A, B)$
%%
%%A fence event F is deletable in $X$ if there exists no events $A, B$ 
%%where $\ex.\lpo(A,X) \land \lpo(X,B)$ such that 
%%not (A = st and B = ld) or 
%%(A = st and B = ld) and there exists another fence $\ex.\lpo(A,D)$ and $\ex.\lpo(A,C)$. 
%%
%%%%%%%%%


\subsection{Fence Elimination in x86}
\label{sec:xfelim}

%%%%%%%%% old but correct %%%%%%%%%%%%
%\begin{theorem}
%\label{th:xfenceelim}
%Let $C$ be an $\mfence$ in a given x86 code sequence of the form $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \in \srcp(i)$ where $i$ is a thread identifier.
%Then $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \leadsto \alpha_1;A;\alpha_2;\skips;\beta_1;B;\beta_2$ results in target program $\tgtp$ where $\alpha_1;A;\alpha_2;\skips;\beta_1;B;\beta_2 \in \tgtp$. 
%The transformation is safe when 
%
%(i) there exists no $A$ and $B$ such that $A = \mov(\Wlab)$ and $B = \mov(\Rlab)$ or 
%
%(ii)  $\alpha_2$ or $\beta_1$ have $\mfence$.
%
%%
%%(i) $\neg (A = \mov(\Wlab) \land B = \mov(\Rlab))$ or 
%%
%%(ii) $\mfence \in \alpha_2 \lor \mfence \in \beta_1$
%\end{theorem}
%%%%%%%%% old but correct %%%%%%%%%%%%


\begin{theorem}
\label{th:xfenceelim}
Let $\srcp$ be an x86 program and $\tgtp$ is the program after eliminating an $\mfence$ from thread $i$ i.e. 
$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \F \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
The transformation is safe when: 

(i) $a=\Wlab(x,v) \land b=\Rlab(y,v') \implies x = y$ or 

(ii) $\F \in \alpha_2 \lor \F \in \beta_1$
\end{theorem}


\begin{proof}

We show:
\[
\inarr{
\srcp \leadsto \tgtp \implies \forall \ex_t \in \denot{\tgtp}~\exists \ex_s \in \denot{\srcp}.~\behav(\ex_t) = \behav(\ex_s) 
}
\]

Given a $\ex_t \in \denot{\tgtp}$ we define $\ex_s \in \srcp$ by introducing the corresponding fence event $\event$ such that  
for all events $w \in \ex_s.\WUlab \cup \ex_s.\F$,
\begin{itemize}
\item if $(w,\event) \in \ex_s.\mo^?;\ex_s.\xhb$ holds then $\ex_s.\mo(w,\event)$. 
\item Otherwise $\ex_s.\mo(\event,w)$.
\end{itemize}

%\begin{itemize}
%\item $\ex_s.\mo(w,\event)$ when $w \in \ex_s.\WUlab \cup \ex_s.\F$ and $(w,\event) \in \ex_s.\mo^?;\ex_s.\xhb$. 
%%\item 
%%$\ex_s.\mo(\event,w)$ when $w \in \ex_s.\WUlab \cup \ex_s.\F$ and $(w,\event) \in \ex_s.\xhb;\ex_s.\mo^?$.
%\end{itemize}
We know $\ex_t$ is consistent. 

Now we show $\ex_s$ is consistent.

We prove by contradiction.

(irrHB)
Assume $\ex_s$ has $\ex_s.\xhb$ cycle. 
We know the incoming and outgoing edges to $\event$ are $\ex_s.\lpo$ edges and therefore 
$\ex_t.\xhb$ already has a cycle. 
However, we know $\ex_t.\xhb$ is irreflexive. Hence a contradiction and $\ex_s.\xhb$ is irreflexive.

\bigskip

(irrMOHB)
Assume $\ex_s$ has $\ex_s.\mo;\ex_s.\xhb$ cycle. 
We already know that $\ex_t.\mo;\ex_t.\xhb$ is irreflexive. 
Therefore the cycle contains $\event$. 
Two possiblilities: 

\Case{$\event \in \dom(\ex_s.\xhb)$ and $\event \in \codom(\ex_s.\mo)$}

Suppose $\ex_s.\xhb(\event,w)$ and $\ex_s.\mo(w,\event)$. 
However, from definition we already know $\ex_s.\xhb(\event,w) \implies \ex_s.\mo(\event,w)$ when $w \in \ex_s.\WUlab \cup \ex_s.\F$. 
Hence a contradiction and $\ex_s.\mo;\ex_s.\xhb$ is irreflexive in this case.

\Case{$\event \in \codom(\ex_s.\xhb)$ and $\event \in \dom(\ex_s.\mo)$}

Suppose $\ex_s.\xhb(w,\event)$ and $\ex_s.\mo(\event,w)$. 
However, from definition we already know $\ex_s.\xhb(w,\event) \implies \ex_s.\mo(w,\event)$ when $w \in \ex_s.\WUlab \cup \ex_s.\F$. 
Hence a contradiction and $\ex_s.\mo;\ex_s.\xhb$ is irreflexive in this case.

\bigskip

(irrFRHB)
We know $\ex_t$ does not have a $\ex_t.\fr;\ex_t.\xhb$ cycle.
We also know $\fr \subseteq (\WUlab \times \WUlab)$ and hence event $\event \in \F$ does not introduce 
any new $\ex_s.\fr;\ex_\xhb$ cycle. 
Therefore $\ex_s.\fr;\ex_\xhb$ is irreflexive. 

\bigskip

(irrFRMO)

We know $\ex_t$ does not have a $\ex_t.\fr;\ex_t.\mo$ cycle.
We also know $\fr \subseteq (\WUlab \times \WUlab)$ and hence event $\event \in \F$ does not introduce 
any new $\ex_s.\fr;\ex_\mo$ cycle. 
Therefore $\ex_s.\fr;\ex_\mo$ is irreflexive. 

\bigskip

(irrFMRP)

Assume $\ex_s$ has a $\ex_s.\fr;\ex_s.\mo;\ex_s.\rfe;\ex_s.\lpo$ cycle in $\ex_s$ cycle.

In that case the cycle is of the form:

$[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo;[\ex_s.\WUlab];\ex_s.\rfe;[\ex_s.\RUlab];\ex_s.\lpo;[\ex_s.\RUlab]$.

We know $\event \in \F$ and therefore does not introduce this cycle in $\ex_s$.

In that case $\ex_t$ already has a $\ex_t.\fr;\ex_t.\mo;\ex_t.\rfe;\ex_t.\lpo$ cycle which is a contradiction.

Hence $\ex_s.\fr;\ex_s.\mo;\ex_s.\rfe;\ex_s.\lpo$ cycle in $\ex_s$ is irreflexive.

\bigskip

(irrUF)

Assume $\ex_s$ has a $\ex_s.\fr;\ex_s.\mo;[\ex_s.\Ulab \cup \ex_s.\F];\ex_s.\lpo$ cycle.

Two possiblities 

\Case{$\ex_s.\fr;\ex_s.\mo;[\ex_s.\Ulab];\ex_s.\lpo$}

It implies a $\ex_t.\fr;\ex_t.\mo;[\ex_t.\Ulab];\ex_t.\lpo$ cycle. 

However, we know $\ex_t$ satisfies (irrUF) and hence a contradiction. 

\Case{$\ex_s.\fr;\ex_s.\mo;[\ex_s.\F];\ex_s.\lpo$}

It implies a $[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo;[\ex_s.\F];\ex_s.\lpo;[\ex_s.\RUlab]$ cycle 
created by the introduced event $\event \in \F$.

It implies $[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$

From definition, we know $[\ex_s.\WUlab];\ex_s.\mo;[\set{\event}]$ when $[\ex_s.\WUlab];\ex_s.\mo^?;\ex_s.\xhb;[\set{\event}]$ holds.

Thus $[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$

$\implies [\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\xhb;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$

$\implies [\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];(\ex_s.\xhb^?;[\ex_s.\WUlab];\ex_s.\rfe;\ex_s.\lpo \cup \ex_s.\lpo);[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$

\begin{flalign*}
\implies &  [\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\xhb^?;[\ex_s.\WUlab];\ex_s.\rfe;\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab] & \\
& \cup [\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab] &
\end{flalign*}

\begin{flalign*}
\implies &  [\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\xhb^?;[\ex_s.\WUlab];\ex_s.\rfe;\ex_s.\lpo;[\ex_s.\RUlab] & \\
& \cup [\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab] &
\end{flalign*}

Now we consider two subcases:

\Subcase{$[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\xhb^?;[\ex_s.\WUlab];\ex_s.\rfe;\ex_s.\lpo;[\ex_s.\RUlab] $}

$\implies [\ex_t.\RUlab];\ex_t.\fr;[\ex_t.\WUlab];\ex_t.\mo^?;[\ex_t.\WUlab];\ex_t.\xhb^?;[\ex_t.\WUlab];\ex_t.\rfe;\ex_t.\lpo;[\ex_t.\RUlab]$

$\implies  [\ex_t.\RUlab];\ex_t.\fr;\ex_t.\mo^?;\ex_t.\rfe;\ex_t.\lpo;[\ex_t.\RUlab]$

This is a contradiction as $\ex_t$ satisfies (irrFMRP).

\Subcase{$[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$}

Now we consider the $[\ex_s.\WUlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$ subsequence.

Possible cases:

\Subsubcase{$[\ex_s.\Wlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\Rlab]$ }

%%%%%%%%
It implies $[\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\F];\ex_t.\lpo;[\ex_t.\Rlab]$ from the definition.

$\implies [\ex_t.\Wlab];\ex_t.\mo;[\ex_t.\F];\ex_t.\lpo;[\ex_t.\Rlab]$.

In that case there exists a $\ex_t.\fr;\ex_t.\mo;[\ex_t.\F];\ex_t.\lpo$ cycle. 

This is a contradiction as $\ex_t$ satisfies (irrFMRP).

\smallskip

\Subsubcase{$[\ex_s.\WUlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\Ulab]$ }

It implies $[\ex_t.\WUlab];\ex_t.\lpo;[\ex_t.\Ulab]$.

It implies $[\ex_t.\WUlab];\ex_t.\mo;[\ex_t.\Ulab]$ as $\ex_t$ satisfies (irrMOHB).

In this case $[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$

$\implies [\ex_t.\RUlab];\ex_t.\fr;[\ex_t.\WUlab];\ex_t.\mo^?;[\ex_t.\WUlab];\ex_t.\mo;[\ex_t.\Ulab]$

$\implies [\ex_t.\RUlab];\ex_t.\fr;\ex_t.\mo;[\ex_t.\Ulab]$

Hence a contradiction as $\ex_t$ satisfies (irrFRMO).

\smallskip

\Subsubcase{$[\ex_s.\Ulab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\Rlab]$}

It implies $[\ex_t.\Ulab];\ex_t.\lpo;[\ex_t.\Rlab]$ and in consequence a 
$[\ex_t.\Rlab];\ex_t.\fr;[\ex_t.\WUlab];\ex_t.\mo^?;[\ex_t.\Ulab];\ex_t.\lpo;[\ex_t.\Rlab]$ cycle.

Now, $[\ex_t.\Rlab];\ex_t.\fr;[\ex_t.\WUlab];\ex_t.\mo^?;[\ex_t.\Ulab];\ex_t.\lpo;[\ex_t.\Rlab]$

$\implies [\ex_t.\Rlab];\ex_t.\fr;[\ex_s.\Ulab];\ex_t.\lpo;[\ex_t.\Rlab] \cup [\ex_t.\Rlab];\ex_t.\fr;\ex_t.\mo;[\ex_t.\Ulab];\ex_t.\lpo;[\ex_t.\Rlab]$

$\implies [\ex_t.\Rlab];\ex_t.\fr;\ex_t.\xhb;[\ex_t.\Rlab] \cup [\ex_t.\Rlab];\ex_t.\fr;\ex_t.\mo;[\ex_t.\Ulab];\ex_t.\lpo;[\ex_t.\Rlab]$

Hence a contradiction as $\ex_t$ satisfies (irrFRHB) and (irrUF).

\bigskip

$\behav(\ex_s) = \behav(\ex_t)$ holds as $\rloc{\ex_s.\mo} = \rloc{\ex_t.\mo}$.
\end{proof}


\subsection{Fence Elimination in ARMv8}
\label{sec:armv8felim}

\begin{observation}
\label{obs:armv8fenceelim}
Let $\mbbp$ be an ARMv8 program generated from an 
x86 program following the mappings in \cref{tab:xarm}. 
In this case for all consistent execution $\ex \in \denot{\mbbp}$ 
the followings hold:

\begin{enumerate}
\item  A non-RMW load event is immediately followed by a $\dmbld$ event.
\[\codom([\ex.\Rlab];(\imm(\ex.\lpo) \setminus \ex.\rmw) = [\ex.\dmbld]\]

\item A non-RMW store event is immediately preceeded by a $\dmbst$ event, 
\[\codom([\ex.\dmbst];\imm(\ex.\lpo)= [\ex.\Wlab]\]  

\item An RMW is immediately preceeded by a $\dmbfull$ event, 
\[\codom(\ex.\rmw^{-1};\imm(\ex.\lpo^{-1})) \subseteq \ex.\dmbfull\]

\item An RMW is immediately followed by a $\dmbfull$ event, 
\[\codom(\ex.\rmw;\imm(\ex.\lpo)) \subseteq \ex.\dmbfull\]
\end{enumerate}
\end{observation}

%\begin{theorem}
%\label{th:arm8dmbfullelim}
%Let $\mapp$ be an ARMv8 program generated from an 
%x86 program following the mappings in \cref{tab:xarm}. 
%Suppose $\mapp$ contains a $\dmbfull$ fence 
%
%
%$\felim(\srcp, \tgtp, A, B, \dmbfull)$ is safe in ARMv8 when 
%$\neg (A = \str \lor \osc \land B = \oll \lor \ldr)$. 
%\end{theorem}



%\begin{theorem}
%\label{th:arm8dmbfullelim}
%Suppose $\srcp$ is an ARMv8 program from an 
%x86 program following the mappings in \cref{tab:xarm}. 
%%$\felim(\srcp, \tgtp, A, B, \dmbfull)$ is safe in ARMv8 when 
%%$\neg (A = \str \lor \osc \land B = \oll \lor \ldr)$. 
%
%Let $C$ be an $\dmbfull$ in a code sequence of the form $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \in \srcp(i)$ where $i$ is a thread identifier.
%Then $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \leadsto \alpha_1;A;\alpha_2;\skips;\beta_1;B;\beta_2$ results in target program $\tgtp$ where $\alpha_1;A;\alpha_2;\skips;\beta_1;B;\beta_2 \in \tgtp$. 
%The transformation is safe when 
%
%(i) there exists no $A$ and $B$ such that $A = \str \lor \osc$ and $B = \oll \lor \ldr$ or 
%
%%$\neg (A = \str \lor \osc \land B = \oll \lor \ldr)$ or 
%
%(ii)  $\alpha_2$ or $\beta_1$ have $\dmbfull$ fence.
%
%%$\dmbfull \in \alpha_2 \land \dmbfull \in \beta_1$
%\end{theorem}
%
%
%%%%%%%%%%%%
%%Alternative theorem:
%%
%%\begin{theorem}
%%Suppose $\srcp$ is an ARMv8 program from an 
%%x86 program following the mappings in \cref{tab:xarm}. 
%%Let $f$ be a $\dmbfull$ fence in $\srcp$. Elimination of $f$ is safe when $(_,f,_) \notin \fenced(G, \Wlab, \dmbfull, \Rlab)$ or there exists 
%%where $G$ is the CFG of program $\srcp$. 
%%\end{theorem}
%%%%%%%%%%%%


\begin{theorem}
\label{th:arm8dmbfullelim}
Let $\srcp$ be an ARMv8 program  generated from an x86 program following the mappings in \cref{tab:xarm} and 
let $\tgtp$ be the program after eliminating a $\dmbfull$ from thread $i$ i.e. 
$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \dmbfull \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
The transformation is safe when: 

(i) $a=\Wlab(x,v) \land b=\Rlab(y,v') \implies x = y$ or 

(ii) $\exists c \in \alpha_2 \cdot \beta_1$ such that $c = \dmbfull$.
\end{theorem}


To prove \cref{th:arm8dmbfullelim}, we show:
\[
\inarr{
\srcp \leadsto \tgtp \implies \forall \ex_t \in \denot{\tgtp}~\exists \ex_s \in \denot{\srcp}.~\behav(\ex_t) = \behav(\ex_s) 
}
\]


\begin{proof}

Given a target execution $\ex_t \in \denot{\tgtp}$ we define a source execution $\ex_s \in \srcp$ by introducing the corresponding fence event $\event \in \dmbfull$. 

We know target execution $\ex_t$ satisfies (internal) and (atomic). 
From definition, source execution $\ex_s$ also supports (internal) and (atomic) as the respective relations remain unchanged. 

We now prove that $\ex_s$ satisfies (external). 

%%%%%%%%%%%%%%%%%%%%%

We prove by contradiction. 

Assume $\ex_s$ violates (external).

From definition we know that $\ex_s.\obs = \ex_t.\obs$, 
$\ex_s.\dob = \ex_t.\dob$, $\ex_s.\aob = \ex_t.\aob$. 

In that case there exists events $(a,b) \in \ex_s.\bob$ but $(a,b) \notin \ex_t.\bob$. 


Considering possible cases of $a$ and $b$:


\Case{$(a,b) \in [\ex_s.\Rlab] \times [\ex_s.\E]$} Two subcases:

\Subcase{$a \notin \dom(\ex_s.\rmw)$}

It implies $(a,b) \in [\ex_t.\Rlab];\ex_t.\lpo;[\ex_t.\dmbld];\ex_t.\lpo;[\ex_t.\E]$ from Observation (1) in \cref{obs:armv8fenceelim}.

$\implies (a,b) \in [\ex_t.\Rlab];\ex_t.\bob;[\ex_t.\E]$

Hence a contradiction and $\ex_s$ violates (external).

\Subcase{$a \in \dom(\ex_s.\rmw)$}

It implies $(a,b) \in [\ex_t.\Rlab];\ex_t.\lpo;[\ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\E]$

$\implies (a,b) \in [\ex_t.\Rlab];\ex_t.\bob;[\ex_t.\E]$

Hence a contradiction and $\ex_s$ violates (external).


\Case{$(a,b) \in [\ex_s.\Wlab] \times [\ex_s.\Wlab]$}

$\implies [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbst];\ex_t.\lpo;[\ex_t.\Wlab]$ from Observation (2) in \cref{obs:armv8fenceelim}.

$\implies [\ex_t.\Wlab];\ex_t.\bob;[\ex_s.\Wlab]$ 

This is a contradiction and hence $\ex_s$ satisfies (external). 

\medskip

\Case{$(a,b) \in [\ex_s.\Wlab] \times [\ex_s.\Rlab]$}

It implies $(a,b) \in [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\Rlab]$ from the condition in \cref{th:armv8dmbfullelim}.

$\implies [\ex_t.\Wlab];\ex_t.\bob;[\ex_s.\Rlab]$ 

This is a contradiction and hence $\ex_s$ satisfies (external). 


%%%%%%%%%%%%%%
%
%\Case{$(a,b) \in [\ex_s.\Rlab] \times [\ex_s.\E]$}
%
%$\implies [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbld];\ex_t.\lpo;[\ex_s.\Wlab]$ from Observation (2) in \cref{obs:armv8fenceelim}.
%
%$\implies [\ex_t.\Wlab];\ex_t.\bob;[\ex_s.\Wlab]$ 
%
%This is a contradiction and hence $\ex_s$ satisfies (external). 
%
%$\Case{$(a,b) \in [\ex_s.\Wlab] \times [\ex_s.\Rlab]$}
%
%$\implies [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbfull];\ex_t.\lpo;[\ex_s.\Rlab]$ from \cref{obs:armv8dmbfullelim}.
%
%$\implies [\ex_t.\Wlab];\ex_t.\bob;[\ex_s.\Rlab]$ 
%
%This is a contradiction and hence $\ex_s$ satisfies (external). 
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%
%
%by showing $\ex_t.\ob = \ex_s.\ob$.
%
%From definition we know that $\ex_t.\obs = \ex_s.\obs$, $\ex_t.\dob = \ex_s.\dob$, $\ex_t.\aob = \ex_s.\aob$. 
%We show that $\ex_s.\bob = \ex_t.\bob$.
%
%Considering the possible cases of $\ex_t.\bob$:
%
%\Case{$[\ex_t.\Wlab];\ex_t.\bob;[\ex_t.\Wlab]$}
%
%$\implies [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbst];\ex_t.\lpo;[\ex_s.\Wlab]$ from Observation (2) in \cref{obs:armv8fenceelim}.
%
%$\implies [\ex_s.\Wlab];\ex_s.\lpo;[\ex_s.\dmbst];\ex_s.\lpo;[\ex_s.\Wlab]$
%
%$\implies [\ex_s.\Wlab];\ex_s.\bob;[\ex_s.\Wlab]$
%
%\medskip
%
%\Case{$[\ex_t.\Wlab];\ex_t.\bob;[\ex_t.\Rlab]$}
%
%It implies $[\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\Rlab]$.
%
%In this case no fence is eliminated and hence $[\ex_s.\Wlab];\ex_s.\bob;[\ex_s.\Rlab]$ holds.
%
%\medskip
%
%\Case{$[\ex_t.\Rlab];\ex_t.\bob;[\ex_t.\Rlab \cup \ex_t.\Wlab]$}
%
%Two subcases:
%
%\Subcase{$[\ex_t.\Rlab];\ex_t.\rmw;\ex_t.\lpo;[\ex_t.\Rlab \cup \ex_t.\Wlab]$}
%
%It implies $[\ex_t.\Rlab];\ex_t.\rmw;\ex_t.\lpo;[\ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\Rlab \cup \ex_t.\Wlab]$
%
%$\implies [\ex_s.\Rlab];\ex_s.\rmw;\ex_s.\lpo;[\ex_s.\dmbfull];\ex_s.\lpo;[\ex_s.\Rlab \cup \ex_s.\Wlab]$
%
%$\implies [\ex_s.\Rlab];\ex_s.\aob;\ex_s.\bob;[\ex_s.\Rlab \cup \ex_s.\Wlab]$
%
%$\implies [\ex_s.\Rlab];\ex_s.\ob;[\ex_s.\Rlab \cup \ex_s.\Wlab]$
%
%\Subcase{Otherwise}
%
%It implies $[\ex_t.\Rlab];\ex_t.\lpo;[\ex_t.\dmbld];\ex_t.\lpo;[\ex_t.\Rlab \cup \ex_t.\Wlab]$
%
%$\implies [\ex_s.\Rlab];\ex_s.\lpo;[\ex_s.\dmbld];\ex_s.\lpo;[\ex_s.\Rlab \cup \ex_s.\Wlab]$
%
%$\implies [\ex_s.\Rlab];\ex_s.\bob;[\ex_s.\Rlab \cup \ex_s.\Wlab]$
%
%$\implies [\ex_s.\Rlab];\ex_s.\ob;[\ex_s.\Rlab \cup \ex_s.\Wlab]$
%
%\bigskip
%
%Thus $\ex_s.\ob = \ex_t.\ob$.

\bigskip

As a result, $\ex_s$ also satisfies (external) and is ARMv8 consistent.

\medskip

Moreover, we know that $\ex_s.\co = \ex_t.\co$. Hence $\behav(\ex_s)=\behav(\ex_t)$.


%\begin{theorem}
%\label{th:arm8dmbstelim}
%Suppose $\srcp$ is an ARMv8 program from an 
%x86 program following the mappings in \cref{tab:xarm}. 
%Let $C$ be an $\dmbst$ in a code sequence of the form $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \in \srcp(i)$ where $i$ is a thread identifier.
%Then $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \leadsto \alpha_1;A;\alpha_2;\skips;\beta_1;B;\beta_2$ results in target program $\tgtp$ where $\alpha_1;A;\alpha_2;\skips;\beta_1;B;\beta_2 \in \tgtp$. 
%The transformation is safe when 
%
%(i) there exists no $A$ and $B$ such that $A = \str \lor \osc$ and $B = \str$ or 
%
%(ii)  $\alpha_2$ or $\beta_1$ have $\dmbfull$ or $\dmbst$ fence.
%%
%%
%%(i) $\neg (A = \str \lor \osc \land B = \str)$ or 
%%
%%(ii) $\set{\dmbst, \dmbfull} \in \alpha_2 \lor \set{\dmbst, \dmbfull} \in \beta_1$
%\end{theorem}


\begin{theorem}
\label{th:arm8dmbstelim}
Let $\srcp$ be an ARMv8 program  generated from an x86 program following the mappings in \cref{tab:xarm} and 
let $\tgtp$ be the program after eliminating a $\dmbfull$ from thread $i$ i.e. 
$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \dmbst \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
The transformation is safe when: 

(i) $a=\Wlab(x,v) \land b=\Wlab(y,v') \implies x = y$ or 

(ii) $\exists c \in \alpha_2 \cdot \beta_1$ such that $c=\dmbfull \lor \dmbst$.
\end{theorem}



To prove \cref{th:arm8dmbstelim}, we show:
\[
\inarr{
\srcp \leadsto \tgtp \implies \forall \ex_t \in \denot{\tgtp}~\exists \ex_s \in \denot{\srcp}.~\behav(\ex_t) = \behav(\ex_s) 
}
\]


\begin{proof}

Given a target execution $\ex_t \in \denot{\tgtp}$ we define a source execution $\ex_s \in \srcp$ by introducing the corresponding fence event $\event \in \dmbfull$. 

We know target execution $\ex_t$ satisfies (internal) and (atomic). 
From definition, source execution $\ex_s$ also supports (internal) and (atomic) as the respective relations remain unchanged. 

We now prove that $\ex_s$ satisfies (external) by showing $\ex_t.\ob = \ex_s.\ob$.

From definition we know that $\ex_t.\obs = \ex_s.\obs$, $\ex_t.\dob = \ex_s.\dob$, $\ex_t.\aob = \ex_s.\aob$. 

In that case there exists events $(a,b) \in \ex_s.\bob$ but $(a,b) \notin \ex_t.\bob$. 


Considering possible cases of $a$ and $b$:


\Case{$(a,b) \in [\ex_s.\Rlab] \times [\ex_s.\E]$}


It implies $(a,b) \in [\ex_t.\Rlab];\ex_t.\lpo;[\ex_t.\dmbld \cup \ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\E]$ from Observation (1) and (4) in \cref{obs:armv8fenceelim}.

$\implies (a,b) \in [\ex_t.\Rlab];\ex_t.\bob;[\ex_t.\E]$

Hence a contradiction and $\ex_s$ violates (external).


\Case{$(a,b) \in [\ex_s.\Wlab] \times [\ex_s.\Wlab]$}

$\implies [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbst \cup \ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\Wlab]$ from the condition in \cref{th:armv8dmbfullelim}.

$\implies [\ex_t.\Wlab];\ex_t.\bob;[\ex_s.\Wlab]$ 

This is a contradiction and hence $\ex_s$ satisfies (external). 

\Case{$(a,b) \in [\ex_s.\Wlab] \times [\ex_s.\Rlab]$}

It implies $(a,b) \in [\ex_s.\Wlab];\ex_s.\lpo;[\ex_s.\dmbfull];\ex_s.\lpo;[\ex_s.\Rlab]$ as $\ex_s.\bob(a,b)$ holds. 

It implies $(a,b) \in [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\Rlab]$ 

$\implies [\ex_t.\Wlab];\ex_t.\bob;[\ex_s.\Rlab]$ 

This is a contradiction and hence $\ex_s$ satisfies (external). 
\end{proof}

































\end{proof}

==> fence-redundant.tex <==
% !TEX root = main.tex

\section{Compositional Analysis Based Redundant Fence Elimination}
\label{sec:cafelim}

\begin{definition}
$\pairs(\mbbp, R) \triangleq \set{(a,b) \mid \exists i.~a \cdot \tau \cdot b \in \mbbp(i) \land R(a.b)}$
\end{definition}

\begin{definition}
$\cyc(\mbbp,R) \triangleq \set{(a,b) \mid (a,b) \in \pairs(\mbbp,R) \land \exists a_1, b_1, c_1, d_1.~(a_1,b_1) \in \pairs(\mbbp,R) \land (a_2,b_2) \in \pairs(\mbbp,R) \land b.\lloc = a_1.\lloc \land a.\lloc = b_2.\lloc}$
\end{definition}

%\begin{definition}
%$\allcycle(\mbbp) \triangleq \set{\cyc(\mbbp, \E \times \E)}$
%\end{definition}

\subsection{x86}

%\begin{theorem}
%%Suppose $\srcp$ is an x86 program and $\str(X);\tau_1;\mfence;\tau_2;\ldr(Y) \in \srcp(i)$. 
%%The intermediate $\mfence$ is redundant if there exists no $fcycle(\set{\str},\set{\ldr})$ and no $fcycle(\set{\str},\set{\str})$.
%Suppose $\srcp$ is an x86 program and let $(a,f,b) \in \fenced(\WUlab, \RUlab,\F,\srcp)$.  
%The fence $f$ is redundant if there exists no $\pairpath$ such that $(a,b) \in \pairpath_n(\WUlab, \RUlab,\srcp)$.
%\end{theorem}

\begin{theorem}
\label{th:xcycfenceelim}
Let $\srcp$ be an x86 program and $\tgtp$ is the program after eliminating an $\mfence$ from thread $i$ i.e. 
$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \F \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
The transformation is safe when $a.\lloc = b.\lloc$ or $(a,b) \notin \cyc(\srcp, (\Wlab \times \Rlab))$.
\end{theorem}

To prove \cref{th:xcycfenceelim}, we show:
\[
\inarr{
\srcp \leadsto \tgtp \implies \forall \ex_t \in \denot{\tgtp}~\exists \ex_s \in \denot{\srcp}.~\behav(\ex_t) = \behav(\ex_s) 
}
\]


\begin{proof}
Given a target execution $\ex_t \in \denot{\tgtp}$, we define a source execution $\ex_s \in \srcp$ by introducing the corresponding fence event $\event \in \F$ such that following relations hold:

\begin{enumerate}
\item $\lpo$ among other events remains same.

$\ex_t.\lpo(x,y) \implies \ex_s.\lpo(x,y)$ where $x \neq \event \land y \neq \event$.

\item $\rfe$ and $\co$ relations remain same i.e. $\ex_s.\rfe = \ex_t.\rfe$ and $\ex_s.\co = \ex_t.\co$.

\item $\mo$ relations are updated as follows:
\[
\inarr{
\ex_t.\mo \cup \set{(a,\event) \mid (a,\event) \in \ex_t.\rfe^?;[\ex_t.\Wlab \cup \ex_t.\Ulab \cup \ex_t.\F]}
\\ \cup \set{(\event,a) \mid (\event,a) \in \ex_t.\lpo;(\ex_t.\mo \cup \ex_t.\fr);[\ex_t.\Wlab \cup \ex_t.\Ulab \cup \ex_t.\F]} \subseteq \ex_s.\mo
}
\]

\end{enumerate}





Also, 
(1) $\ex_t.\xhb(x,y) \implies \ex_s.\xhb(x,y)$ where $x \neq \event \land y \neq \event$.

(2) $\ex_s.\fr = \ex_t.\fr$


\end{proof}


\subsection{ARMv8}

%\begin{theorem}
%Suppose $\srcp$ is an ARMv8 program and let $(a,f,b) \in \fenced(\E, \E,\dmbfull,\srcp)$.  
%The fence $f$ is redundant if there exists no $\pairpath$ such that $(a,b) \in \pairpath_n(\E, \E,\srcp)$.
%\end{theorem}


\begin{theorem}
\label{th:xcycfenceelim}
Let $\srcp$ be an x86 program and $\tgtp$ is the program after eliminating a fence from thread $i$ i.e. 
$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot c \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$ where $c = \dmbfull \lor \dmbld \lor \dmbst$. 
The transformation is safe when $(a,b) \notin \cyc(\srcp, \aob \cup \bob \cup \dob)$.
\end{theorem}

\subsection{ARMv7}

%\begin{theorem}
%Suppose $\srcp$ is an ARMv7 program and let $(a,f,b) \in \fenced(\E, \E,\dmbfull,\srcp)$.  
%The fence $f$ is redundant if there exists no $\pairpath$ such that $(a,b) \in \pairpath_n(\E, \E,\srcp)$.
%\end{theorem}

\begin{theorem}
\label{th:xcycfenceelim}
Let $\srcp$ be an x86 program and $\tgtp$ is the program after eliminating a $\dmb$ fence from thread $i$ i.e. 
$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \dmb \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
The transformation is safe when $(a,b) \notin \cyc(\srcp, \ppo)$.
\end{theorem}



==> fence-weaken.tex <==
% !TEX root = main.tex

\section{Fence Weakening in ARMv8}
\label{sec:armv8fweaken}

We can perform fence weakening $\dmbfull \leadsto \dmbld;\dmbst$ transformation in ARMv8 when the fence is not between a pair of $\str$ and $\ldr$, and there is no other $\dmbfull$ fence.

%\begin{theorem}
%\label{th:arm8dmbfullweaken}
%$\alpha_1;A;\alpha_2;\dmbfull;\beta_1;B;\beta_2 \leadsto \alpha_1;A;\alpha_2;\dmbld;\dmbst;\beta_1;B;\beta_2$ 
% is safe when 
%
%(i) there exists no $A$ and $B$ such that $A = \str \lor \osc$ and $B = \oll \lor \ldr$ or
%
%
%(ii) $\alpha_2$ and $\beta_1$ have $\dmbfull$ fence.
%
%%$\dmbfull \in \alpha_2 \land \dmbfull \in \beta_1$
%\end{theorem}


\begin{theorem}
\label{th:arm8dmbfullweaken}
Let $\srcp$ and $\tgtp$ be ARMv8 programs such that
$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \dmbld \cdot \dmbst \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \dmbst \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
The transformation is safe when: 

(i) $a=\Wlab(x,v) \land b=\Rlab(y,v') \implies x = y$ or 

(ii) $\exists c \in \alpha_2 \cdot \beta_1$ such that $c=\dmbfull$.
\end{theorem}


To prove \cref{th:arm8dmbfullweaken}, we show:
\[
\inarr{
\srcp \leadsto \tgtp \implies \forall \ex_t \in \denot{\tgtp}~\exists \ex_s \in \denot{\srcp}.~\behav(\ex_t) = \behav(\ex_s) 
}
\]


\begin{proof}

Given a target execution $\ex_t \in \denot{\tgtp}$ we define a source execution $\ex_s \in \srcp$. 
%by introducing the corresponding fence event $\event \in \dmbfull$. 

From definition we know that $\ex_t.\obs = \ex_s.\obs$, $\ex_t.\dob = \ex_s.\dob$, $\ex_t.\aob = \ex_s.\aob$. 

We know target execution $\ex_t$ satisfies (internal) and (atomic). 
From definition, source execution $\ex_s$ also supports (internal) and (atomic) as the respective relations remain unchanged. 

We now prove that $\ex_s$ satisfies (external). 

Considering $a = \denot{A}$ and $b = \denot{B}$ we consider following possibilities:

\Case{$(a,b) \in [\Rlab] \times [\E]$} 

In this case $(a,b) \in [\ex_s.\Rlab];\ex_s.\lpo;[\ex_s.\dmbfull];\ex_s.\lpo;[\ex_s.\E]$ and $(a,b) \in [\ex_t.\Rlab];\ex_t.\lpo;[\ex_t.\dmbld];\ex_t.\lpo;[\ex_t.\E]$

It implies both $\ex_s.\bob(a,b)$ and $\ex_t.\bob(a,b)$ hold.

\Case{$(a,b) \in [\Wlab] \times [\Wlab]$} 

In this case $(a,b) \in [\ex_s.\Wlab];\ex_s.\lpo;[\ex_s.\dmbfull];\ex_s.\lpo;[\ex_s.\Wlab]$ and $(a,b) \in [\ex_s.\Wlab];\ex_s.\lpo;[\ex_s.\dmbst];\ex_s.\lpo;[\ex_s.\Wlab]$

It implies both $\ex_s.\bob(a,b)$ and $\ex_t.\bob(a,b)$ hold.

We know that $\ex_t.\ob$ is acyclic and hence $\ex_s.\ob$ is also acyclic.

As a result, $\ex_s$ also satisfies (external) and is ARMv8 consistent.

\medskip

Moreover, we know that $\ex_s.\co = \ex_t.\co$. Hence $\behav(\ex_s)=\behav(\ex_t)$.

\end{proof}


%\begin{theorem}
%\label{th:arm8dmbldweaken}
%Suppose $\srcp$ is an ARMv8 program from an 
%x86 program following the mappings in \cref{tab:xarm}. 
%Let $C$ be an $\dmbld$ in a code sequence of the form $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \in \srcp(i)$ where $i$ is a thread identifier.
%Then $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \leadsto \alpha_1;A;\alpha_2;\cmp;\bc;\isync;\beta_1;B;\beta_2$ results in target program $\tgtp$ where $\alpha_1;A;\alpha_2;\skips;\beta_1;B;\beta_2 \in \tgtp(i)$. 
%The transformation is safe when 
%
%(i) there exists no $A$ and $B$ such that $A = \str \lor \osc$ and $B = \str$ or 
%
%(ii)  $\alpha_2$ or $\beta_1$ have $\dmbfull$ or $\dmbst$ fence.
%%
%%
%%(i) $\neg (A = \str \lor \osc \land B = \str)$ or 
%%
%%(ii) $\set{\dmbst, \dmbfull} \in \alpha_2 \lor \set{\dmbst, \dmbfull} \in \beta_1$
%\end{theorem}


\begin{theorem}
\label{th:arm8dmbldweaken}
Let $\srcp$ be an ARMv8 program  generated from an x86 program following the mappings in \cref{tab:xarm} and 
let $\tgtp$ be the program after weakening a $\dmbld$ to $\cmp;\bc;\isync$ in thread $i$ i.e. 
$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \isb \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \dmbld \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
The transformation is safe when: 

(i) $a=\Wlab(x,v) \land b=\Wlab(y,v') \implies x = y$ or 

(ii) $\exists c \in \alpha_2 \cdot \beta_1$ such that $c=\dmbfull \lor \dmbst$.
\end{theorem}



To prove \cref{th:arm8dmbldweaken}, we show:
\[
\inarr{
\srcp \leadsto \tgtp \implies \forall \ex_t \in \denot{\tgtp}~\exists \ex_s \in \denot{\srcp}.~\behav(\ex_t) = \behav(\ex_s) 
}
\]


\begin{proof}

Given a target execution $\ex_t \in \denot{\tgtp}$ we define a source execution $\ex_s \in \srcp$ by introducing the corresponding fence event $\event \in \dmbfull$. 

We know target execution $\ex_t$ satisfies (internal) and (atomic). 
From definition, source execution $\ex_s$ also supports (internal) and (atomic) as the respective relations remain unchanged. 

We now prove that $\ex_s$ satisfies (external) by showing $\ex_t.\ob = \ex_s.\ob$.

From definition we know that $\ex_t.\obs = \ex_s.\obs$, $\ex_t.\dob = \ex_s.\dob$, $\ex_t.\aob = \ex_s.\aob$. 

We now prove that $\ex_s$ satisfies (external). 

Considering $a = \denot{A}$ and $b = \denot{B}$ we consider following possibilities:

\Case{$(a,b) \in [\Rlab] \times [\E]$} 

In this case 

(i) $(a,b) \in [\ex_s.\Rlab];\ex_s.\lpo;[\ex_s.\Rlab];\ex_s.\lpo;[\ex_s.\dmbld];\ex_s.\lpo;[\ex_s.\Rlab];\ex_s.\lpo;[\ex_s.\Rlab];\ex_s.\lpo;[\ex_s.\E]$ and 

(ii) $(a,b) \in [\ex_t.\Rlab];\ex_t.\lpo;[\ex_t.\Rlab];\ex_t.\cmp;\ex_t.\bc;[\ex_t.\isb];\ex_t.\lpo;[\ex_t.\Rlab];\ex_t.\lpo;[\ex_t.\dmbld];\ex_t.\lpo;[\ex_t.\E]$ from \cref{tab:xarm}.

It implies both $\ex_s.\bob(a,b)$ and $\ex_t.\bob(a,b)$ hold.

\Case{$(a,b) \in [\Wlab] \times [\Wlab]$} 

In this case 

(i) $(a,b) \in [\ex_s.\Wlab];\ex_s.\lpo;[\ex_s.\Rlab];\ex_s.\lpo;[\ex_s.\dmbld];\ex_s.\lpo;[\ex_s.\Rlab];\ex_s.\lpo;[\ex_s.\Rlab];\ex_s.\lpo;[\ex_s.\E]$ and 

(ii) $(a,b) \in [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\Rlab];\ex_t.\cmp;\ex_t.\bc;[\ex_t.\isb];\ex_t.\lpo;[\ex_t.\Rlab];\ex_t.\lpo;[\ex_t.\dmbld];\ex_t.\lpo;[\ex_t.\E]$ from \cref{tab:xarm}.

In this case $\ex_s.\bob(a,b) \iff \ex_t.\bob(a,b)$.

We know that $\ex_t.\ob$ is acyclic and hence $\ex_s.\ob$ is also acyclic.

As a result, $\ex_s$ also satisfies (external) and is ARMv8 consistent.

\medskip

Moreover, we know that $\ex_s.\co = \ex_t.\co$. Hence $\behav(\ex_s)=\behav(\ex_t)$.
\end{proof}





%\section{Wrong Fence Weakening in ARMv8}
%
%Considering the strength of the fences in ARMv8,  we know $\isb \sqsubseteq \dmbld \dmbfull$ and $\dmbst \sqsubseteq \dmbfull$. 
%We can weaken fences based on its position especially after compiling from x86 and ARMv8. 
%For instance it is safe to weaken the $\dmbld$ 
%fence between read accesse pair, i.e. $\ldr;\dmbld;\ldr;\dmbld \leadsto \ldr;\isb;\bc;\ldr;\dmbld$ after
%$\mov(\Rlab);\mov(\Rlab) \leadsto \ldr;\dmbld;\ldr;\dmbld$ mappings. 
%
%Note that such weakening is not safe in general e.g. $\ldr;\dmbld;\ldr;\str \leadsto \ldr;\isb;\bc;\ldr;\str$ as in this case 
%we are removing a fence between the $\ldr$ and $\str$.  
%
%
%\begin{theorem}
%\label{th:arm8dmbstelim}
%{\color{red}
%This s wrong. Counter example $\str;\ldr;\dmbld;\ldr$. There is $\bob$ relation between the $\str$ and second $\ldr$. 
%Replacing $\dmbld$ by $\isync$ removes the $\bob$ relation.
%}
%Suppose $\srcp$ is an ARMv8 program from an 
%x86 program following the mappings in \cref{tab:xarm} and  
%there exists $\alpha;\ldr;\dmbld;\ldr;\beta \in \srcp(i)$ where $i$ is a thread identifier. 
%Then $\alpha;\ldr;\dmbld;\ldr;\beta \leadsto \alpha;\ldr;\cmp;\bc;\isync;\ldr;\beta$ transformation is safe.
%\end{theorem}
%
%To prove \cref{th:arm8dmbfullelim}, we show:
%\[
%\inarr{
%\srcp \leadsto \tgtp \implies \forall \ex_t \in \denot{\tgtp}~\exists \ex_s \in \denot{\srcp}.~\behav(\ex_t) = \behav(\ex_s) 
%}
%\]




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%Fences are required only between certain access pairs, for rest of the cases fences can be safely removed for x86, ARMv8, ARMv7 
%programs. 
%
%We define fence elimination transformation as follows: 
%\[
%\alpha;C;\beta \leadsto \alpha;\skips;\beta
%\]
%where $C$ is a fence.
%
%
%
%%$\felim(\srcp, \tgtp, A, B, C)$ where there exists $i$ such that  
%%\begin{itemize}
%%\item $\tau_1.A.\tau_2.\tau_3.B.\tau_4 \in \tgtp(i)$ 
%%\item $\tau_1.A.\tau_2.C.\tau_3.B.\tau_4 \in \srcp(i)$
%%%\item $\tau_2$ and $\tau_3$ have no fence access $D$ such that $C \sqsubseteq D$ 
%%\item $\denot{A}.\lloc \neq \denot{B}.\lloc$, $\denot{C}.\lloc = \bottom$
%%\end{itemize}
%%
%%We define 'singluar' fence as follows:
%%
%%
%%%%%%%%%%
%%%
%%%$\deletable(\ex, F, A, B)$
%%%
%%%A fence event F is deletable in $X$ if there exists no events $A, B$ 
%%%where $\ex.\lpo(A,X) \land \lpo(X,B)$ such that 
%%%not (A = st and B = ld) or 
%%%(A = st and B = ld) and there exists another fence $\ex.\lpo(A,D)$ and $\ex.\lpo(A,C)$. 
%%%
%%%%%%%%%%
%
%
%\subsection{Fence Elimination in x86}
%
%\begin{theorem}
%\label{th:xfenceelim}
%Let $C$ be an $\mfence$ in a given x86 code sequence of the form $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \in \srcp(i)$ where $i$ is a thread identifier.
%Then $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \leadsto \alpha_1;A;\alpha_2;\skips;\beta_1;B;\beta_2$ results in target program $\tgtp$ where $\alpha_1;A;\alpha_2;\skips;\beta_1;B;\beta_2 \in \tgtp$. 
%The transformation is safe when 
%
%(i) there exists no $A$ and $B$ such that $A = \mov(\Wlab)$ and $B = \mov(\Rlab)$ or 
%
%(ii)  $\alpha_2$ and $\beta_1$ have no $\mfence$.
%
%%
%%(i) $\neg (A = \mov(\Wlab) \land B = \mov(\Rlab))$ or 
%%
%%(ii) $\mfence \in \alpha_2 \lor \mfence \in \beta_1$
%\end{theorem}
%
%
%\begin{proof}
%
%We show:
%\[
%\inarr{
%\srcp \leadsto \tgtp \implies \forall \ex_t \in \denot{\tgtp}~\exists \ex_s \in \denot{\srcp}.~\behav(\ex_t) = \behav(\ex_s) 
%}
%\]
%
%Given a $\ex_t \in \denot{\tgtp}$ we define $\ex_s \in \srcp$ by introducing the corresponding fence event $\event$ such that  
%for all events $w \in \ex_s.\WUlab \cup \ex_s.\F$,
%\begin{itemize}
%\item if $(w,\event) \in \ex_s.\mo^?;\ex_s.\xhb$ holds then $\ex_s.\mo(w,\event)$. 
%\item Otherwise $\ex_s.\mo(\event,w)$.
%\end{itemize}
%
%%\begin{itemize}
%%\item $\ex_s.\mo(w,\event)$ when $w \in \ex_s.\WUlab \cup \ex_s.\F$ and $(w,\event) \in \ex_s.\mo^?;\ex_s.\xhb$. 
%%%\item 
%%%$\ex_s.\mo(\event,w)$ when $w \in \ex_s.\WUlab \cup \ex_s.\F$ and $(w,\event) \in \ex_s.\xhb;\ex_s.\mo^?$.
%%\end{itemize}
%We know $\ex_t$ is consistent. 
%
%Now we show $\ex_s$ is consistent.
%
%We prove by contradiction.
%
%(irrHB)
%Assume $\ex_s$ has $\ex_s.\xhb$ cycle. 
%We know the incoming and outgoing edges to $\event$ are $\ex_s.\lpo$ edges and therefore 
%$\ex_t.\xhb$ already has a cycle. 
%However, we know $\ex_t.\xhb$ is irreflexive. Hence a contradiction and $\ex_s.\xhb$ is irreflexive.
%
%\bigskip
%
%(irrMOHB)
%Assume $\ex_s$ has $\ex_s.\mo;\ex_s.\xhb$ cycle. 
%We already know that $\ex_t.\mo;\ex_t.\xhb$ is irreflexive. 
%Therefore the cycle contains $\event$. 
%Two possiblilities: 
%
%\Case{$\event \in \dom(\ex_s.\xhb)$ and $\event \in \codom(\ex_s.\mo)$}
%
%Suppose $\ex_s.\xhb(\event,w)$ and $\ex_s.\mo(w,\event)$. 
%However, from definition we already know $\ex_s.\xhb(\event,w) \implies \ex_s.\mo(\event,w)$ when $w \in \ex_s.\WUlab \cup \ex_s.\F$. 
%Hence a contradiction and $\ex_s.\mo;\ex_s.\xhb$ is irreflexive in this case.
%
%\Case{$\event \in \codom(\ex_s.\xhb)$ and $\event \in \dom(\ex_s.\mo)$}
%
%Suppose $\ex_s.\xhb(w,\event)$ and $\ex_s.\mo(\event,w)$. 
%However, from definition we already know $\ex_s.\xhb(w,\event) \implies \ex_s.\mo(w,\event)$ when $w \in \ex_s.\WUlab \cup \ex_s.\F$. 
%Hence a contradiction and $\ex_s.\mo;\ex_s.\xhb$ is irreflexive in this case.
%
%\bigskip
%
%(irrFRHB)
%We know $\ex_t$ does not have a $\ex_t.\fr;\ex_t.\xhb$ cycle.
%We also know $\fr \subseteq (\WUlab \times \WUlab)$ and hence event $\event \in \F$ does not introduce 
%any new $\ex_s.\fr;\ex_\xhb$ cycle. 
%Therefore $\ex_s.\fr;\ex_\xhb$ is irreflexive. 
%
%\bigskip
%
%(irrFRMO)
%
%We know $\ex_t$ does not have a $\ex_t.\fr;\ex_t.\mo$ cycle.
%We also know $\fr \subseteq (\WUlab \times \WUlab)$ and hence event $\event \in \F$ does not introduce 
%any new $\ex_s.\fr;\ex_\mo$ cycle. 
%Therefore $\ex_s.\fr;\ex_\mo$ is irreflexive. 
%
%\bigskip
%
%(irrFMRP)
%
%Assume $\ex_s$ has a $\ex_s.\fr;\ex_s.\mo;\ex_s.\rfe;\ex_s.\lpo$ cycle in $\ex_s$ cycle.
%
%In that case the cycle is of the form:
%
%$[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo;[\ex_s.\WUlab];\ex_s.\rfe;[\ex_s.\RUlab];\ex_s.\lpo;[\ex_s.\RUlab]$.
%
%We know $\event \in \F$ and therefore does not introduce this cycle in $\ex_s$.
%
%In that case $\ex_t$ already has a $\ex_t.\fr;\ex_t.\mo;\ex_t.\rfe;\ex_t.\lpo$ cycle which is a contradiction.
%
%Hence $\ex_s.\fr;\ex_s.\mo;\ex_s.\rfe;\ex_s.\lpo$ cycle in $\ex_s$ is irreflexive.
%
%\bigskip
%
%(irrUF)
%
%Assume $\ex_s$ has a $\ex_s.\fr;\ex_s.\mo;[\ex_s.\Ulab \cup \ex_s.\F];\ex_s.\lpo$ cycle.
%
%Two possiblities 
%
%\Case{$\ex_s.\fr;\ex_s.\mo;[\ex_s.\Ulab];\ex_s.\lpo$}
%
%It implies a $\ex_t.\fr;\ex_t.\mo;[\ex_t.\Ulab];\ex_t.\lpo$ cycle. 
%
%However, we know $\ex_t$ satisfies (irrUF) and hence a contradiction. 
%
%\Case{$\ex_s.\fr;\ex_s.\mo;[\ex_s.\F];\ex_s.\lpo$}
%
%It implies a $[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo;[\ex_s.\F];\ex_s.\lpo;[\ex_s.\RUlab]$ cycle 
%created by the introduced event $\event \in \F$.
%
%It implies $[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$
%
%From definition, we know $[\ex_s.\WUlab];\ex_s.\mo;[\set{\event}]$ when $[\ex_s.\WUlab];\ex_s.\mo^?;\ex_s.\xhb;[\set{\event}]$ holds.
%
%Thus $[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$
%
%$\implies [\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\xhb;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$
%
%$\implies [\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];(\ex_s.\xhb^?;[\ex_s.\WUlab];\ex_s.\rfe;\ex_s.\lpo \cup \ex_s.\lpo);[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$
%
%\begin{flalign*}
%\implies &  [\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\xhb^?;[\ex_s.\WUlab];\ex_s.\rfe;\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab] & \\
%& \cup [\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab] &
%\end{flalign*}
%
%\begin{flalign*}
%\implies &  [\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\xhb^?;[\ex_s.\WUlab];\ex_s.\rfe;\ex_s.\lpo;[\ex_s.\RUlab] & \\
%& \cup [\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab] &
%\end{flalign*}
%
%Now we consider two subcases:
%
%\Subcase{$[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\xhb^?;[\ex_s.\WUlab];\ex_s.\rfe;\ex_s.\lpo;[\ex_s.\RUlab] $}
%
%$\implies [\ex_t.\RUlab];\ex_t.\fr;[\ex_t.\WUlab];\ex_t.\mo^?;[\ex_t.\WUlab];\ex_t.\xhb^?;[\ex_t.\WUlab];\ex_t.\rfe;\ex_t.\lpo;[\ex_t.\RUlab]$
%
%$\implies  [\ex_t.\RUlab];\ex_t.\fr;\ex_t.\mo^?;\ex_t.\rfe;\ex_t.\lpo;[\ex_t.\RUlab]$
%
%This is a contradiction as $\ex_t$ satisfies (irrFMRP).
%
%\Subcase{$[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$}
%
%Now we consider the $[\ex_s.\WUlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$ subsequence.
%
%Possible cases:
%
%\Subsubcase{$[\ex_s.\Wlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\Rlab]$ }
%
%%%%%%%%%
%It implies $[\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\F];\ex_t.\lpo;[\ex_t.\Rlab]$ from the definition.
%
%$\implies [\ex_t.\Wlab];\ex_t.\mo;[\ex_t.\F];\ex_t.\lpo;[\ex_t.\Rlab]$.
%
%In that case there exists a $\ex_t.\fr;\ex_t.\mo;[\ex_t.\F];\ex_t.\lpo$ cycle. 
%
%This is a contradiction as $\ex_t$ satisfies (irrFMRP).
%
%\smallskip
%
%\Subsubcase{$[\ex_s.\WUlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\Ulab]$ }
%
%It implies $[\ex_t.\WUlab];\ex_t.\lpo;[\ex_t.\Ulab]$.
%
%It implies $[\ex_t.\WUlab];\ex_t.\mo;[\ex_t.\Ulab]$ as $\ex_t$ satisfies (irrMOHB).
%
%In this case $[\ex_s.\RUlab];\ex_s.\fr;[\ex_s.\WUlab];\ex_s.\mo^?;[\ex_s.\WUlab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\RUlab]$
%
%$\implies [\ex_t.\RUlab];\ex_t.\fr;[\ex_t.\WUlab];\ex_t.\mo^?;[\ex_t.\WUlab];\ex_t.\mo;[\ex_t.\Ulab]$
%
%$\implies [\ex_t.\RUlab];\ex_t.\fr;\ex_t.\mo;[\ex_t.\Ulab]$
%
%Hence a contradiction as $\ex_t$ satisfies (irrFRMO).
%
%\smallskip
%
%\Subsubcase{$[\ex_s.\Ulab];\ex_s.\lpo;[\set{\event}];\ex_s.\lpo;[\ex_s.\Rlab]$}
%
%It implies $[\ex_t.\Ulab];\ex_t.\lpo;[\ex_t.\Rlab]$ and in consequence a 
%$[\ex_t.\Rlab];\ex_t.\fr;[\ex_t.\WUlab];\ex_t.\mo^?;[\ex_t.\Ulab];\ex_t.\lpo;[\ex_t.\Rlab]$ cycle.
%
%Now, $[\ex_t.\Rlab];\ex_t.\fr;[\ex_t.\WUlab];\ex_t.\mo^?;[\ex_t.\Ulab];\ex_t.\lpo;[\ex_t.\Rlab]$
%
%$\implies [\ex_t.\Rlab];\ex_t.\fr;[\ex_s.\Ulab];\ex_t.\lpo;[\ex_t.\Rlab] \cup [\ex_t.\Rlab];\ex_t.\fr;\ex_t.\mo;[\ex_t.\Ulab];\ex_t.\lpo;[\ex_t.\Rlab]$
%
%$\implies [\ex_t.\Rlab];\ex_t.\fr;\ex_t.\xhb;[\ex_t.\Rlab] \cup [\ex_t.\Rlab];\ex_t.\fr;\ex_t.\mo;[\ex_t.\Ulab];\ex_t.\lpo;[\ex_t.\Rlab]$
%
%Hence a contradiction as $\ex_t$ satisfies (irrFRHB) and (irrUF).
%
%\bigskip
%
%$\behav(\ex_s) = \behav(\ex_t)$ holds as $\rloc{\ex_s.\mo} = \rloc{\ex_t.\mo}$.
%\end{proof}
%
%
%\subsection{Fence Elimination in ARMv8}
%
%\begin{observation}
%\label{obs:armv8fenceelim}
%Let $\mbbp$ be an ARMv8 program generated from an 
%x86 program following the mappings in \cref{tab:xarm}. 
%In this case for all consistent execution $\ex \in \denot{\mbbp}$ 
%the followings hold:
%
%\begin{enumerate}
%\item  A non-RMW load event is immediately followed by a $\dmbld$ event.
%\[\codom([\ex.\Rlab];(\imm(\ex.\lpo) \setminus \ex.\rmw) = [\ex.\dmbld]\]
%
%\item A non-RMW store event is immediately preceeded by a $\dmbst$ event, 
%\[\codom([\ex.\dmbst];\imm(\ex.\lpo)= [\ex.\Wlab]\]  
%
%\item An RMW is immediately preceeded by a $\dmbfull$ event, 
%\[\codom(\ex.\rmw^{-1};\imm(\ex.\lpo^{-1})) \subseteq \ex.\dmbfull\]
%
%\item An RMW is immediately followed by a $\dmbfull$ event, 
%\[\codom(\ex.\rmw;\imm(\ex.\lpo)) \subseteq \ex.\dmbfull\]
%\end{enumerate}
%\end{observation}
%
%%\begin{theorem}
%%\label{th:arm8dmbfullelim}
%%Let $\mapp$ be an ARMv8 program generated from an 
%%x86 program following the mappings in \cref{tab:xarm}. 
%%Suppose $\mapp$ contains a $\dmbfull$ fence 
%%
%%
%%$\felim(\srcp, \tgtp, A, B, \dmbfull)$ is safe in ARMv8 when 
%%$\neg (A = \str \lor \osc \land B = \oll \lor \ldr)$. 
%%\end{theorem}
%
%
%
%\begin{theorem}
%\label{th:arm8dmbfullelim}
%Suppose $\srcp$ is an ARMv8 program from an 
%x86 program following the mappings in \cref{tab:xarm}. 
%%$\felim(\srcp, \tgtp, A, B, \dmbfull)$ is safe in ARMv8 when 
%%$\neg (A = \str \lor \osc \land B = \oll \lor \ldr)$. 
%
%Let $C$ be an $\dmbfull$ in a code sequence of the form $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \in \srcp(i)$ where $i$ is a thread identifier.
%Then $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \leadsto \alpha_1;A;\alpha_2;\skips;\beta_1;B;\beta_2$ results in target program $\tgtp$ where $\alpha_1;A;\alpha_2;\skips;\beta_1;B;\beta_2 \in \tgtp$. 
%The transformation is safe when 
%
%(i) there exists no $A$ and $B$ such that $A = \str \lor \osc$ and $B = \oll \lor \ldr$ or 
%
%%$\neg (A = \str \lor \osc \land B = \oll \lor \ldr)$ or 
%
%(ii)  $\alpha_2$ and $\beta_1$ have no $\dmbfull$ fence.
%
%%$\dmbfull \in \alpha_2 \land \dmbfull \in \beta_1$
%\end{theorem}
%
%To prove \cref{th:arm8dmbfullelim}, we show:
%\[
%\inarr{
%\srcp \leadsto \tgtp \implies \forall \ex_t \in \denot{\tgtp}~\exists \ex_s \in \denot{\srcp}.~\behav(\ex_t) = \behav(\ex_s) 
%}
%\]
%
%
%\begin{proof}
%
%Given a target execution $\ex_t \in \denot{\tgtp}$ we define a source execution $\ex_s \in \srcp$ by introducing the corresponding fence event $\event \in \dmbfull$. 
%
%We know target execution $\ex_t$ satisfies (internal) and (atomic). 
%From definition, source execution $\ex_s$ also supports (internal) and (atomic) as the respective relations remain unchanged. 
%
%We now prove that $\ex_s$ satisfies (external). 
%
%%%%%%%%%%%%%%%%%%%%%%
%
%We prove by contradiction. 
%
%Assume $\ex_s$ violates (external).
%
%From definition we know that $\ex_s.\obs = \ex_t.\obs$, 
%$\ex_s.\dob = \ex_t.\dob$, $\ex_s.\aob = \ex_t.\aob$. 
%
%In that case there exists events $(a,b) \in \ex_s.\bob$ but $(a,b) \notin \ex_t.\bob$. 
%
%
%Considering possible cases of $a$ and $b$:
%
%
%\Case{$(a,b) \in [\ex_s.\Rlab] \times [\ex_s.\E]$} Two subcases:
%
%\Subcase{$a \notin \dom(\ex_s.\rmw)$}
%
%It implies $(a,b) \in [\ex_t.\Rlab];\ex_t.\lpo;[\ex_t.\dmbld];\ex_t.\lpo;[\ex_t.\E]$ from Observation (1) in \cref{obs:armv8fenceelim}.
%
%$\implies (a,b) \in [\ex_t.\Rlab];\ex_t.\bob;[\ex_t.\E]$
%
%Hence a contradiction and $\ex_s$ violates (external).
%
%\Subcase{$a \in \dom(\ex_s.\rmw)$}
%
%It implies $(a,b) \in [\ex_t.\Rlab];\ex_t.\lpo;[\ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\E]$
%
%$\implies (a,b) \in [\ex_t.\Rlab];\ex_t.\bob;[\ex_t.\E]$
%
%Hence a contradiction and $\ex_s$ violates (external).
%
%
%\Case{$(a,b) \in [\ex_s.\Wlab] \times [\ex_s.\Wlab]$}
%
%$\implies [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbst];\ex_t.\lpo;[\ex_t.\Wlab]$ from Observation (2) in \cref{obs:armv8fenceelim}.
%
%$\implies [\ex_t.\Wlab];\ex_t.\bob;[\ex_s.\Wlab]$ 
%
%This is a contradiction and hence $\ex_s$ satisfies (external). 
%
%\medskip
%
%\Case{$(a,b) \in [\ex_s.\Wlab] \times [\ex_s.\Rlab]$}
%
%It implies $(a,b) \in [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\Rlab]$ from the condition in \cref{th:armv8dmbfullelim}.
%
%$\implies [\ex_t.\Wlab];\ex_t.\bob;[\ex_s.\Rlab]$ 
%
%This is a contradiction and hence $\ex_s$ satisfies (external). 
%
%
%%%%%%%%%%%%%%%
%%
%%\Case{$(a,b) \in [\ex_s.\Rlab] \times [\ex_s.\E]$}
%%
%%$\implies [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbld];\ex_t.\lpo;[\ex_s.\Wlab]$ from Observation (2) in \cref{obs:armv8fenceelim}.
%%
%%$\implies [\ex_t.\Wlab];\ex_t.\bob;[\ex_s.\Wlab]$ 
%%
%%This is a contradiction and hence $\ex_s$ satisfies (external). 
%%
%%$\Case{$(a,b) \in [\ex_s.\Wlab] \times [\ex_s.\Rlab]$}
%%
%%$\implies [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbfull];\ex_t.\lpo;[\ex_s.\Rlab]$ from \cref{obs:armv8dmbfullelim}.
%%
%%$\implies [\ex_t.\Wlab];\ex_t.\bob;[\ex_s.\Rlab]$ 
%%
%%This is a contradiction and hence $\ex_s$ satisfies (external). 
%%
%%
%%
%%
%%%%%%%%%%%%%%%%%%%%%%%
%%
%%by showing $\ex_t.\ob = \ex_s.\ob$.
%%
%%From definition we know that $\ex_t.\obs = \ex_s.\obs$, $\ex_t.\dob = \ex_s.\dob$, $\ex_t.\aob = \ex_s.\aob$. 
%%We show that $\ex_s.\bob = \ex_t.\bob$.
%%
%%Considering the possible cases of $\ex_t.\bob$:
%%
%%\Case{$[\ex_t.\Wlab];\ex_t.\bob;[\ex_t.\Wlab]$}
%%
%%$\implies [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbst];\ex_t.\lpo;[\ex_s.\Wlab]$ from Observation (2) in \cref{obs:armv8fenceelim}.
%%
%%$\implies [\ex_s.\Wlab];\ex_s.\lpo;[\ex_s.\dmbst];\ex_s.\lpo;[\ex_s.\Wlab]$
%%
%%$\implies [\ex_s.\Wlab];\ex_s.\bob;[\ex_s.\Wlab]$
%%
%%\medskip
%%
%%\Case{$[\ex_t.\Wlab];\ex_t.\bob;[\ex_t.\Rlab]$}
%%
%%It implies $[\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\Rlab]$.
%%
%%In this case no fence is eliminated and hence $[\ex_s.\Wlab];\ex_s.\bob;[\ex_s.\Rlab]$ holds.
%%
%%\medskip
%%
%%\Case{$[\ex_t.\Rlab];\ex_t.\bob;[\ex_t.\Rlab \cup \ex_t.\Wlab]$}
%%
%%Two subcases:
%%
%%\Subcase{$[\ex_t.\Rlab];\ex_t.\rmw;\ex_t.\lpo;[\ex_t.\Rlab \cup \ex_t.\Wlab]$}
%%
%%It implies $[\ex_t.\Rlab];\ex_t.\rmw;\ex_t.\lpo;[\ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\Rlab \cup \ex_t.\Wlab]$
%%
%%$\implies [\ex_s.\Rlab];\ex_s.\rmw;\ex_s.\lpo;[\ex_s.\dmbfull];\ex_s.\lpo;[\ex_s.\Rlab \cup \ex_s.\Wlab]$
%%
%%$\implies [\ex_s.\Rlab];\ex_s.\aob;\ex_s.\bob;[\ex_s.\Rlab \cup \ex_s.\Wlab]$
%%
%%$\implies [\ex_s.\Rlab];\ex_s.\ob;[\ex_s.\Rlab \cup \ex_s.\Wlab]$
%%
%%\Subcase{Otherwise}
%%
%%It implies $[\ex_t.\Rlab];\ex_t.\lpo;[\ex_t.\dmbld];\ex_t.\lpo;[\ex_t.\Rlab \cup \ex_t.\Wlab]$
%%
%%$\implies [\ex_s.\Rlab];\ex_s.\lpo;[\ex_s.\dmbld];\ex_s.\lpo;[\ex_s.\Rlab \cup \ex_s.\Wlab]$
%%
%%$\implies [\ex_s.\Rlab];\ex_s.\bob;[\ex_s.\Rlab \cup \ex_s.\Wlab]$
%%
%%$\implies [\ex_s.\Rlab];\ex_s.\ob;[\ex_s.\Rlab \cup \ex_s.\Wlab]$
%%
%%\bigskip
%%
%%Thus $\ex_s.\ob = \ex_t.\ob$.
%
%\bigskip
%
%As a result, $\ex_s$ also satisfies (external) and is ARMv8 consistent.
%
%\medskip
%
%Moreover, we know that $\ex_s.\co = \ex_t.\co$. Hence $\behav(\ex_s)=\behav(\ex_t)$.
%
%
%\begin{theorem}
%\label{th:arm8dmbstelim}
%Suppose $\srcp$ is an ARMv8 program from an 
%x86 program following the mappings in \cref{tab:xarm}. 
%Let $C$ be an $\dmbst$ in a code sequence of the form $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \in \srcp(i)$ where $i$ is a thread identifier.
%Then $\alpha_1;A;\alpha_2;C;\beta_1;B;\beta_2 \leadsto \alpha_1;A;\alpha_2;\skips;\beta_1;B;\beta_2$ results in target program $\tgtp$ where $\alpha_1;A;\alpha_2;\skips;\beta_1;B;\beta_2 \in \tgtp$. 
%The transformation is safe when 
%
%(i) there exists no $A$ and $B$ such that $A = \str \lor \osc$ and $B = \str$ or 
%
%(ii)  $\alpha_2$ and $\beta_1$ have no $\dmbfull$ or $\dmbst$ fence.
%%
%%
%%(i) $\neg (A = \str \lor \osc \land B = \str)$ or 
%%
%%(ii) $\set{\dmbst, \dmbfull} \in \alpha_2 \lor \set{\dmbst, \dmbfull} \in \beta_1$
%\end{theorem}
%
%To prove \cref{th:arm8dmbstelim}, we show:
%\[
%\inarr{
%\srcp \leadsto \tgtp \implies \forall \ex_t \in \denot{\tgtp}~\exists \ex_s \in \denot{\srcp}.~\behav(\ex_t) = \behav(\ex_s) 
%}
%\]
%
%
%\begin{proof}
%
%Given a target execution $\ex_t \in \denot{\tgtp}$ we define a source execution $\ex_s \in \srcp$ by introducing the corresponding fence event $\event \in \dmbfull$. 
%
%We know target execution $\ex_t$ satisfies (internal) and (atomic). 
%From definition, source execution $\ex_s$ also supports (internal) and (atomic) as the respective relations remain unchanged. 
%
%We now prove that $\ex_s$ satisfies (external) by showing $\ex_t.\ob = \ex_s.\ob$.
%
%From definition we know that $\ex_t.\obs = \ex_s.\obs$, $\ex_t.\dob = \ex_s.\dob$, $\ex_t.\aob = \ex_s.\aob$. 
%
%In that case there exists events $(a,b) \in \ex_s.\bob$ but $(a,b) \notin \ex_t.\bob$. 
%
%
%Considering possible cases of $a$ and $b$:
%
%
%\Case{$(a,b) \in [\ex_s.\Rlab] \times [\ex_s.\E]$}
%
%
%It implies $(a,b) \in [\ex_t.\Rlab];\ex_t.\lpo;[\ex_t.\dmbld \cup \ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\E]$ from Observation (1) and (4) in \cref{obs:armv8fenceelim}.
%
%$\implies (a,b) \in [\ex_t.\Rlab];\ex_t.\bob;[\ex_t.\E]$
%
%Hence a contradiction and $\ex_s$ violates (external).
%
%
%\Case{$(a,b) \in [\ex_s.\Wlab] \times [\ex_s.\Wlab]$}
%
%$\implies [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbst \cup \ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\Wlab]$ from the condition in \cref{th:armv8dmbfullelim}.
%
%$\implies [\ex_t.\Wlab];\ex_t.\bob;[\ex_s.\Wlab]$ 
%
%This is a contradiction and hence $\ex_s$ satisfies (external). 
%
%\Case{$(a,b) \in [\ex_s.\Wlab] \times [\ex_s.\Rlab]$}
%
%It implies $(a,b) \in [\ex_s.\Wlab];\ex_s.\lpo;[\ex_s.\dmbfull];\ex_s.\lpo;[\ex_s.\Rlab]$ as $\ex_s.\bob(a,b)$ holds. 
%
%It implies $(a,b) \in [\ex_t.\Wlab];\ex_t.\lpo;[\ex_t.\dmbfull];\ex_t.\lpo;[\ex_t.\Rlab]$ 
%
%$\implies [\ex_t.\Wlab];\ex_t.\bob;[\ex_s.\Rlab]$ 
%
%This is a contradiction and hence $\ex_s$ satisfies (external). 
%\end{proof}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%\end{proof}

==> fenceopt-reachdefs.tex <==
% !TEX root = paper.tex


\section{Fence Optimizations}
\label{sec:fenceopt}

The proposed mapping schemes in \cref{sec:mappings} may introduce fences 
between access pairs where it is redundant. 
Some of these fences are redundant fences which can safely be eliminated without 
violating translation correctness.
To do so, we first check if a fence is \emph{non-eliminable}. 
If not, we delete the fence.  

In this section we prove the correctness of such fence eliminations. 
Along with we also propose respective fence elimination algorithms 
and prove their correctness. 

\subsection{x86 Fence Elimination}
\label{sec:xfenceelim}
In x86 only a store-load pair on different locations is unordered. 
Therefore if a fence appear between such a pair and there is such other fence 
then it is eliminable.
\begin{definition}
\label{def:xfelim}
Suppose an x86 program thread is of the form $\set{a \cdot \alpha_2 \cdot \Flab \cdot \beta_1 \cdot b \cdot \beta_2}$ where 
there $\nexists c \in  \alpha_2 \cdot \beta_1.~c = \Flab$. 
Fence $\Flab$ is \emph{non-eliminable} when $a=\Wlab(X,v) \land b=\Rlab(Y,v')$ where $X \neq Y$.
\end{definition}
If an $\mfence$ appears between any other pair 
of accesses then it is redundant. 
Such redundant fence may appear when an ARMv8 program is  
translated to x86 program following the mapping in \cref{tab:armx}. 
For instance, $\stlr;\str$ instruction sequence in ARMv8 results 
in $\movst;\mfence;\movst;$ access sequence. 
As $\movst$ accesses are ordered in x86, the intermediate $\mfence$ 
is redundant can safely be deleted. 
We prove the theorem in \cref{app:xfenceelim}.
\begin{restatable}{theorem}{xfenceelim}
\label{th:xfenceelim}
An \emph{$\mfence$} elimination is safe when it is \emph{not} non-eliminable as defined in \cref{def:xfelim}.
\end{restatable}

%%%%%%%%%%
%Considering such case we define \emph{non-eliminable} fence in x86. 
%
%Considering such case we state the safe fence 
%elimination in \cref{th:xfenceelim}. 
%We prove the theorem in \cref{app:xfenceelim}.
%
%\begin{restatable}{theorem}{xfenceelim}
%\label{th:xfenceelim}
%A fence elimination is safe when it is not \emph{non-eliminable}.
%%Let $\srcp$ be an x86 program and $\tgtp$ is the program after eliminating an $\mfence$ from thread $i$ i.e. 
%%$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \Flab \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
%%The transformation is safe when: 
%%
%%(i) $\neg (a=\Wlab(x,v) \land b=\Rlab(y,v') \land x \neq y)$ or
%%
%%%(ii) $a=\Wlab(x,v) \land b=\Rlab(y,v') \implies x = y$ or 
%%
%%(ii) $\Flab \in \alpha_2 \cdot \beta_1$
%\end{restatable}
%%%%%%%%%%%

\subsection{ARMv8 Fence Elimination (After x86 to ARMv8 Mapping)}

x86 to ARMv8 mapping scheme in \cref{tab:xarm} introduces various fence 
some of which are redundant.  
%different types of leading and/or trailing fences along with 
%memory accesses. 
Based on the access sequence in x86 some fences introduced in  
the translated ARMv8 sequence are redundant. 
For instance, an x86 access sequence $\movld;\movst$ on different locations 
results in $\ldr;\idmbld;\idmbst;\str$ sequence in ARMv8 where 
the $\dmbld$ suffices to order the load and store access pair and 
the $\dmbst$ is not required. 
However, we cannot immediately conclude that such a $\idmbst$ fence 
is entirely redundant if we consider an x86 access sequence 
$\mov(\Wlab);\mov(\Rlab);\mov(\Wlab)$. 
In this case the generated access sequence is 
$\dmbst;\Wlab;\Rlab;\dmbld;\dmbst;\str$ where the 
$\dmbst$ orders the two stores and therefore is not redundant.   
Considering these scenarios we define the non-eliminable 
$\idmbfull$ and $\idmbst$ fences in \cref{def:dmbfullelim,def:dmbst} and 
prove the safe fence eliminations in \cref{th:dmbfullelim,th:dmbstelim}.
\begin{definition}
\label{def:dmbfullelim}
Suppose $\mbbp$ be an ARMv8 program generated from an x86 program following the mappings in \cref{tab:xarm} with a thread 
of the form $\set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \dmbfull \cdot \beta_1 \cdot b \cdot \beta_2}$ where 
there $\nexists c \in  \alpha_2 \cdot \beta_1.~c = \dmbfull$. 
Fence $\dmbfull$ is \emph{non-eliminable} when $a=\Wlab(X,v) \land b=\Rlab(Y,v')$ where $X \neq Y$.
\end{definition}
\begin{restatable}{theorem}{dmbfullelim}
\label{th:dmbfullelim}
A \emph{$\idmbfull$} elimination is safe when it is \emph{not} non-eliminable as defined in \cref{def:dmbfullelim}.
%
%Let $\srcp$ be an ARMv8 program  generated from an x86 program following the mappings in \cref{tab:xarm} and 
%let $\tgtp$ be the program after eliminating a $\dmbfull$ from thread $i$ i.e. 
%$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \dmbfull \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
%The transformation is safe when: 
%
%(i) $\neg (a=\Wlab(x,v) \land b=\Rlab(y,v') \land x \neq y)$ or
%
%%(ii) $a=\Wlab(x,v) \land b=\Rlab(y,v') \implies x = y$ or 
%
%(ii) $\exists c \in \alpha_2 \cdot \beta_1$ such that $c = \dmbfull$
%
%%(iv) $(a,b) \in \slocs \setminus (\Rlab \times \Wlab)$
%%\TODO{Update the proof}
\end{restatable}
\begin{definition}
\label{def:dmbst}
Suppose $\mbbp$ be an ARMv8 program generated from an x86 program following the mappings in \cref{tab:xarm} with a thread 
of the form $\set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \dmbst \cdot \beta_1 \cdot b \cdot \beta_2}$ where 
there $\nexists c \in  \alpha_2 \cdot \beta_1.~c \in \set{\dmbfull, \dmbst}$. 
Fence $\dmbst$ is \emph{non-eliminable} when $a=\Wlab(X,v) \land b=\Wlab(Y,v')$ where $X \neq Y$.
\end{definition}  
\begin{restatable}{theorem}{dmbstelim}
\label{th:dmbstelim}
A \emph{$\idmbst$} elimination is safe when it is \emph{not} non-eliminable as defined in \cref{def:dmbst}.
%Let $\srcp$ be an ARMv8 program  generated from an x86 program following the mappings in \cref{tab:xarm} and 
%let $\tgtp$ be the program after eliminating a $\dmbst$ from thread $i$ i.e. 
%$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \dmbst \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
%The transformation is safe when: 
%
%(i) $\neg (a=\Wlab(x,v) \land b=\Wlab(y,v') \land x \neq y)$ or
%%
%%(ii) $a=\Wlab(x,v) \land b=\Wlab(y,v') \implies x = y$ or 
%
%(ii) $\exists c \in \alpha_2 \cdot \beta_1$ such that $c=\dmbfull \lor \dmbst$.
%%
%%(iv) $(a,b) \in \slocs \setminus (\Rlab \times \Wlab)$
%%\TODO{Update the proof}
\end{restatable}


\subsection{ARMv8 Fence Weakening}

In ARMv8 fence weakening implies replaces a $\idmbfull$ by a pair of $\idmbld$ and $\idmbst$ 
fences. 
We define safe fence weakening in \cref{th:dmbfullweaken} below 
and the detailed proof is in \cref{app:armv8fweaken}.
\begin{restatable}{theorem}{dmbfullweaken}
\label{th:dmbfullweaken}
Let $\srcp$ and $\tgtp$ be ARMv8 programs such that
$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \dmbld \cdot \dmbst \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \dmbfull \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
The transformation is safe when $\neg (a=\Wlab(x,v) \land b=\Rlab(y,v') \land x \neq y)$ 
%\TODO{Update the proof}
\end{restatable}
While fence weakening can be applied on any ARMv8 program, 
it is especially applicable after ARMv7/ARMv7-mca to ARMv8 mapping. 
ARMv7 has only $\idmb$ fence (except $\isb$) to order any pair of memory 
accesses and these $\idmb$ fences translates to $\idmbfull$ fence in ARMv8.  
In many cases these $\idmbfull$ fences can be weakened which in turn enable further 
fence eliminations.
 
\subsection{Fence Elimination in ARMv7/ARMv7-mca}

In ARMv7/ARMv7-mca we safely eliminate repeated fences and otherwise a fence is non-eliminable.

%%%%%%

\begin{definition}
\label{def:armsfelim}
Suppose an ARMv7 program thread is of the form $\set{a \cdot \alpha_2 \cdot \dmb \cdot \beta_1 \cdot b \cdot \beta_2}$ where $a$ and $b$ are memory accesses. 
Fence $\dmb$ is \emph{non-eliminable} when $\nexists c \in \alpha_2 \cdot \beta_1$ such that $c = \dmb$.
\end{definition}
\begin{restatable}{theorem}{armvsfenceelim}
\label{th:dmbelim}
A \emph{$\idmb$} elimination is safe when it is \emph{not} non-eliminable as defined in \cref{def:armsfelim}.
\end{restatable}
%\begin{proof}
%From the mapping scheme and the constraint in \cref{th:dmbelim}, in all the cases 
%there is a pair of $\dmb$ fences between the 
%access pairs and therefore one of the fences can be safely eliminated. 
%\end{proof}
We observe ARMv7 $\idmb$ fence elimination opportunities 
after the mapping from ARMv8 following the scheme in \cref{tab:armv8v7}.
%\begin{restatable}{theorem}{armvsfenceelim}
%\label{th:dmbelim}
%Let $\srcp$ be an ARMv7/ARMv7-mca program  generated from an ARMv8 program following the mappings in \cref{tab:armv8v7} and 
%let $\tgtp$ be the program after eliminating a $\dmb$ from thread $i$ i.e. 
%$\tgtp(i) \subseteq \srcp(i) \cup \set{\alpha_1 \cdot a \cdot \alpha_2 \cdot \beta_1 \cdot b \cdot \beta_2 \mid \alpha_1 \cdot a \cdot \alpha_2 \cdot \dmb \cdot \beta_1 \cdot b \cdot \beta_2 \in \srcp(i)} \land \forall j\neq i. \tgtp(j) = \srcp(j)$. 
%The transformation is safe when: 
%
%(i) $\neg (a.\op = \Wlab \lor b.\op = \Wlab)$ or 
%
%(ii) $\exists c \in \alpha_2 \cdot \beta_1.~c = \dmb$
%\end{restatable}
%
%\begin{figure}[t]
%\begin{subfigure}{0.9\textwidth}
%\begin{align*}
%\\ \opath(\iteri,\fnc,\iterj) & \triangleq \cfgto(\iteri,\fnc) \land \cfgto(\fnc,\iterj)
%\\ \mathsf{Imm}(\iteri,\iterj,\fnc) & \triangleq \iteri.\mathsf{next()} == \fnc \lor \iterj.\mathsf{prev()} == \fnc
%\\ \fexists(\nfs,  F, \iteri, \iterj) & \triangleq \exists \fnc' \in (\nfs \cap F).~\opath(\iteri,\fnc',\iterj) \land \predom(\fnc',\iterj)
%\\ \textbf{procedure } \oelim(\fs, \nfs) & \triangleq \fs \setminus \nfs 
%\end{align*}
%\end{subfigure}
%\\[1.1ex]
%\begin{subfigure}{0.47\textwidth}
%\begin{algorithmic}[1]
%\Procedure{$\getnfs$}{$\mathsf{lab},\maccs, \fs, F,\nfs$}
%\For{$\iteri \in \maccs$}
%\For{$\iterj \in \maccs$}
%\If {$\uord(\llab,\nfs,F,\iteri,\iterj)$}
%\If{$\cfgto(\iteri,\iterj)$}
%\State $\updnfs(\iteri,\iterj,\fs,F,\nfs)$
%\EndIf
%\EndIf  %\Comment{j-loop}
%\EndFor
%\EndFor
%\EndProcedure
%\end{algorithmic}
%%\vspace{4mm}
%\end{subfigure}
%\hfill
%\begin{subfigure}{0.47\textwidth}
%\begin{algorithmic}[1]
%\Procedure{$\updnfs$}{$\iteri,\iterj,\fs,F,\nfs$}
%\For{$\fnc \in \fs$}
%\If {$\opath(\iteri,\fnc,\iterj)$}
%%\If {$\uord(\mathsf{nfs},F,\iteri,\iterj)$}
%\State$\nfs \leftarrow \nfs \cup \fnc$
%%\EndIf %\Comment{unord}
%\If{$\oimm(\iteri,\iterj,\fnc)$}
%\State $\mathsf{return}$
%\EndIf  %\Comment{break}
%\EndIf
%\EndFor %\Comment{f}
%\EndProcedure
%\end{algorithmic}
%\end{subfigure}
%\caption{Helpers conditions and functions}
%\label{fig:helpers}
%\end{figure}
\subsection{Fence Optimization Algorithms}
We observe that the mapping schemes 
introduce fences which are not required and 
eliminating these fences do not affect 
program correctness. 
Therefore we propose fence elimination and fence weakening 
algorithms to remove redundant fences from a translated program. 
Our proposed algorithms broadly work in two steps. 
First, we check if a fence is \emph{non-eliminable}, 
that is, the fence is required to order a pair of memory accesses 
in at least one execution of the program.  
Second, we delete the fences which are not \emph{non-eliminable}. 
To perform these analyses we define a number of helper conditions and procedures  
in \cref{fig:helpers}. 
These helper conditions and procedures are used by various fence elimination algorithms.
\paragraph{Helper conditions and procedures} 
%We define a number of helper conditions in \cref{fig:conditions}.
Condition $\opath(\iteri,\fnc,\iterj)$ holds when 
$\fnc$ is reachable (checked by $\cfgto$ procedure) from $\iteri$ and $\iterj$ is reachable from 
$\fnc$ in the control-flow-graph(CFG) of program $P$. 
Given the CFG of program $P$,   
Condition $\oimm(\iteri,\fnc,\iterj)$ indicates that $\fnc$ is the immediate 
successor of $\iteri$ in the same basic block or immediate 
predecessor of $\iterj$ in the same basic block 
in the CFG of program $P$.
Condition $\fexists(\nfs, F, \iteri, \iterj)$ checks whether there exists 
some non-eliminable $F$ fence $\fnc'$ on the path from 
$\iteri$ to $\iterj$ and $\fnc'$ predominates $\iterj$ 
such that for all consistent executions events from $\iteri$ and $\iterj$ 
are always ordered by fence events from $\fnc'$. 

Procedure $\getnfs$ computes the set of non-eliminable fences $\nfs$ for 
fence type $\llab$ using the set of memory accesses $M$, 
set of fences $\fs$ of type $\llab$, and by $\updnfs$ procedure 
which populates $\nfs$. 
In this computation $\uord$ procedure call checks whether a pair 
of memory accesses from $M$ is already ordered by any 
non-eliminable fence from $\nfs$. 
We define $\uord$ conditions in detail for respective fence optimizations. 
Finally, $\oelim$ procedure eliminates the fences from $\fs$ 
which are redundant, that is, not in $\nfs$.  

%\begin{figure}
%\begin{algorithmic}[1]
%\Procedure{$\fexists$}{$\nfs, \fnc,  F, \iteri, \iterj$}
%\If{$\exists \fnc' \in \nfs \cap F~\postdom(\iteri,\fnc') \land \predom(\fnc',\iterj)$}
%\State return $\true$
%\EndIf
%\State return $\false$ 
%\EndProcedure
%\Procedure{$\uord$}{$\Flab, \iteri,\iterj$}
%\State return $\isSt(\iteri) \land \isLd(\iterj) \land \slocs(\iteri,\iterj) \land \neg \fexists(\nfs,\fnc,\Flab,\iteri,\iterj)$
%\EndProcedure
%\Procedure{$\uord$}{$\dmbfull,\iteri,\iterj$}
%\State return $\isSt(\iteri) \land \isLd(\iterj) \land \slocs(\iteri,\iterj) \land \neg \fexists(\nfs,\fnc,\dmbfull,\iteri,\iterj)$
%\EndProcedure
%\Procedure{$\uord$}{$\dmbst,\iteri,\iterj$}
%\State return $\isSt(\iteri) \land \isSt(\iterj) \land \slocs(\iteri,\iterj) \land \neg \fexists(\nfs,\fnc,\dmbfull \cup \dmbst,\iteri,\iterj)$
%\EndProcedure
%\end{algorithmic}
%\caption{$\uord$ functions.}
%\end{figure}

\paragraph{$\uord$ condition}
In \cref{th:xfenceelim,th:dmbfullelim,th:dmbstelim,th:dmbfullweaken,th:dmbelim} we define 
the conditions of safe fence elimination or weakening. 
A fence elimination or weakening may be unsafe in a consistent execution if the safety 
condition is not met due to the memory accesses around the fence.
For instance, in x86 consistent executions fence elimination between a pair of 
store ($\Wlab$) and load ($\Rlab$) events on different location 
may violate the safety condition.
Therefore we term $(\Wlab \times \Rlab) \setminus \slocs$ as an \emph{unordered} 
combination in x86. 
We lift the notion of \emph{unordered} combination in executions to memory access pairs in 
programs for a memory model or a mapping scheme and. 
We over-approximate such \emph{unordered} memory access pair for given instructions $\iteri$ and $\iterj$ 
by $\uord(\iteri,\iterj)$ analysis on a program for each fence elimination optimization.

%\begin{figure}[t]
%%\begin{subfigure}{0.9\textwidth}
%\begin{align*}
%\uord(\dmbfull,\nfs, F,\iteri,\iterj) & \triangleq \isSt(\iteri) \land \isLd(\iterj) \land \neg \slocs(\iteri,\iterj) \land \neg \fexists(\nfs,F,\iteri,\iterj)
%\\ \uord(\dmbst,\nfs,F,\iteri,\iterj) & \triangleq \isSt(\iteri) \land \isSt(\iterj) \land \neg \slocs(\iteri,\iterj) \land \neg \fexists(\nfs,F,\iteri,\iterj)
%\end{align*}
%%\end{subfigure}
%%\\[1.1ex]
%%\begin{subfigure}{0.47\textwidth}
%%\begin{algorithmic}[1]
%%\Procedure{Elimdmbfull}{$M,\df$}
%%\State $\getmemaccs(P,\maccs)$
%%\State $\getfences(P,\dmbfull,\df)$ %\Comment{enlist $\mfence$ operations}
%%%\State $\mathsf{nfs} \leftarrow \emptyset$
%%\State $\getnfs(\llab,\maccs,\df,\df,\nfs)$ %\mathsf{getnoelimfs}(\maccs,\fs)$
%%\State $\oelim(\df,\nfs)$
%%\EndProcedure
%%\end{algorithmic}
%%%\caption{Eliminate redundant $\dmbfull$ fences}
%%%\label{alg:dmbfelim}
%%\end{subfigure}
%%\hfill
%%\begin{subfigure}{0.47\textwidth}
%\begin{algorithmic}[1]
%\Procedure{ARMv8dmbElim}{$P$}
%\State $\getmemaccs(P,\maccs)$ \Comment{enlist shared memory accesses}
%\State $\getfences(P,\dmbfull,\df)$ \Comment{enlist $\dmbfull$ fences in $\df$}
%\State $\getfences(P,\dmbst,\ds)$  \Comment{enlist $\dmbst$ fences in $\ds$}
%%\State $\mathsf{nfs} \leftarrow \emptyset$
%\State $\getnfs(\dmbfull,\maccs,\df,\df,\nfs)$ \Comment{compute non-eliminable $\dmbfull$ fences in $\nfs$}
%\State $\getnfs(\dmbst,\maccs,\ds,\df \cup \ds,\nfs)$ \Comment{append non-eliminable $\dmbst$ fences to $\nfs$}
%\State $\oelim(\df \cup \ds,\nfs)$ \Comment{eliminate rest of the $\dmbfull$ and $\dmbst$ fences}
%\EndProcedure
%\end{algorithmic}
%%\caption{Eliminate redundant $\dmbst$ fences}
%%\label{alg:dmbstelim}
%%\end{subfigure}
%%
%%\hfill
%%\begin{subfigure}{0.47\textwidth}
%%\begin{algorithmic}[1]
%%\Procedure{$\mathsf{ARMv8FOpt}$}{$P$}
%%\State $\getmemaccs(P,\maccs)$
%%\State $\getfences(P,\dmbfull,\mathsf{df})$ %\Comment{enlist $\mfence$ operations}
%%%\State $\mathsf{nfs} \leftarrow \emptyset$
%%\State $\mathsf{getNFs}(\maccs,\mathsf{df},\mathsf{df},\mathsf{nfs})$ %\mathsf{getnoelimfs}(\maccs,\fs)$
%%\State $\getfences(P,\dmbst,\mathsf{ds})$ %\Comment{enlist $\mfence$ operations}
%%%\State $\mathsf{weakenf}(\mathsf{ds},\mathsf{nfs})$
%%\State $\mathsf{getNFs}(\llab,\maccs,\mathsf{ds},\mathsf{df} \cup \mathsf{ds},\mathsf{nfs})$ %\mathsf{getnoelimfs}(\maccs,\fs)$
%%\State $\mathsf{deletef}(\mathsf{ds},\mathsf{nfs})$
%%\EndProcedure
%%\end{algorithmic}
%%\caption{Fence Opt for x86-> ARMv8}
%%\label{alg:nonelimmf}
%%\end{subfigure}
%\caption{Fence Elimination after x86 to ARMv8 mapping. Initialize $\maccs, \mathsf{df}, \mathsf{ds},\mathsf{nfs}$ to $\emptyset$}
%\label{fig:armv8fopt}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{subfigure}{0.47\textwidth}
%\begin{algorithmic}[1]
%\Procedure{dmbFWeaken}{$P$}
%\State $\getmemaccs(P,\maccs)$
%\State $\getfences(P,\dmbfull,\mathsf{df})$ %\Comment{enlist $\mfence$ operations}
%%\State $\mathsf{nfs} \leftarrow \emptyset$
%\State $\mathsf{getNFs}(\llab,\maccs,\mathsf{df},\mathsf{df},\mathsf{nfs})$ %\mathsf{getnoelimfs}(\maccs,\fs)$
%\State $\mathsf{weakenf}(\mathsf{df},\mathsf{nfs})$
%\EndProcedure
%\end{algorithmic}
%\caption{Weaken $\dmbfull$ fences}
%\label{alg:nonelimmf}
%\end{subfigure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{minipage}{0.5\textwidth}
%\begin{algorithm}[H]
%\caption{Path Computation and Eliminate Redundant Fences}
%\label{alg:pathandelim}
%\begin{algorithmic}[1]
%\Procedure{$\opath$}{$\iteri,f,\iterj$}
%\State return $\cfgto(\iteri,f) \land \cfgto(f,\iterj)$
%\EndProcedure
%\Procedure{$\oelim$}{$\nelimfs, \mfences$}
%\For {$f \in \mfences$}
%\If{$f \notin \nelimfs$}
%\State $\mfences \leftarrow \mfences \setminus f$
%\EndIf
%\EndFor
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}
%\end{minipage}
%\hfill
%\begin{minipage}{0.49\textwidth}
%\begin{algorithm}[H]
%\caption{Mark non-eliminable fences}
%\label{alg:nonelim}
%\begin{algorithmic}[1]
%\Procedure{$\isnoelim$}{$f, \maccs$}
%\For{$\iteri \in \maccs$}
%\For{$\iterj \in \maccs$}
%\If {$\uord(\iteri,\iterj) \! \land \! \opath(\iteri,f,\iterj)$}
%\State return $\true$
%\EndIf
%\EndFor
%\EndFor
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}
%\end{minipage}
%\paragraph{Identify Non-eliminable Fences} 
%In this step we identify whether a fence is \emph{non-eliminable} 
%by analyzing the program.
%Suppose a program $P$ has a pair of unordered shared memory accesses 
%$\iteri$, $\iterj$ along with an intermediate fence $\fnc$, that is, 
%$f$ is reachable from $\iteri$ and $\iterj$ is reachable from 
%$f$ in control-flow-graph(CFG) of program $P$. 
%In this case fence $\fnc$ is \emph{non-eliminable}. 
%Thus the set of non-eliminable fences is a conservative 
%overapproximation of the fences required to preserve 
%the relations enforced by fence events during consistent executions. 
%We capture the non-eliminable fence computation in \cref{alg:getnfs} and \cref{alg:updnfs}.
%\paragraph{Fence Elimination}
%The fences which are not non-eliminable can safely be deleted 
%from a program as performed by $\oelim$ procedure.

%\begin{minipage}{0.5\textwidth}
%\begin{algorithm}[H]
%\caption{x86 Fence Elimination}
%\begin{algorithmic}[1]
%
%\Procedure{x86FenceElimination}{$P$}
%%\Algphase{Phase 1 - collect access pairs and fences}
%%\State $\maccs \leftarrow \emptyset$, $\mfences \leftarrow \emptyset$, $\nelimf \leftarrow \emptyset$ 
%%\State $\mfences \leftarrow \emptyset$ 
%\State $\nelimfs \leftarrow \emptyset$ 
%\State $\getmemaccs(P,\maccs)$
%\State $\getfences(\Flab,\mfences)$ %\Comment{enlist $\mfence$ operations}
%%\Algphase{Phase 2 - identify non-eliminable fences}
%\For {$f \in \mfences$}
%\If{$\isnoelim(f,\maccs)$}
%\State $\nelimfs \leftarrow \nelimfs \uplus f$ %\Comment{enlist non-eliminable fences}
%%\State $\mathsf{break}$
%\EndIf
%\EndFor
%%\Algphase{Phase 3 - eliminate fences which are not non-eliminable}
%\State $\oelim(\nelimfs, \mfences)$
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}
%\end{minipage}
%\hfill
%\begin{minipage}{0.49\textwidth}
%\begin{algorithm}[H]
%\caption{Check if $\iteri$ and $\iterj$ are unordered}
%\label{alg:x86uord}
%\begin{algorithmic}[1]
%\Procedure{$\uord$}{$\iteri,\iterj$}
%\State return
%\begin{align*}
%& \ \iteri.\op==\mov(\Wlab)
%\\ & \land \iterj.\op==\mov(\Rlab)
%\\ & \land \iteri.\locs \ !\!= \iterj.\locs
%\end{align*}
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}
%\end{minipage}
%
%
%\begin{algorithm}[H]
%\caption{mfence Elimination}
%\begin{algorithmic}[1]
%\Procedure{mfenceElim}{$P$}
%\State $\maccs \leftarrow \getmemaccs(P)$
%\State $\fs \leftarrow \getfences(\Flab)$ %\Comment{enlist $\mfence$ operations}
%\State $\nfs \leftarrow \mathsf{getnfs}(\maccs,\fs)$
%\State $\mathsf{deletef}(\fs,\nelimfs)$
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}l
%
%\begin{algorithm}[H]
%\caption{$\dmbfull$ Elimination}
%\begin{algorithmic}[1]
%\Procedure{mfenceElim}{$P$}
%\State $\maccs \leftarrow \getmemaccs(P)$
%\State $\fs \leftarrow \getfences(\dmbfull)$ %\Comment{enlist $\mfence$ operations}
%\State $\nelimfs \leftarrow \mathsf{getnoelimfs}(\maccs,\fs)$
%\State $\mathsf{deletef}(\fs,\nelimfs)$
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}
%
%
%
%
%\begin{figure}
%\begin{subfigure}{0.5\textwidth}
%\begin{algorithmic}[1]
%\Procedure{mFsElim}{$P$}
%\State $\maccs \leftarrow \getmemaccs(P)$
%\State $\fs \leftarrow \getfences(\Flab)$ %\Comment{enlist $\mfence$ operations}
%\State $\nfs \leftarrow \mathsf{getnfs}(\maccs,\fs)$
%\State $\mathsf{deletef}(\fs,\nelimfs)$
%\EndProcedure
%\end{algorithmic}
%\caption{Mark non-eliminable fence}
%\label{alg:nonelimmf}
%\end{subfigure}
%\hfill
%\begin{subfigure}{0.5\textwidth}
%\begin{algorithmic}[1]
%\Procedure{dFsElim}{$P$}
%\State $\maccs \leftarrow \getmemaccs(P)$
%\State $\fs \leftarrow \getfences(\Flab)$ %\Comment{enlist $\mfence$ operations}
%\State $\nfs \leftarrow \mathsf{getnfs}(\maccs,\fs)$
%\State $\mathsf{deletef}(\fs,\nelimfs)$
%\EndProcedure
%\end{algorithmic}
%\caption{Mark non-eliminable $\mfence$}
%\label{alg:nonelimmf}
%\end{subfigure}
%\caption{Mark non-eliminable $\mfence$}
%\label{alg:nonelimmf}
%\end{figure}



\begin{figure}[t]
\begin{align*}
%\acc(\cfg,i,\ell) \triangleq &  i \in \cfg.\V \land \itype(i) = \ell
%\\ 
%\pairs(\cfg, a, b) \triangleq & \set{(i,j) \mid \itype(i)=a \land \itype(j) = b \land \reach(\cfg,i,j)}
%\reach(\cfg,i,j) \triangleq & (i,j) \in [\cfg.\V];\cfg.\E^+;[\cfg.\V] 
\\ \reach(\cfg,i,j) \triangleq & \exists \tau \in \cfg.~\tau = \tau_1 \cdot (\denot{i}.\llab) \cdot \tau_2 (\denot{j}.\llab) \cdot \tau_3
\\ \opath(\cfg,i,f,j) \triangleq & \exists \tau \in \cfg.~\tau = \tau_1 \cdot (\denot{i}.\llab) \cdot \tau_2 (\denot{f}.\llab) \cdot \tau_3\cdot (\denot{j}.\llab) \cdot \tau_4
%\\ \opath(\cfg,i,f,j) \triangleq & \reach(\cfg,i,f) \land \reach(\cfg,f,j) 
%\\ \reachwo(\cfg, i, j, F) \triangleq & \reach(\cfg',i,j) \text{ where }
%\\  & \cfg'.\V = \cfg.\V \setminus F
%\text{ and } \cfg'.\E = \cfg.\E \setminus B \text{ where } B = (G.\V \times F) \cup (F \times G.\V)  
%\\ 
\\ \reachwo(\cfg, i, j, F) \triangleq & \forall \tau \in \cfg.~\exists f \in F.~\tau = \tau_1 \cdot (\denot{i}.\llab) \cdot \tau_2 (\denot{f}.\llab) \cdot \tau_3\cdot (\denot{j}.\llab) \cdot \tau_4
\\ \mpairs(\cfg, a, b) \triangleq & \set{(i,j) \mid \denot{i}.\op=a \land \denot{j}.\op=b \land \reach(\cfg,i,j)}
\\ \rnloc {\mpairs(\cfg, a, b)} \triangleq & \set{(i,j) \mid \mpairs(\cfg,a,b) \land \neg \mustalias(i,j)}
\\ \rloc {\mpairs(\cfg, a, b)} \triangleq & \set{(i,j) \mid \mpairs(\cfg,a,b) \land \mustalias(i,j)}
\end{align*}
\begin{subfigure}{0.45\textwidth}
\begin{algorithmic}[1]
\Procedure{getNFS}{$\cfg,PR,F, \nelim$}
\State $B \leftarrow \nelim$
\For{$f \in F, \ (i,j) \in PR$}
\If{$\opath(\cfg,i,f,j)$}
\If{$\reachwo(\cfg, i, j, B)$}
\State $B \leftarrow B \cup \set{f};$ 
\State $\lbreak;$
\EndIf
\EndIf
\EndFor
\State \Return $B$
\EndProcedure
\end{algorithmic}
\caption{Collect non-eliminable fences}
\end{subfigure}
\begin{subfigure}{0.52\textwidth}
\begin{algorithmic}[1]
\Procedure{FDelete}{$\cfg, F$}
%\State $\cfg'.\V \leftarrow \cfg.\V \setminus F$
%\State $\cfg'.\E \leftarrow \cfg.\E \setminus ((\cfg.\V \times F) \cup (F \times \cfg.\V))$ 

\State $\cfg' \leftarrow \forall f \in F.~\cfg \setminus \set{\tau \mid \exists f \in F.~\tau = \tau_1 \cdot \denot{f}.\llab \cdot \tau_2}$

\State \Return $\cfg'$
\EndProcedure
%\subcaption{Delete fences}
\Procedure{FWeaken}{$\cfg,F$}
\For{$f \in F$}
\State $\V_1 \leftarrow \cfg.\V \cup \set{a,b \mid \denot{a} = \dmbld \land \denot{b}=\dmbst}$
\State $\E_1 \leftarrow \cfg.\E \cup \set{(f,a), (a,b)}$ 
\State $\E_2 \leftarrow \E_1 \cup \set{(e,a) \mid G.\E(e,f)}$ 
\State $\E_3 \leftarrow \E_2 \cup \set{(b,e) \mid G.\E(f,e)}$
\State $\cfg'.\V \leftarrow \V_1 \setminus \set{f}$
\State $\cfg'.\E \leftarrow \E_3 \setminus ((\cfg'.\V \times \set{f}) \cup (\set{f} \times \cfg'.\V))$
\EndFor
\State \Return $\cfg'$
\EndProcedure
%\subcaption{Weaken fences}
\end{algorithmic}
\end{subfigure}
\caption{Helpers conditions and functions}
\end{figure}


\begin{figure}[t]
\begin{subfigure}{0.47\textwidth}
\begin{algorithmic}[1]
\Procedure{x86FElim}{$\cfg$}
\State $F = \set{f \mid f \in G.\V \land \denot{f}.\op = \F}$;
\State $SL \leftarrow \rnloc {\mpairs(\cfg,\Wlab,\Rlab)}$
\State $\nelim \leftarrow \texttt{getNFS}(\cfg,SL,F,\emptyset)$;
\State $\cfg \leftarrow \texttt{FDelete}(\cfg, \cfg.\V \setminus \nelim)$;
\EndProcedure
\end{algorithmic}
\subcaption{x86 fence elimination}
\bigskip
\bigskip
\begin{algorithmic}[1]
\Procedure{ARMv7FElim}{$\cfg$}
\State $F = \set{f \mid f \in G.\V \land \denot{f} = \dmb}$;
\State $SL \leftarrow \mpairs(\cfg,\Wlab,\Rlab)$;
\State $SS \leftarrow \mpairs(\cfg,\Wlab,\Wlab)$;
\State $LS \leftarrow \mpairs(\cfg,\Rlab,\Wlab)$;
\State $LL \leftarrow \mpairs(\cfg,\Rlab,\Rlab)$;
\State $M \leftarrow SL \cup SS \cup LS \cup LL$; 
\State $\nelim \leftarrow \texttt{getNFS}(\cfg,M,F,\emptyset)$;
\State $\cfg \leftarrow \texttt{FDelete}(\cfg, \cfg.\V \setminus \nelim)$;
\EndProcedure
\end{algorithmic}
\subcaption{ARMv7 fence elimination}
\end{subfigure}
\begin{subfigure}{0.47\textwidth}
\begin{algorithmic}[1]
\Procedure{ARMv8FElim}{$\cfg,\cfg'$}
\State $\nelim \leftarrow \emptyset$
\State $F = \set{f \mid f \in G.\V \land \denot{f} = \idmbfull}$;
\State $SL \leftarrow \rnloc {\mpairs(\cfg,\Wlab,\Rlab)}$
\State $\nelim \leftarrow \texttt{getNFS}(\cfg,SL,F,\emptyset)$;
\If{$\xarch \mapsto \arma$}
\State $\texttt{FDelete}(\cfg, \cfg.\V \setminus \nelim)$;
\Else
\State $\texttt{FWeaken}(\cfg,F \setminus \nelim)$
\EndIf
\State $FS = \set{f \mid f \in \cfg_1.\V \land \denot{f} = \idmbst}$;
\State $SS \leftarrow \rnloc {\mpairs(\cfg_1,\Wlab,\Wlab)}$
\State $FF \leftarrow \texttt{getNFS}(\cfg_1,SS,FS,\nelim)$;
\State $\texttt{FDelete}(\cfg_1, \cfg_2, FS \setminus FF)$;
\State $FF' \leftarrow \nelim$
\State $FL = \set{f \mid f \in \cfg_2.\V \land \denot{f} = \idmbld}$;
\State $LS \leftarrow \rnloc {\mpairs(\cfg_2,\Rlab,\Wlab)}$
\State $LL \leftarrow \rnloc {\mpairs(\cfg_2,\Rlab,\Rlab)}$
\State $FF' \leftarrow \texttt{getNFS}(\cfg_2,LL \cup LS,FL, \nelim)$;
\State $\texttt{FDelete}(\cfg_2, \cfg', FL \setminus FF')$;
\EndProcedure
\end{algorithmic}
\caption{ARMv8 fence elimination}
\end{subfigure}
\caption{Fence elimination algorithms}
\end{figure}

\subsubsection{Fence Elimination after x86 to ARMv8 Mapping (\cref{tab:xarm})}
We eliminate redundant $\dmbfull$ and $\dmbst$ 
fences after x86 to ARMv8 mapping in $\textsc{ARMv8dmbElim}$ procedure as shown in \cref{fig:armv8fopt}.
We first enlist shared memory accesses and fences. 
Then we compute non-eliminable $\dmbfull$ fences followed by non-eliminable $\dmbst$ fences. 
To compute the respective non-eliminable fences we define and use the $\uord$ 
conditions following \cref{th:dmbfullelim,th:dmbstelim} in \cref{fig:armv8fopt}.
Finally we eliminate rest of the fences.


%\begin{figure}[t]
%%\begin{subfigure}{0.9\textwidth}
%\begin{align*}
%\uord(\dmbfull,\nfs, F,\iteri,\iterj) & \triangleq \isSt(\iteri) \land \isLd(\iterj) \land \neg \slocs(\iteri,\iterj) \land \neg \fexists(\nfs,F,\iteri,\iterj)
%\\ \uord(\dmbld,\nfs,F,\iteri,\iterj) & \triangleq \isLd(\iteri) \land (\isLd(\iterj) \lor \isSt(\iterj)) \land (\iteri,\iterj) \notin \ollsc \land \neg \fexists(\nfs,F,\iteri,\iterj)
%\\ \uord(\dmbst,\nfs,F,\iteri,\iterj) & \triangleq \isSt(\iteri) \land \isSt(\iterj) \land \neg \slocs(\iteri,\iterj) \land \neg \fexists(\nfs,F,\iteri,\iterj)
%\\ \mathsf{weaken}(P,\nfs) & \triangleq P[\dmbfull \mapsto \dmbld;\dmbst]
%\end{align*}
%\begin{algorithmic}[1]
%\Procedure{ARMv8dmbWeaken}{$P$}
%\State $\getmemaccs(P,\maccs)$ \Comment{enlist shared memory accesses}
%\State $\getfences(P,\dmbfull,\df)$ \Comment{enlist $\dmbfull$ fences in $\df$}
%\State $\getfences(P,\dmbst,\ds)$  \Comment{enlist $\dmbst$ fences in $\ds$}
%\State $\getnfs(\dmbfull,\maccs,\df,\df,\nfs)$ \Comment{compute non-eliminable $\dmbfull$ fences in $\nfs$}
%\State $\weaken(\df,\nfs)$ \Comment{weaken rest of the $\dmbfull$ fences}
%\State $\getnfs(\dmbld,\maccs,\mathsf{dl},\df \cup \mathsf{dl},\nfs)$ \Comment{append non-eliminable $\dmbld$ fences to $\nfs$}
%\State $\getnfs(\dmbst,\maccs,\ds,\df \cup \ds,\nfs)$ \Comment{append non-eliminable $\dmbst$ fences to $\nfs$}
%\State $\oelim(\df \cup \ds,\nfs)$ \Comment{eliminate rest of the $\dmbld$ and $\dmbst$ fences}
%\EndProcedure
%\end{algorithmic}
%\caption{Fence Weakening and Elimination after ARMv7 to ARMv8 mapping. Initialize $\maccs, \mathsf{df}, \mathsf{ds},\mathsf{nfs}$ to $\emptyset$}
%\label{fig:armv8fopt}
%\end{figure}

\subsubsection{Fence Elimination after ARMv7 to ARMv8 Mapping (\cref{tab:armv7v8})}
Following the mapping scheme if an ARMv7 program is translated to a ARMv8 program 
then the ARMv8 program has only $\dmbfull$ fences. 
These $\dmbfull$ fences cannot be eliminated as they provide ordering between certain access pairs. 
However, in many cases a $\dmbld$ or a $\dmbst$ fence is enough to provide the desired ordering. 
Therefore following the \cref{th:dmbfullweaken} we weaken a $\dmbfull$ whenever possible.
\TODO{write the weakening theorem}
After weakening $\dmbfull$ fences, we perform the elimination of redundant $\dmbld$ and $\dmbst$ fences as 
shown in the $\textsc{ARMv7v8Opt}$ procedure in \cref{fig:ARMv7v8opt}.

\TODO{should we change the writing structure of armv8 fence elimination. Fence weakeing can be applied to any armv8.
program. Will see later.}

\subsection{x86 Fence Optimization}
In x86 an $\mfence$ is non-eliminable only when it appears between a pair of store and load accesses on different locations and  as shown in \cref{th:xfenceelim}. 
Note that the $\uord$ condition for $\mfence$ elimination in x86 is similar to that of $\dmbfull$ elimination in ARMv8 as follows.
\[
\uord(\F,\nfs, \F,\iteri,\iterj) \triangleq \isSt(\iteri) \land \isLd(\iterj) \land \neg \slocs(\iteri,\iterj) \land \neg \fexists(\nfs,\F,\iteri,\iterj)
\]
Therefore $\mfence$ elimination procedure is similar to that of ARMv8 $\dmbfull$ elimination. 

Considering the mapping scheme in \cref{tab:armx}, in the absence of $\stlr;\ldar$ access sequence on different locations, an $\stlr$ in introduces redundant fences. 
These fences can be eliminated by $\mfence$ elimination procedure.  

\subsection{ARMv7/ARMv7-mca Fence Optimization}

In ARMv7 a $\dmb$ is redundant when it it appears between a pair of same-location load-load, store-store, store-load, and atomic 
load-store accesses. 
Thus we define $\uord$ condition for $\dmb$ elimination in ARMv7 as follows.
\begin{align*}
\uord(\dmb,\nfs, \dmb,\iteri,\iterj) \triangleq & (\neg \slocs(\iteri,\iterj) \lor \slocs(\iteri,\iterj) \land \isLd(\iteri) \land \isSt(\iterj) \land (\iteri,\iterj) \notin \ollsc) 
\\ & \land \neg \fexists(\nfs,\dmb,\iteri,\iterj)
\end{align*}

Redundant fences appear in ARMv7 program after mapping ARMv8 programs to ARMv7/ARMv7-mca following the mapping scheme in \cref{tab:armv8v7}.
For example, a sequence $\ldr;\ldr$ in ARMv8 results in a sequence $\ldr;\dmb;\ldr;\dmb$ in ARMv7 where 
the introduced $\dmb$ instructions are redundant.  

\paragraph{Summary.} In this section we have discussed a number of fence elimination techniques using shared memory 
access sequences analysis around the fences. 
When analyzing the analyses do not consider the knowledge of other threads which may run in concurrence. 
Therefore the analyses preserve certain fences which are actually redundant considering the overall program structure. 
To optimize such programs further, in the next section we propose compositional analysis to perform further fences elimination.

==> robustness.tex <==
% !TEX root = paper.tex

\section{Static Robustness Analysis}
\label{sec:robustness}

A program $\mbbp$ is M-robust against K when all $M$ 
consistent executions of $\mbbp$ is also K-consistent.

If $M$ and $K$ are defined on same set of accesses then 
we check if an $M$-consistent execution also satisfies the 
consistency conditions of memory model $K$. 
However, if the accesses are different then we map a program 
$\srcp$ to $\tgtp$ and check whether for each $M$ consistent 
execution of $\srcp$ there exists a corresponding 
$K$ consistent execution of $\tgtp$.    

Note that for any program respective mapping schemes 
ensure robustness by introducing additional fences 
along with memory accesses. 
In this section we will consider mappings where we do not introduce 
addtional fence along with memory accesses during mapping. 

\paragraph{Approach} We apply compositional analysis to check robustness properties 
statically for a program for different architectural models. 
Note that in this analysis we compose the memory access pairs from possible 
different thread functions. 
However, we do not assume the number of threads created during an 
execution from each thread function.  
Therefore we provide a stronger guarantee; rather than one program 
our analysis guarantees robustness for a class of programs 
which uses same set of thread functions.

In this analysis we extend $\cyc$ to $\rcyc$ for relation $R$; 
we compute $\rcyc(\mbbp, R)$ where the memory access pairs are in relation $R$. 

\begin{definition}
$\ex.\epo = \ex.\lpo \cap \codom(\ex.\rfe \cup \ex.\coe \cup \ex.fre) \times \dom(\ex.\rfe \cup \ex.\coe \cup \ex.\fre)$ 
\label{def:epo}
\end{definition}


\begin{definition}
\begin{align*}
\rcyc(\mbbp,R) \triangleq & \set{(a,b) \mid (a,b) \in \pairs(\mbbp) \cap R \land \exists (p,q),( r,s) \in \pairs \cap R.~(a,b) \neq (p,q) \land (a,b) \neq (r,s) 
\\ & \land b.\lloc = p.\lloc \land a.\lloc = s.\lloc}
\end{align*}
\label{def:rcyc}
\end{definition}


\begin{definition}
$\pairs(\mbbp,i) \triangleq \set{(a,b) \mid a \cdot \tau \cdot b \in \mbbp(i)}$
\end{definition}

\begin{definition}
%$Re(a) \triangleq \exists j,p.~j \neq a.\tid \land p \in \mbbp(j). \land one(p,a) = \WUlab \land one(p,a) = \RUlab \land a.\lloc = p.\lloc$
% NOTE. We have to take R-->R cases also for non-MCA pattern.
$Re(a) \triangleq \exists j,p.~j \neq a.\tid \land p \in \mbbp(j). \land a.\lloc = p.\lloc \land (a \in \RUlab \implies \WUlab_{a.\lloc} \neq \emptyset) \land (a \in \WUlab \implies \RUlab_{a.\lloc} \neq \emptyset)$
\end{definition}


\begin{definition}
$\cyc(\mbbp,i) \triangleq \set{(a,b) \mid (a,b) \in \pairs(\mbbp,i) \land \exists j,k.~j \neq i \land k \neq i \land Re(a) \land Re(b)}$ 
\end{definition}

\begin{definition}
$\robust(\mbbp,R) \triangleq \forall i.~\cyc(\mbbp,i) \subseteq R$.
\end{definition}

\begin{definition}
An x86 program is x86-robust against SC if $\robust(\mbbp,R)$ holds where $R=...$.
\end{definition}


%\begin{definition}
%$\rcyc(\mbbp,i,R) \triangleq \forall (a,b) \in \pairs(\mbbp,i).~\exists j,k.~j \neq i \land k \neq i \land Re(a) \land Re(b) \implies R(a,b)$ 
%\end{definition}
 
%\begin{table}
%\begin{tabular}{c|c}
%x86 & ARMv8    \\
%\hline
%$\mov(\Rlab)$ & $\ldr$ \\
%$\mov(\Wlab)$ & $\ldr$ \\
%$\mathsf{lock \ cmpxchg}$ & $\ollsc$ \\
%$\mfence$ & $\dmbfull$   \\
%\end{tabular}
%\caption{Static Robustness of x86 to ARMv8 Mappings.}
%\label{tab:robustness-armx}
%\end{table}
%
%\begin{table}
%\begin{tabular}{c|c}
%ARMv8 & ARMv7    \\
%\hline
%$\ldr/\ldar$ & $\ldr$ \\
%$\str/\stlr$ & $\str$ \\
%$\ollsc$ & $\ollsc$ \\
%$\dmbfull$ & $\dmb$   \\
%$\dmbld$ & $\dmb$ \\
%$\dmbst$ & $\dmb$ \\
%$\isb$ & $\isync$
%\end{tabular}
%\caption{Static Robustness of ARMv8 to ARMv7 Mappings.}
%\label{tab:robustness-arm87}
%\end{table}
%
%More specifically we check if a program is:
%\begin{itemize}
%\item ARMv8 robust against SC and x86.
%\item ARMv7 robust against SC, x86, ARMv8, and ARMv7-mca.
%\item ARMv7-mca robust against SC, x86, and ARMv8.
%\end{itemize}

\subsection{x86}

%\begin{theorem}
%For a given program $\srcp$, mappings in \cref{tab:robustness-armx} is robust (has only x86 behaviors) if $\srcp$ has no $static-\ob$ cycle with $\Wlab \times \Wlab \cup \Rlab \times \Rlab \cup \Rlab \times \Wlab$ pairs.
%\end{theorem}

Now we check robustness of x86 programs against SC. 
An x86 program is robust against SC when the program has only 
SC behaviors, that is, interleaving executions. 
We define the required condition in the following \cref{th:xsc}.

\begin{restatable}{theorem}{xsc}
\label{th:xsc}
An x86 program $\mbbp$ is x86-robust against SC if $\robust(\mbbp,R)$ holds where $R = [\RUlab];\lpo \cup \lpo;[\WUlab] \cup \slocs \cup \cup \lpo;[\Flab];\lpo$ i.e. for all x86 consistent execution $\ex$, $\ex.\epo \subseteq \ex.R$ holds.
\end{restatable}

%Next, instead of enumerating all executions of program $\mbbp$ 
%we lift the notion to the thread semantics and perform a 
%conservative analysis of program robustness using the 
%following theorem \cref{th:pxsc}.
%
%\begin{restatable}{theorem}{pxsc}
%\label{th:pxsc} 
%An x86 program $\mbbp$ is x86-robust against SC if $\robust(\mbbp,R)$ holds
%%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp, R)$ 
%where $R = [\RUlab];\lpo \cup \lpo;[\WUlab] \cup \slocs \cup \cup \lpo;[\Flab];\lpo$.
%%$R= (\RWUlab \times \RWUlab) \setminus ([\Wlab];\lpo;[\Rlab] \setminus (\slocs \cup \lpo;[\Flab];\lpo))$.
%%%
%%%there exists no $\cyc(\mbbp, (\Wlab \times \Rlab) \setminus \slocs)$.
%\end{restatable}
%
%\begin{proof}
%For all consistent execution $\ex \in \denot{\mbbp}_{x86}$ 
%$\ex$ satifies SC. 
%Also from definition $\forall \ex \in \denot{\mbbp}_{x86}~R \implies \ex.\epo$. 
%Therefore we check a stricter condition under thread semantics and 
%as a result the program is x86 robust against SC.
%\end{proof}


\subsection{ARMv8}

%\begin{theorem}
%For a given program $\srcp$, mappings in \cref{tab:robustness-arm87} is robust if $\srcp$ has no $static-\wb$ cycle with $\Rlab \times \Rlab$ pairs where there exists set of $\Wlab$ with same locations.
%\end{theorem}

\begin{restatable}{theorem}{armasc}
\label{th:armasc}
An ARMv8 program $\mbbp$ is ARMv8-robust against SC if $\robust(\mbbp, R)$ hold where 
$R= \poloc \cup (\aob \cup \dob \cup \bob)^+$  i.e. for all x86 consistent execution $\ex$, $\ex.\epo \subseteq \ex.R$. 
\end{restatable}

%
%
%\begin{restatable}{theorem}{parmasc}
%\label{th:parmasc}
%An ARMv8 program $\mbbp$ is ARMv8-robust against SC if $\robust(\mbbp,\slocs)$ or $\robust(\mbbp, R)$ hold where 
%$R= \poloc \cup (\aob \cup \dob \cup \bob)^+$ hold.
%
%%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp,\slocs) \cup \rcyc(\mbbp, \aob \cup \bob \cup \dob)$.
%%%
%%%
%%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,\slocs) \lor c = \cyc(\mbbp, R)$ where $R = \aob \cup \bob \cup \dob$. 
%\end{restatable}
%
%\begin{proof}
%
%$\robust(\mbbp,\slocs)$ implies that a cycle may happen only by same-location events. 
%However, it would violate (sc-per-loc) in an execution. 
%Therefore no consistent execution would have such a cycle and all consistent execution 
%are SC consistent.
%Moreover, following \cref{tharmsc}, $\robust(\mbbp, (\ex.\aob \cup \ex.\dob \cup \ex.\bob)^+)$ satisfies SC robustness.
%\end{proof}

We define x86A; x86 constraints for ARMv8 consistent execution $\ex$.
\begin{itemize}
\item $\ex.\xhb$ is irreflexive. \hfill (AirrHB)
\item $\ex.\mo;\ex.\xhb$ is irreflexive. \hfill (AirrMOHB)
\item $\ex.\fr;\ex.\xhb$ is irreflexive. \hfill (AirrFRHB)
%\item $\ex.\fr;\ex.\mo$ is irreflexive. \hfill (AirrFRMO)
\item $\ex.\fr;\ex.\mo;\ex.\rfe;\ex.\lpo$ is irreflexive  \hfill (AirrFMRP)
\item $\ex.\fr;\ex.\mo;[\codom(\ex.\rmw) \cup \ex.\dmbfull];\ex.\lpo$ is irreflexive. \hfill (AirrUF)
%\item $[\ex.\rmw] \cap \ex.\fre;\ex.\coe = \emptyset$ is irreflexive. \hfill (ARMW)
\end{itemize}

We define $\ex.\mo$ such that   

\begin{itemize}

\item $[\ex.\Wlab \cup \ex.\dmbfull];\ex.\ob;[\ex.\Wlab \cup \ex.\dmbfull] \implies \ex.\mo$

\item $[\ex.\Wlab \cup \ex.\dmbfull];\ex.\lpo;[\ex.\Wlab \cup \ex.\dmbfull] \implies \ex.\mo$

\item $ [\ex.\dmbfull];\ex.\lpo;\ex.\fr \implies \ex.\mo$

\item $\ex.\co \implies \rloc {\ex.\mo}$

\end{itemize}


\begin{restatable}{theorem}{xA}
\label{th:x86A}
x86 and x86A are equivalent.
\end{restatable}

We define relation $\xwr$ as follows 
\[
\inarr{
\xwr= [\Wlab \cup \Llab \setminus \codom(\rmw)];\lpo;[\Rlab \cup \Alab \setminus \dom(\rmw)] \setminus (\slocs \cup (\Llab \times \Alab))
}
\]

\begin{restatable}{theorem}{robustarmax}
\label{th:robustarmax}
An ARMv8 program $\mbbp$ is ARMv8-robust against x86 if $\robust(\mbbp, R)$ holds where $R=\poloc \cup \xwr \cup (\aob \cup \bob \cup \dob)^+$   i.e. for all x86 consistent execution $\ex$, $\ex.\epo \subseteq \ex.R$ holds. 
\end{restatable}

%
%\begin{restatable}{theorem}{probustarmax}
%\label{th:probustarmax}
%An ARMv8 program $\mbbp$ is ARMv8-robust against x86 if $\robust(\mbbp, R)$ holds where $R=\poloc \cup \xwr \cup (\aob \cup \bob \cup \dob)^+$. 
%%%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp,\slocs) \cup \rcyc(\mbbp, R \cup \aob \cup \bob \cup \dob)$
%%
%%where $R= [\Wlab \cup \Llab \setminus \codom(\rmw)];\lpo;[\Rlab \cup \Alab \setminus \dom(\rmw)] \setminus (\slocs \cup (\Llab \times \Alab))$.
%%
%%
%%%
%%%
%%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,\slocs) \lor c = \cyc(\mbbp, R)$ where $R = \Wlab \setminus \codom(\rmw) \times \Rlab$. 
%\end{restatable}


\subsection{ARMv7}

\begin{restatable}{theorem}{robustarmssc}
\label{th:robustarmssc}
An ARMv7/ARMv7-mca program $\mbbp$ is ARMv7-robust against SC if $\robust(\mbbp,  R)$ hold where $R=\poloc \cup \fence$  i.e. for all x86 consistent execution $\ex$, $\ex.\epo \subseteq \ex.\poloc \cup \ex.\fence$ holds. 
%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp,\slocs) \cup \rcyc(\mbbp, R)$ 
%where $R =  \ppo \cup \fence$.
%%
%%
%%$\allcycle(\mbbp) \subseteq \set{\cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp, R) \mid R = \ppo \cup \fence}$.
%%
%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,\slocs) \lor c = \cyc(\mbbp, R)$ where $R = \ppo \cup \fence$. 
\end{restatable}

\begin{restatable}{theorem}{robustarmsx}
\label{th:robustarmsx}
An ARMv7/ARMv7-mca program $\mbbp$ is ARMv7-robust against x86 if $\robust(\mbbp, R)$ hold 
%
%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp,\slocs) \cup \rcyc(\mbbp, R)$ 
where $R = \poloc \cup \fence \cup [\Wlab \setminus \codom(\rmw)];\lpo;[\Rlab \setminus \dom(\rmw)]$  i.e. for all ARMv7 consistent execution $\ex$, $\ex.\epo \subseteq \ex.R$ holds.
%
%$\allcycle(\mbbp) \subseteq \set{\cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp, R) \mid R = \ppo \cup \fence \cup (\Wlab \setminus \codom(\rmw) \times \Rlab)}$.
%
%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,\slocs) \lor c = \cyc(\mbbp, R)$ where $R = \ppo \cup \fence \cup (\Wlab \setminus \codom(\rmw) \times \Rlab)$. 
\end{restatable}

\begin{restatable}{theorem}{robustarmsa}
\label{th:robustarmsa}
An ARMv7/ARMv7-mca program $\mbbp$ is ARMv7-robust against ARMv8 if $\robust(\mbbp,\slocs)$ or $\robust(\mbbp, R)$ hold where  $R= \poloc \cup [\Wlab];\lpo \cup \fence$ i.e. for all ARMv7 consistent execution $\ex$, $\ex.\epo \subseteq \ex.R$ holds.
%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp,\slocs) \cup \rcyc(\mbbp, [\Rlab];\ppo;[\Wlab] \cup \fence)$
%%$\cyc(\mbbp,[\Rlab];\ppo;[\Rlab]) \subseteq \set{\cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp,\fence)}$.
%%
%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,[\Rlab];\ppo;[\Rlab]) \implies c = \cyc(\mbbp, \slocs) \lor c = \cyc(\mbbp, \fence)$.
\end{restatable}

\begin{restatable}{theorem}{robustarmssmca}
\label{th:robustarmssmca}
An ARMv7 program $\mbbp$ is ARMv7-robust against ARMv7-mca if $\robust(\mbbp,\slocs)$ or $\robust(\mbbp, R)$ hold where $R=\poloc \cup \fence \cup [\Wlab];\lpo$ i.e. for all ARMv7 consistent execution $\ex$, $\ex.\epo \subseteq \ex.R$ holds.
%$\rcyc(\mbbp, \E \times \E) \subseteq \rcyc(\mbbp,\slocs) \cup \rcyc(\mbbp, [\Rlab];\ppo;[\Wlab] \cup \fence)$
%
%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,[\Rlab];\ppo;[\Rlab]) \implies c = \cyc(\mbbp, \slocs) \lor c = \cyc(\mbbp, \fence)$.
\end{restatable}

NOTE. $\data;\coi$ is not captured by $\ppo$. 
So having a $\ppo$ doe not guarantee $\dob$. 
scalar read read may have dob and ii0. 
But we keep fences in between. 
We'll use it in the analysis algorithm.

%
%\begin{theorem}
%An ARMv7-mca program $\mbbp$ is ARMv7-mca-robust against SC if 
%
%$\set{\cyc(\mbbp, \E \times \E)} \subseteq \set{ \cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp, R) \mid R =  \ppo \cup \fence}$.
%%
%%
%%$\allcycle(\mbbp) \subseteq \set{\cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp, R) \mid R = \ppo \cup \fence}$.
%%
%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,\slocs) \lor c = \cyc(\mbbp, R)$ where $R = \ppo \cup \fence$. 
%\end{theorem}
%
%\begin{theorem}
%An ARMv7-mca program $\mbbp$ is ARMv7-mca-robust against x86 if 
%
%$\set{\cyc(\mbbp, \E \times \E)} \subseteq \set{ \cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp, R) \mid R =  \ppo \cup \fence \cup (\Wlab \setminus \codom(\rmw) \times \Rlab)}$.
%%
%%$\allcycle(\mbbp) \subseteq \set{\cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp, R) \mid R = \ppo \cup \fence \cup (\Wlab \setminus \codom(\rmw) \times \Rlab)}$.
%%
%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,\slocs) \lor c = \cyc(\mbbp, R)$ where $R = \ppo \cup \fence \cup (\Wlab \setminus \codom(\rmw) \times \Rlab)$. 
%\end{theorem}
%
%\begin{theorem}
%An ARMv7-mca program $\mbbp$ is ARMv7-mca-robust against ARMv8 if 
%
%$\cyc(\mbbp,[\Rlab];\ppo;[\Rlab]) \subseteq \set{\cyc(\mbbp,\slocs)} \cup \set{\cyc(\mbbp,\fence)}$.
%%
%%$\forall c \in \allcycle(\mbbp).~ c = \cyc(\mbbp,[\Rlab];\ppo;[\Rlab]) \implies c = \cyc(\mbbp, \slocs) \lor c = \cyc(\mbbp, \fence)$.
%\end{theorem}

\TODO{Proofs done. Later revise.}

\TODO{Algorithm}

\subsection{Robustness Based Optimization}
If an ARMv8 program is x86 robust then we can remove a $\dmbfull$ fence between store and load. 
It keeps the ARMv8 program x86 robust.
